Interacting models for twisted bilayer graphene: a quantum chemistry approach

The nature of correlated states in twisted bilayer graphene (TBG) at the magic angle has received intense attention in recent years. We present a numerical study of an interacting Bistritzer-MacDonald (IBM) model of TBG using a suite of methods in quantum chemistry, including Hartree-Fock, coupled cluster singles, doubles (CCSD), and perturbative triples (CCSD(T)), as well as a quantum chemistry formulation of the density matrix renormalization group method (DMRG). Our treatment of TBG is agnostic to gauge choices, and hence we present a new gauge-invariant formulation to detect the spontaneous symmetry breaking in interacting models. To benchmark our approach, we focus on a simplified spinless, valleyless IBM model. At integer filling ($\nu=0$), all numerical methods agree in terms of energy and $C_{2z} \mathcal{T}$ symmetry breaking. Additionally, as part of our benchmarking, we explore the impact of different schemes for removing ``double-counting'' in the IBM model. Our results at integer filling suggest that cross-validation of different IBM models may be needed for future studies of the TBG system. After benchmarking our approach at integer filling, we perform the first systematic study of the IBM model near integer filling (for $|\nu|< 0.2$). In this regime, we find that the ground state can be in a metallic and $C_{2z} \mathcal{T}$ symmetry breaking phase. The ground state appears to have low entropy, and therefore can be relatively well approximated by a single Slater determinant. Furthermore, we observe many low entropy states with energies very close to the ground state energy in the near integer filling regime.

==> Quantum chemistry TBG/backup/comutator_norm.tex <==
Now that we have discussed how symmetry acts on our initial choice of creation and annihilation operators, will derive two gauge independent quantities, $\mc{C}_{\vk}$ and $\mc{C}_{\vk}^{\text{anti}}$, which check for symmetry breaking for unitary and antiunitary symmetries respectively.

Suppose that $\hat{H}_{\mathrm{IBM}}$ indeed satisfies a unitary symmetry $g$, and we are interested in whether the symmetry is spontaneously broken in the mean-field solutions \kds{I think we can use this to check whether the symmetry is broken using any method?}.\QZ{I agree.} 
If the many-body wavefunction $\ket{\Psi}$ satisfies the symmetry $g$, then
\[
g\ket{\Psi}\bra{\Psi}g^{-1}=\ket{\Psi}\bra{\Psi}.
\]
Here $g$ acting on $\ket{\Psi}$ is implemented by $g$ acting on each individual creation operators, and the vaccum is an eigenfunction of any symmetry $g\ket{0}=\ket{0}$.
Therefore the 1-RDM should satisfy
\begin{equation}
\begin{split}
[P(\vk)]_{nm}=&\braket{\Psi|\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}|\Psi}=\Tr[\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}\ket{\Psi}\bra{\Psi}]\\
=&\Tr[g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}g\ket{\Psi}\bra{\Psi}g^{-1}]\\
=&\braket{\Psi|g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}|\Psi}\\
=&\sum_{pq} [B(g)]_{\vk,pm} [B(g)]^*_{\vk,qn}\braket{\hat{f}^{\dag}_{p,g\vk} \hat{f}_{q,g\vk}}=([B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk})_{nm}.
\end{split}
\end{equation}
Therefore we can check the norm 
\begin{equation}
\label{eqn:order-parameter}
\mc{C}_{\vk}(g)=\norm{[B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk}-P(\vk)}=\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}
\end{equation}
to detect broken symmetry.

Similarly, for antiunitary symmetries we can check the norm
\begin{equation}
\label{eqn:order-parameter-anti}
\mc{C}^{\text{anti}}_{\vk}(g)=\norm{[B(g)]_{\vk}^{\dag}P(-g\vk)[B(g)]_{\vk}-P(\vk)^*}=\norm{P(-g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)^*}.
\end{equation}

Let us also show the connection between $\mc{C}_{\vk}(\mc{C}_{2z}\mc{T})$ and the order parameter used in \cite{SoejimaParkerBultinckEtAl2020} using a particular gauge fixing called the Chern band basis. In the Chern band basis, we have
\[
[B(C_{2z}\mc{T})]_{\vk}=\sigma_x  e^{\I \theta(\vk)}
\]
for some $\vk$-dependent phase $\theta(\vk)$. 
In this basis, the $C_{2z}\mc{T}$ symmetry breaking is detected by computing
\begin{equation}
\gamma_z(\vk)=\Tr[P(\vk)\sigma_z]=P_{11}(\vk)-P_{22}(\vk).
\end{equation}

\QZ{Should $C_{2z}\mc{T}$ be antiunitary?}

On the other hand, the commutator satisfies
\[
P(\vk)[B(C_{2z}\mc{T})]_{\vk}-[B(C_{2z}\mc{T})]_{\vk}P(\vk)=e^{\I \theta(\vk)}
\begin{pmatrix}
P_{21}(\vk)-P_{12}(\vk) & P_{22}(\vk)-P_{11}(\vk)\\
P_{11}(\vk)-P_{22}(\vk) & P_{12}(\vk)-P_{21}(\vk)
\end{pmatrix}
\]
Therefore $\gamma_z(\vk)$ can be interpreted as checking the magnitude of the off-diagonal element of commutator in the Chern band basis. \QZ{However, the order parameter $\gamma_z(\vk)$ is designed specifically for the Chern band basis and $C_{2z}\mathcal{T}$ symmetry, which is unable to generalize to the other band basis and other symmetries. On the other hand, the commutator is designed for any symmetries of our interests and works for any band basis. Using the norm of commutator, a clear spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetries is observed for both BM band basis and Chern band basis in Section \ref{sec:numerical}.}



==> Quantum chemistry TBG/backup/multi_band.tex <==
In our previous sections, two flat bands $u_{\pm1,\vk}$ with different sublattice index $\sigma=\pm$ are used to project the Hamiltonian and compute the corresponding sewing matrices. Meanwhile, we make the assumption that all the states with band index $n<-1$ ($n>1$) are full (empty). This is enough for the first magic angle $\theta=1.1^{\circ}$, since this two flat bands are isolated from the other energy bands in the band structure of BM model. However, for the other magic angles, there doesn't exist such isolated flat bands. Therefore, we need to include more bands in our projection in order to get numerically accurate results. Generally, we assume that $2N_{\max}$ bands are used and all the states with band index $n<-N_{\max}$ ($n>N_{\max}$) are full (empty). Away from the flat band case, the band energies are also relatively away from zero. One more symmetry needs to be defined here for the multi-band case, which is unitary ``particle-hole symmetry'' $\mc{P}$\cite{song_2019}\cite{TBGII}\cite{TBGIII}:
\begin{equation}
[D(P)]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',-\vG} \delta_{l',-l} \delta_{\sigma',\sigma}\zeta_l,
\end{equation}
where $\mc{P}\vk=-\vk$ and $\zeta_l=\pm1$ for $l=\pm$. Note that $\mc{P}$ anticommutes with the BM Hamiltonian and $\mc{P}$ maps creation operators to creation operators (rather than annihilation operators). Therefore, ``particle-hole symmetry'' is mainly a map from positive energy band $u_{n\vk}$ to negative energy band $u_{-n\vk}$. Using the particle-hole symmetry $\mc{P}$ and rotation symmetry $C_{2z}$, the band structure of the BM Hamiltonian has the property:
\begin{equation}
    \epsilon_{n,\vk}=-\epsilon_{-n,-\vk},\ \epsilon_{n,\vk}=\epsilon_{n,-\vk}\ \to\ \epsilon_{n,\vk}=-\epsilon_{-n,\vk}.
\end{equation}

This band structure also implicitly reflects that $\epsilon_{1,\vk}=\epsilon_{-1,\vk}=0$ in the two flat band case. Away from the flat band case, one pair of bands with positive/negative energies should be included in our set of bands and this pair is connected by the ``particle-hole symmetry''. Besides that, in order to ensure the ``completeness'' of the symmetry operation, $u_{n\vk}$ and $D(g)u_{n\vk}$ should also be included. with this setup, our norm of the commutator can be generalized to the multi-band case by defining
\begin{equation}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u_{n\vk}},\ \ \ m,n\in[-N_{\max},N_{\max}].
\end{equation}


% This is enough for our discussion about $C_{2z}\mc{T}$ and $C_{3z}$ symmetry in the single-valley, spinless system. However, if we want to further discuss about other symmetries, more bands are needed. One example is the rotation symmetry $C_{2x}$:
% \begin{equation}
% [D(C_{2x})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',C_{2x}\vG} \delta_{l',-l} \left(\sigma_x\right)_{\sigma',\sigma},
% \end{equation}
% where $C_{2x}\vk=C_{2x}\left(k_x,k_y\right)=\left(k_x,-k_y\right)$.

% The sewing matrices are $[B(C_{2x})]_{\vk,mn}=[B(C_{2z})]_{\vk,mn}$ if only two flat bands are used. Moreover, the ``completeness'' is broken since $D(C_{2z})$


==> Quantum chemistry TBG/backup/symm_bm.tex <==


\QZ{In this section, we introduce the matrix representation of the symmetry operation and discuss the discrete symmetries of the non-interacting BM model. These definitions help us get prepared for the following discussion about the projected IBM Hamiltonian in Section \ref{sec:ibm-symm} and the spontaneous symmetry breaking in Section \ref{sec:symm-broken}.}

%\QZ{In the single-valley, spinless system, we abbreviate the valley and spin dimension.} We introduce a multi-index $\alpha=(\vG,\sigma,l)$ to denote the ``internal variables'', i.e., the BM wavefunction is $u_{n\vk}(\alpha)$, and the total number of internal variables is $N_{\alpha}$. The action of a discrete symmetry operator $g$ on the fermion basis $\hat c^{\dag}_{\vk}(\alpha)$ is
%\begin{equation}
%g\hat{c}^{\dag}_{\vk}(\alpha)g^{-1} = \sum_{\alpha'} 
%\hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha}.
%\end{equation}
%The unitary matrix $D(g)\in \CC^{N_{\alpha}\times N_{\alpha}}$ is called the representation matrix.
%Similarly $g$ acting on the annihilation operators 
%\begin{equation}
%g\hat{c}_{\vk}(\alpha)g^{-1} = \sum_{\alpha'} 
%\hat{c}_{g\vk}(\alpha') [D(g)]^*_{\alpha',\alpha}.
%\end{equation}
%A symmetry $g$ is unitary if for any $c\in \CC$, $gcg^{-1}=c$. 
%A symmetry $g$ is antiunitary if for any $c\in \CC$, $gcg^{-1}=c^*$. 

For example, the $C_{3z}$ symmetry is unitary which maps the $\vK$ valley into an equivalent $\vK$ valley. Specifically, it maps $\vK+\vk\to \vK+C_{3z}\vk$.
So
\begin{equation}
(C_{3z})\hat{c}^{\dag}_{\vk}(\vG,\sigma,l)(C_{3z})^{-1} = \sum_{\alpha'}
\hat{c}^{\dag}_{C_{3z}\vk}(\vG',\sigma',l') [D(C_{3z})]_{\alpha',\alpha}.
\end{equation}
with
\begin{equation}
[D(C_{3z})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',C_{3z}\vG} \delta_{l',l} \left(e^{\I \frac{2\pi}{3} \sigma_z}\right)_{\sigma',\sigma}.
\end{equation}
The $C_{2z}\mc{T}$ symmetry is antiunitary which maps $\vk\to \vk$
\begin{equation}
(C_{2z}\mc{T})\hat{c}^{\dag}_{\vk}(\vG,\sigma,l)(C_{2z}\mc{T})^{-1} = \sum_{\alpha'}
\hat{c}^{\dag}_{\vk}(\vG',\sigma',l') [D(C_{2z}\mc{T})]_{\alpha',\alpha}.
\end{equation}
with
\begin{equation}
[D(C_{2z}\mc{T})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',\vG} \delta_{l',l} (\sigma_x)_{\sigma',\sigma}.
\end{equation}
 
The BM Hamiltonian commutes with both $C_{2z}\mc{T}$ and $C_{3z}$. 




==> Quantum chemistry TBG/backup/symm_broken.tex <==
\QZ{I adjusted the indices in this follwing content.}


%When the energy band basis $\hat{f}^{\dagger}_{n\vk}$ is fixed, the matrix representations of unitary/antiunitary operators are also fixed. In the other word, sewing matrices are the same up to a arbitrary unitary rotation and explicit forms of sewing matrices can be obtained only when this unitary rotation is fixed.
Next, we will show that $\mc{C}_{\vk}(g)$ is invariant under arbitrary unitary rotation. We perform an unitary rotation $U(\vk)$ on the original basis. Towards these ends, suppose that we perform the mapping
%In particular, we are able to map the original basis into the Chern band basis using the unitary rotation defined in \cite{SoejimaParkerBultinckEtAl2020}.
\[
\hat{f}^{\dagger}_{n\vk} \mapsto \sum_{n'}\hat{f}^{\dagger}_{n'\vk}[U(\vk)]_{n'n}.
\]

Under this unitary rotation, the 1-RDM is
\begin{equation}
\begin{split}
[P(\vk)]_{nm}\to&\braket{\Psi|\sum_{m'}\hat{f}^{\dagger}_{m'\vk}[U(\vk)]_{m'm} \sum_{n'}[U(\vk)]^*_{n'n}\hat{f}_{n'\vk}|\Psi}\\
=&\sum_{m'n'}[U(\vk)]_{m'm}[U(\vk)]^*_{n'n}\braket{\Psi|\hat{f}^{\dagger}_{m'\vk} \hat{f}_{n'\vk}|\Psi},\\
=&(U^{\dagger}(\vk)P(\vk)U(\vk))_{nm}.
\end{split}
\end{equation}
By a similar calculation, it can be checked that the sewing matrices transform as:
\begin{equation}
[B(g)]_{\vk,mn} \mapsto (U^{\dagger}(g\vk)B(g)_{\vk}U(\vk))_{mn}
\end{equation}
Therefore, the norm is
\begin{equation}
\begin{split}
\mc{C}_{\vk}(g)\to&\norm{U^{\dagger}(g\vk)P(g\vk)U(g\vk)U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)-U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)U^{\dagger}(\vk)P(\vk)U(\vk)},\\
=&\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}.
\end{split}
\end{equation}

\LL{ The antiunitary case requires separate treatment.} 

==> Quantum chemistry TBG/backup/symm_ibm.tex <==
In order to check the symmetries of the interacting BM model, we need to discuss the interacting term in \cref{eqn:interaction_simplify}. For unitary/antiunitary operator, it is sufficient to verify the symmetries of form factors:
$$
[\Lambda_{\vk}(\vq)]_{mn}=\braket{u_{m\vk}|u_{n,\vk+\vq}},
$$
where $u_{m\vk}$, $u_{n,\vk+\vq}$ are the flat bands in the BM band structure. It has been proven that the BM model has $C_{2z}\mc{T}$ symmetry. Given a flat band $u_{m\vk}$, another band $D[g]u_{m\vk}$ is also a flat band. For example, two flat bands can be chosen as $u_{1,\vk}$ and $u_{-1,\vk}=\sigma_xu^*_{1,\vk}$. With this kind of setup, the flat bands always include the pairs of bands and each pair is connected by one specific symmetry. In this case, the symmetry operation using sewing matrix can also be ``closed'' and ``complete''. In Chern band basis $u_{\pm,\vk}=u_{\pm1,\vk}$, the sewing matrix is defined as $[B(C_{2z}\mathcal{T})]_{\vk,mn}=\braket{u_{m\vk}|\sigma_x|u^*_{n\vk}}=\braket{u_{m\vk}|u_{-n\vk}}=\delta_{m,-n}$. In random band basis $u_{\pm,\vk}=c_{\pm,1,\vk}u_{1,\vk}+c_{\pm,-1,\vk}u_{-1,\vk}$, the sewing matrix is $[B(C_{2z}\mathcal{T})]_{\vk,mn}=c^*_{m,-1,\vk}c^*_{n,1,\vk}+c^*_{m,1,\vk}c^*_{n,-1,\vk}$. It's easy to verify that these sewing matrices are ``closed'' and ``complete''.


Then for unitary operator, we have

\begin{equation}
\begin{split}
[[B(g)]^{\dag}_{\vk} \Lambda_{g\vk}(\vq) [B(g)]_{\vk+\vq}]_{mn}&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'} [\Lambda_{g\vk}(\vq)]_{n'm'}[B(g)]_{\vk+\vq,m'n},\\
&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'}\braket{u_{n',g\vk}|u_{m',g\vk+g\vq}}[B(g)]_{\vk+\vq,m'n}\\
&=\braket{u_{m\vk}|D^{\dag}(g)D(g)|u_{n,\vk+\vq}},\\
&=\braket{u_{m\vk}|u_{n,\vk+\vq}}=[\Lambda_{\vk}(\vq)]_{mn},
\end{split}
\end{equation}
and for antiunitary operator: 
\begin{equation}
\begin{split}
[[B(g)]^{\dag}_{\vk} \Lambda_{g\vk}(\vq) [B(g)]_{\vk+\vq}]_{mn}&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'} [\Lambda_{g\vk}(\vq)]_{n'm'}[B(g)]_{\vk+\vq,m'n},\\
&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'}\braket{u_{n',g\vk}|u_{m',g\vk+g\vq}}[B(g)]_{\vk+\vq,m'n}\\
&=\braket{u^*_{m\vk}|D^{\dag}(g)D(g)|u^*_{n,\vk+\vq}},\\
&=\braket{u^*_{m\vk}|u^*_{n,\vk+\vq}}=[\Lambda^*_{\vk}(\vq)]_{mn}.
\end{split}
\end{equation}

This holds for both BM and Chern band basis. To summarize, the flat bands connected by the desired symmetry should be included to form a complete set of basis in the projected space.

For the subtraction term in \cref{eqn:subtracted_HF}, it can be verified using
\begin{equation}
[B(g)]^{\dag}_{\vk}h_s(g\vk)[B(g)]_{\vk}=h_s(\vk),
\end{equation}
which is equivalent to verify that $[B(g)]^{\dag}_{\vk}\delta P^0(g\vk+g\vq)[B(g)]_{\vk}=\delta P^0(\vk+\vq)$ for unitary operator. Therefore, the symmetries of the subtracted Hamiltonian still holds if the reference density also have the same symmetries. Some common choice of the reference density includes: (i) the ground state density of the BM model; (ii) the ground state density of the decoupled BM model; (iii) the charge neural point ($\delta P^0=0$). All these choice share the same symmetries with BM model.

==> Quantum chemistry TBG/backup/symm_notation.tex <==
\QZ{ For the eigenstates $u_{n\vk}$, we have $u_{n\vk}=u_{n\vk}(\alpha)$.}

Symmetries play an important role in both the theoretical understanding of the Bistrizter MacDonald Hamiltonian as well as in numerical simulations. In this work, we consider symmetries which can be written as a composition of operators from two different classes (1) Euclidean symmetries (i.e. translations, rotations, and reflections) and (2) complex conjugation. While these \kds{first few sections. (depends on how the rest of the section is written)} will focus on studying symmetries at a very abstract level, in Section \ref{sec:bm-symm} we will explicitly show how $C_{2z} \mc{T}$ and $C_{3z}$ can be realized in our parameterization of the IBM.

Given a choice of creation and annihilation operations, any symmetry operation can be completely determined by how it acts on the Fock space. For unitary symmetries, it suffices to describe how the symmetry acts on a basis of creation and annilhilation operators. In particular, for any Euclidean symmetry $g$, due to the properties of the Bloch transform, there exists a unitary $D(g)$, called the representation matrix, so that the creation operators transform via the rule
\begin{equation}
\begin{split}
    (g \hat{\vc}_{\vk}^\dag g^{-1})(\alpha) & = \sum_{\alpha'} \hat{\vc}_{g\vk}^\dag(\alpha') [D(g)]_{\alpha',\alpha} \\
    (g \hat{\vc}_{\vk} g^{-1})(\alpha) & = \sum_{\alpha'} \hat{\vc}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha}^{*}
\end{split}
\end{equation}
where $g\vk$ denotes the action of the symmetry $g$ in $\vk$-space and $\hat{\vc}_{\vk}$ are the creation operators \kds{defined in Section III}. 

In contrast to unitary symmetries, the action of complex conjugation must be defined with respect to a fixed choice of creation and annihilation operators. Throughout this section, we will define complex conjugation with respect to creation operators $\{ \hat{\vc}_{\vk}^\dag \}$ so that if $\mc{K}$ denote complex conjugation, then any linear combination of creation operators transforms as:
\begin{equation}
\begin{split}
    \mc{K} \left( \sum_{\alpha} a_{\alpha} \hat{\vc}_{\vk}^\dag(\alpha)  \right) \mc{K} =  \sum_{\alpha} a_{\alpha}^{*} \hat{\vc}_{-\vk}^\dag(\alpha) \\
    \mc{K} \left( \sum_{\alpha} a_{\alpha} \hat{\vc}_{\vk}(\alpha)  \right) \mc{K} =  \sum_{\alpha} a_{\alpha}^{*} \hat{\vc}_{-\vk}(\alpha) 
\end{split}
\end{equation}


As a first step toward studying symmetries in the Bistrizter Macdonald model, we will first show how we can write the action of $g$ in terms of its representation matrix $D(g)$. If $g$ is a unitary symmetry with corresponding representation matrix $D(g)$, then
\begin{equation}
\begin{split}
g\hat{H}_{\mathrm{BM}} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
=& \sum_{\vk} [D(g)h(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
\end{split}
\end{equation}
If $\hat{H}_{\mathrm{BM}}$ is invariant under $g$, then this calculation shows that at the matrix level:
\begin{equation}
D(g) h(\vk)=h(g\vk) D(g).
\end{equation}
In other words, 
\begin{equation}
h(g\vk)D(g)u_{n\vk}=D(g)h(\vk)u_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk},
\end{equation}
or equivalently $D(g)u_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$.

This allows us to define a ``sewing matrix'', $[B(g)]_{\vk}$,
\begin{equation}
\label{eqn:matrix_representation}
(D(g) u_{n\vk})(\alpha)=
\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}(\alpha')=
\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
\end{equation}
\kds{It is critical here that the system is gapped. If the bands are entangled, we are no longer guaranteed that $\{ \ket{u_{n,g\vk}} \}_{n \in \mc{I}}$ spans the same space as $\{ D(g) \ket{u_{n,\vk}} \}_{n \in \mc{I}}$ where $\mc{I}$ is an arbitrary index set. Not sure how to explain this...} Here 
\begin{equation}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk} | D(g) | u_{n\vk}},
\end{equation}
and $[B(g)]_{\vk}$ is a unitary matrix. \kds{Note that $D(g)$ isn't Hermitian, perhaps we should use different notation here?} \QZ{ The original representation matrix $D(g)$ is defined in the space of combined indices $\alpha$, while sewing matrix $[B(g)]_{\vk}$ is defined in the band space. It's obvious that the symmetry operation is complete using the representation matrix. Using sewing matrix, the symmetry operation is also complete when all the bands are used. In practice, the number of bands is limited. Therefore, our goal is that the symmetry operations of our interests are ``closed'' and ``complete'' using the corresponding sewing matrices: Given a set of bands $\{u_{n\vk}\}_{n,\vk}$, a)``closed'':  for any unitary/antiunitary operator $g$ of interest, $\sum_{m}  u_{m,g\vk} [B(g)]_{\vk,mn}\in\{u_{n\vk}\}_{n,\vk}$; b) ``complete'': for any $u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ and unitary (antiunitary) operator $g$ of interest, $D(g)u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ ($D(g)u^*_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$) and $D(g)u_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$ ($D(g)u^*_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$). In this note, we are particularly interested in the spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetry. In a single-valley, spinless system, one pair of flat bands with different sublattice index $\sigma=\pm$ is enough to satisfy the conditions above. More details are in Section \ref{sec:ibm-symm}}


Given the definition of sewing matrices, for unitary operator $g$, one can calculate that:
\[
\begin{split}
g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}(\alpha')\\
=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
u_{n\vk}(\alpha)\\
=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
\end{split}
\]
Hence the sewing matrices define how $\hat{f}^{\dag}_{n\vk}$ transforms under the symmetry action.

Now to turn to consider antiunitary symmetries. Since any antiunitary transformation can be written as $g \mc{K}$ where $g$ is a unitary transform and $\mc{K}$ is complex conjugation, similar calculations show that if $\hat{H}_{\mathrm{BM}}$ is invariant under an antiunitary symmetry then the corresponding matrix equation is:
\begin{equation}
D(g) h(\vk)=h(-g\vk)^* D(g).
\end{equation}
From this matrix relation, one can check that the corresponding sewing matrix can be defined by the relations:
\begin{equation}
\begin{split}
(D(g) u_{n\vk})(\alpha) & =
\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}^*(\alpha')=
\sum_{m}  u_{m,-g\vk}(\alpha) [B(g)]_{\vk,mn} \\
[B(g)]_{\vk,mn} & = \braket{u_{m,-g\vk} | D(g) | u^*_{n\vk}}.
\end{split}
\end{equation}
Using these definitions, we can now calculate how $f^\dag_{n\vk}$ transforms under antiunitary symmetry: 
\[
\begin{split}
(g \mc{K}) \hat{f}^{\dag}_{n\vk} (g \mc{K})^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}^*(\alpha')\\
=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
u_{n\vk}^*(\alpha)\\
=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,-g\vk}(\alpha') [B(g)]_{\vk,mn} \\
=& \sum_{m} \hat{f}^{\dag}_{m,-g\vk}  [B(g)]_{\vk,mn}.
\end{split}
\]



%\QZ{Maybe move the antiunitary case to the Appendix.}
%
%The case when $g$ is antiunitary is similar. 
%Here
%\begin{equation}
%\begin{split}
%g\hat{H}_{\mathrm{BM}} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
%=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]^*_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
%=& \sum_{\vk} [D(g)h^*(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
%\end{split}
%\end{equation}
%So
%\begin{equation}
%D(g) h^*(\vk)=h(g\vk) D(g).
%\end{equation}
%Hence
%\begin{equation}
%h(g\vk)D(g) u^*_{n\vk}=D(g) h^*(\vk)u^*_{n\vk}=\varepsilon^*_{n\vk} D(g)u^*_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk}.
%\end{equation}
%In other words, $D(g)u^*_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$. 
%The sewing matrix is then given by 
%\begin{equation}
%(D(g) u^{*}_{n\vk})(\alpha)=
%\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u^{*}_{n\vk}(\alpha')=
%\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
%\end{equation}
%Here 
%\[
%[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u^*_{n\vk}}
%\]
%and $[B(g)]_{\vk}$ is a unitary matrix. The transformation rule remains the same
%\begin{equation}
%\begin{split}
%g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u^*_{n\vk}(\alpha')\\
%=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
%u^*_{n\vk}(\alpha)\\
%=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
%=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
%\end{split}
%\end{equation}
%


With the transformation rule set by the sewing matrices, we can check whether a quadratic Hamiltonian 
$\hat{A}=\sum_{\vk}\sum_{mn}[A(\vk)]_{mn} \hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}$
commutes with the symmetry $g$. 
If $g\hat{A}g^{-1}=\hat{A}$, and assume that the Monkhorst-Pack grid discretizing the mBZ is invariant under $g$, then
\begin{equation}
\begin{split}
g\hat{A}g^{-1}=&\sum_{\vk}\sum_{mn} [A(\vk)]_{mn}\sum_{pq} [B(g)]_{\vk,pm} [B(g)]^*_{\vk,qn} \hat{f}^{\dag}_{p,g\vk}\hat{f}_{q,g\vk}\\
=&\sum_{g\vk} \sum_{pq} \left([B(g)]_{\vk} A(\vk) [B(g)]_{\vk}^{\dag}\right)_{pq}\hat{f}^{\dag}_{p,g\vk}\hat{f}_{q,g\vk}.
\end{split}
\end{equation}
Therefore we have the relation 
\begin{equation}
[B(g)]_{\vk} A(\vk) [B(g)]^{\dag}_{\vk}-A(g\vk)=0.
\end{equation}
Similarly, if $g$ is antiunitary, then
\begin{equation}
[B(g)]_{\vk} A^*(\vk) [B(g)]^{\dag}_{\vk}-A(-g\vk)=0.
\end{equation}

The same procedure can be used to check whether the quartic Hamiltonian commutes with $g$. \QZ{ As in \cref{eqn:subtracted_HF}, the single-particle term in the subtracted Hamiltonian is a quartic term. Therefore, the symmetries will be verified by setting $A(\vk)=h_s(\vk)$ in Section \ref{sec:ibm-symm}.}

\QZ{ For the coulomb interaction term,} due to the structure in \cref{eqn:interaction_simplify}, it is sufficient to verify that $g$ commutes with the pseudo-density operator $\hat{\rho}_{\vq}$ in \cref{eqn:rho_operator}, which is a quadratic operator.
Direct computation shows that if $g$ is unitary and commutes with $\hat{\rho}_{\vq}$,
then
\begin{equation}
[B(g)]_{\vk} \Lambda_{\vk}(\vq) [B(g)]^{\dag}_{\vk+\vq}-\Lambda_{g\vk}(g\vq)=0.
\end{equation}
If $g$ is antiunitary, then
\begin{equation}
[B(g)]_{\vk} \Lambda^*_{\vk}(\vq) [B(g)]^{\dag}_{\vk+\vq}-\Lambda_{g\vk}(g\vq)=0.
\end{equation}

Using the strategy above, we can verify that $g\hat{H}_{\mathrm{IBM}}g^{-1}=\hat{H}_{\mathrm{IBM}}$ for $g=C_{2z}\mc{T},C_{3z}$ in the continuous limit. \QZ{ More details are in Section \ref{sec:ibm-symm}.} However, in a calculation with a finite number of $\vk$ points, the symmetry may be slightly broken. 
Therefore we need to check the norm of the commutators above to verify that the magnitude of the broken symmetry is sufficiently small. \QZ{ The definition of the norm and the discussion of symmetry breaking are discussed in Section \ref{sec:symm-broken}.}



% KDS: I think what you have below is good, but the operators $\hat{\vc}$ are already defined in Section III
%\QZ{ $\hat{\vc}_{n\vk}^\dag/\hat{\vc}_{n\vk}$ is the creation/annihilation operator defined in the space of combined indices $\alpha=(\vG, s,\sigma,\tau,l)$, including the Moir\'e reciprocal lattice vector, spin, sublattice, valley, layer, and $n$ represents the unique band index. Note that the combined indices $\alpha$ and band indices $n$ are correlated with each other.} Unlike unitary symmetries, the action of complex conjugation is defined with respect to a choice of basis. Recalling


==> Quantum chemistry TBG/preamble.tex <==
\usepackage{color, xcolor, colortbl}
\usepackage{graphicx}
\usepackage{geometry}
\usepackage{amsthm,amsmath,amssymb,amsfonts}
%\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{epstopdf}
\usepackage{bm}
%\usepackage[caption=false]{subfig}
%\usepackage{subcaption}
\usepackage{appendix}
\usepackage{multirow}
\usepackage{braket}
\usepackage[english]{babel}
\usepackage{hyperref}
\usepackage[capitalize]{cleveref}
%\usepackage[notref,notcite]{showkeys}
\usepackage{xpatch}
\usepackage{tikz}
\usepackage{adjustbox}
\usepackage{xspace}
\usepackage{enumitem} 
\usepackage{comment}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\bvec}[1]{\mathbf{#1}}

\newcommand{\va}{\bvec{a}}
\newcommand{\vb}{\bvec{b}}
\newcommand{\vc}{\bvec{c}}
\newcommand{\vd}{\bvec{d}}
\newcommand{\ve}{\bvec{e}}
\newcommand{\vf}{\bvec{f}}
\newcommand{\vg}{\bvec{g}}
\newcommand{\vh}{\bvec{h}}
\newcommand{\vi}{\bvec{i}}
\newcommand{\vj}{\bvec{j}}
\newcommand{\vk}{\bvec{k}}
\newcommand{\vl}{\bvec{l}}
\newcommand{\vm}{\bvec{m}}
\newcommand{\vn}{\bvec{n}}
\newcommand{\vo}{\bvec{o}}
\newcommand{\vp}{\bvec{p}}
\newcommand{\vq}{\bvec{q}}
\renewcommand{\vr}{\bvec{r}}
\newcommand{\vs}{\bvec{s}}
\newcommand{\vt}{\bvec{t}}
\newcommand{\vu}{\bvec{u}}
\newcommand{\vv}{\bvec{v}}
\newcommand{\vw}{\bvec{w}}
\newcommand{\vx}{\bvec{x}}
\newcommand{\vy}{\bvec{y}}
\newcommand{\vz}{\bvec{z}}

\newcommand{\vA}{\bvec{A}}
\newcommand{\vB}{\bvec{B}}
\newcommand{\vC}{\bvec{C}}
\newcommand{\vD}{\bvec{D}}
\newcommand{\vE}{\bvec{E}}
\newcommand{\vF}{\bvec{F}}
\newcommand{\vG}{\bvec{G}}
\newcommand{\vH}{\bvec{H}}
\newcommand{\vI}{\bvec{I}}
\newcommand{\vJ}{\bvec{J}}
\newcommand{\vK}{\bvec{K}}
\newcommand{\vL}{\bvec{L}}
\newcommand{\vM}{\bvec{M}}
\newcommand{\vN}{\bvec{N}}
\newcommand{\vO}{\bvec{O}}
\newcommand{\vP}{\bvec{P}}
\newcommand{\vQ}{\bvec{Q}}
\newcommand{\vR}{\bvec{R}}
\newcommand{\vS}{\bvec{S}}
\newcommand{\vT}{\bvec{T}}
\newcommand{\vU}{\bvec{U}}
\newcommand{\vV}{\bvec{V}}
\newcommand{\vW}{\bvec{W}}
\newcommand{\vX}{\bvec{X}}
\newcommand{\vY}{\bvec{Y}}
\newcommand{\vZ}{\bvec{Z}}

\newcommand{\diag}{\operatorname{diag}}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\polylog}{\operatorname{poly}\log}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\Tr}{\operatorname{Tr}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\I}{\mathrm{i}}

\newcommand{\opr}[1]{\ensuremath{\operatorname{#1}}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\gives}{\quad\Rightarrow\quad}

\newcommand{\ud}{\,\mathrm{d}}
\newcommand{\Or}{\mathcal{O}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}

\newtheorem{thm}{\protect\theoremname}
\newtheorem{lem}[thm]{\protect\lemmaname}
\newtheorem{rem}[thm]{\protect\remarkname}
\newtheorem{prop}[thm]{\protect\propositionname}
\newtheorem{cor}[thm]{\protect\corollaryname}
\newtheorem{assumption}[thm]{\protect\assumptionname}
\newtheorem{defn}[thm]{\protect\definitionname}
\newtheorem{notation}[thm]{Notation}
\newtheorem{fact}[thm]{Fact}

\providecommand{\definitionname}{Definition}
\providecommand{\assumptionname}{Assumption}
\providecommand{\corollaryname}{Corollary}
\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\remarkname}{Remark}
\providecommand{\theoremname}{Theorem}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\LL}[1]{\textcolor{blue}{[LL:#1 ]}}
\newcommand{\QZ}[1]{\textcolor{orange}{[QZ:#1 ]}}
\definecolor{purp}{RGB}{160, 32, 240}
\newcommand{\kds}[1]{\textsf{\textcolor{purp}{[KS: #1]}}}
\definecolor{forestgreen}{rgb}{0.13, 0.55, 0.13}
\newcommand{\TS}[1]{\textcolor{forestgreen}{[TS:#1 ]}}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\newcommand{\FF}[1]{\textcolor{airforceblue}{[FF:#1 ]}}
\newcommand{\mz}[1]{\textcolor{cyan}{[MZ:#1 ]}}
\newcommand{\RK}[1]{\textcolor{teal}{[RK:#1 ]}}

%%%%%% BEGIN Extra packages %%%%%%
\usetikzlibrary{quantikz}
\newcommand{\qwb}{\qwbundle{}}
%
%\usepackage{hyperref}

% Tikz to highlight matrix elements
\usetikzlibrary{fit}
\tikzset{%
  highlight/.style={rectangle,rounded corners,fill=blue!15,draw,fill opacity=0.3,thick,inner sep=0pt}
}
\newcommand{\tikzmark}[2]{\tikz[overlay,remember picture,baseline=(#1.base)] \node (#1) {#2};}
%
\newcommand{\Highlight}[1][submatrix]{%
    \tikz[overlay,remember picture]{
    \node[highlight,fit=(left.north west) (right.south east)] (#1) {};}
}

%%%%%% END Extra packages %%%%%%


==> Quantum chemistry TBG/sections/hartree_fock.tex <==
\subsection{Hartree--Fock theory}

The Hartree--Fock approximation is the starting point for various high-accuracy electronic-structure methods~\cite{Helgaker2014}. 
The underlying assumption is that the many-body wavefunction takes the form of a Slater determinant, i.e., 
\begin{equation}
\ket{\Psi_S}=\prod_{\vk}\prod_{i\in\mathrm{occ}} b_{i\vk}^{\dag}\ket{\mathrm{vac}},
\end{equation}
where $\ket{\mathrm{vac}}$ is the vacuum state, and 
\begin{equation}
b_{i\vk}^{\dag}=\sum_{n}f_{n\vk}^{\dag} \Xi_{ni}(\vk)
\end{equation}
defines the creation operator for the Hartree--Fock orbitals for each $\vk\in\Omega^*$.
For integer filling, the number of occupied orbitals per $\vk$ point is $\nu$ (indexed by $\mathrm{occ}$). 
The 1-RDM associated with a given Slater determinant $\ket{\Psi_S}$ is then
\begin{equation}
[P(\vk)]_{nm}=\braket{\Psi_S|\hat{f}_{m\vk}^{\dagger}\hat{f}_{n\vk}|\Psi_S}=
\sum_{i\in\mathrm{occ}} \Xi_{ni}(\vk)\Xi_{mi}^*(\vk).
\end{equation}
Following the standard derivation of Hartree--Fock theory (see e.g.,~\cite{SzaboOstlund1989,MartinReiningCeperley2016}), we begin with the characterization of the Hartree--Fock energy, i.e., 
\begin{equation}
\label{eq:e_hf}
E_{\rm HF}
=
\min_{P\in \mathcal{M}}{\rm Tr}[PH],
\end{equation}
where $\mathcal{M}$ is the set of 1-RDMs associated with the possible single Slater determinants of the system.
A common way to seek the solution to Eq.~\eqref{eq:e_hf} is by finding a stationary point, which is equivalent to diagonalizing the Fock operator~\cite{SzaboOstlund1989}, i.e., 
\begin{equation}
\hat{F}[P]=\hat{H}_0+ \hat{J}[P] - \hat{K}[P]= \hat{H}_0+ \hat{V}_{HF}[P].
\end{equation}
We here employ quantum chemistry notation where $H_0$ is the core Hamiltonian, $\hat{J}[\cdot]$ and $\hat{K}[\cdot]$ are the Coulomb and exchange operator, respectively, and $\hat{V}_{HF}[\cdot]$ is the Hartree--Fock potential.
This non-linear eigenvalue problem is determined by self-consistently evaluating the 1-RDM~\cite{Lehtola2020}.

For an explicit definition of the Coulomb term, we apply Wick's theorem to the interaction term~\eqref{eqn:interaction_simplify}, and use the relation in \cref{eqn:average_f}. 
This yields
%can be obtained using , which replaces $\hat{\rho}_{-\vq}$ by its mean-field %average. Replacing $\hat{\rho}_{\vq}$ by its mean-field average gives an %identical contribution, which cancels the factor $\frac12$ in the interaction %Hamiltonian.
%The Hartree potential is 
% \begin{equation}
% \begin{split}
% \hat{H}_{\mathrm{h}}[P]=&\frac{1}{ |\Omega|} 
% \sum_{\vq} V(\vq)\hat{\rho}_{\vq}\frac{1}{N_{\vk}}\braket{\Psi_S|\hat{\rho}_{-\vq}|\Psi_S}\\
% =&\frac{1}{|\Omega|} 
% \sum_{\vG} V(\vG)\hat{\rho}_{\vG} \left(\frac{1}{N_{\vk}}\sum_{\vk'\in \Omega^*} \Tr[ \Lambda_{\vk'}(-\vG) P(\vk')]\right)\\
% =:&\frac{1}{|\Omega|} 
% \sum_{\vG} V(\vG)\hat{\rho}_{\vG} \varrho(-\vG).
% \end{split}
% \end{equation}
%\kds{I think $\Lambda_{k'}$ needs a transpose above?}

\begin{equation}
\label{eq:Coulomb_op_long}
\begin{split}
\hat{J}[P]=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}
\\
&
\times \left(\braket{\Psi_S|\hat f_{m\vk}^{\dagger}\hat f_{n(\vk+\vq')}|\Psi_S} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq')}+ \braket{\Psi_S|\hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq')}|\Psi_S} \hat f_{m\vk}^{\dagger}\hat f_{n(\vk+\vq')}\right)\\
=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}\\
&
\times \sum_{\vG\in\mathbb{L}^*} \left([P(\vk)]_{nm}\delta_{\vq',-\vG}\hat f_{m'\vk'}^{\dagger} \hat f_{n'\vk'}+[P(\vk')]_{n'm'}\delta_{\vq',\vG}\hat f_{m\vk}^{\dagger}\hat f_{n\vk}\right)\\
=&\frac{1}{|\Omega|} 
\sum_{\vG\in\mathbb{L}^*} V(\vG)\left(\frac{1}{N_{\vk}}\sum_{\vk'\in \Omega^*} \Tr[ \Lambda_{\vk'}(-\vG) P(\vk')]\right)\left(\sum_{\vk\in \Omega^*} \sum_{mn} [\Lambda_{\vk}(\vG)]_{mn}\hat f_{m\vk}^{\dagger}  \hat f_{n\vk}\right).
\end{split}
\end{equation}
In the last step we have used the fact that $V(\vq')=V(-\vq')$. 
To simplify the expression in Eq.~\eqref{eq:Coulomb_op_long}, we can define the electron density $\wt{\rho}$, i.e., 
\begin{equation}
\wt{\rho}[P](\vG)=\frac{1}{N_{\vk}} 
\sum_{\vk'\in \Omega^*}\Tr[ \Lambda_{\vk'}(\vG) P(\vk')],
\end{equation}
which is periodic with respect to the moir\'e unit cell.  
Using the definition of the pseudo-density operator in~\cref{eqn:rho_operator}, the expression of the Coulomb operator can be simplified into the standard density--density form 
\begin{equation}
\hat{J}[P]=\frac{1}{|\Omega|} \sum_{\vG} V(\vG) \wt{\rho}[P](-\vG)\hat{\rho}_{\vG}.
\end{equation}


We proceed similarly for the exchange operator; using Wick's theorem yields
\begin{equation}
\begin{split}
\hat{K}[P]=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}
\\
&
\times\left(\braket{\Psi_S|\hat f_{m\vk}^{\dagger}\hat f_{n'(\vk'-\vq')}|\Psi_S} \hat f_{m'\vk'}^{\dagger}\hat f_{n(\vk+\vq')} + \braket{\Psi_S|\hat f_{m'\vk'}^{\dagger}\hat f_{n(\vk+\vq')}|\Psi_S} \hat f_{m\vk}^{\dagger}\hat f_{n'(\vk'-\vq')}\right)\\
=&
\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}\\
&
\times \sum_{\vG\in\mathbb{L}^*} \left([P(\vk)]_{n'm}\delta_{\vk,\vk'-\vq'+\vG}
\hat f_{m'\vk'}^{\dagger}\hat f_{n(\vk+\vq')}+[P(\vk')]_{nm'}\delta_{\vk',\vk+\vq'+\vG}
\hat f_{n'(\vk'-\vq')}\right)\\
=&
\frac{1}{ |\Omega| N_{\vk}} \sum_{\vq'}\sum_{\vk\in \Omega^*}
\sum_{mm'nn'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [P(\vk+\vq')]_{nm'}[\Lambda_{\vk+\vq'}(-\vq')]_{m'n'}
\hat f_{m\vk}^{\dagger}\hat f_{n'\vk}. 
\end{split}
\end{equation}
In summary, the Hartree--Fock potential can be written as
\begin{equation}
\hat{V}_{\mathrm{HF}}[P]
=\hat{J}[P]- \hat{K}[P]
=\sum_{\vk\in \Omega^*} \hat f_{m\vk}^{\dagger}[v_{\mathrm{hf}}[P](\vk)]_{mn}
\hat f_{n\vk},
\end{equation}
where
\begin{equation}
\label{eq:hf-rho}
\begin{split}
[v_{\mathrm{hf}}[P](\vk)]_{mn}=&\frac{1}{|\Omega|} 
\sum_{\vG\in\mathbb{L}^*} V(\vG) \left(\frac{1}{N_{\vk}}\sum_{\vk'\in \Omega^*} \Tr[ \Lambda_{\vk'}(-\vG) P(\vk')]\right)[\Lambda_{\vk}(\vG)]_{mn}\\
&-\frac{1}{ |\Omega| N_{\vk}} \sum_{\vq'} \sum_{m'n'}
 V(\vq') [\Lambda_{\vk}(\vq')]_{mn'} [P(\vk+\vq')]_{n'm'}[\Lambda_{\vk+\vq'}(-\vq')]_{m'n}.
\end{split}
\end{equation}

% 
% Note that BM bands are different from HF bands here. $\hat{f}^{\dagger}_{n\vk}$ represents the creation operator corresponding to the BM band basis $u_{n\vk}=\hat{f}^{\dagger}_{n\vk}\ket{0}$, where $u_{n\vk}$ is an eigenfunction of the first quantized single-particle Hamiltonian $h(\textbf{k})$ with the eigenvalue $\epsilon_{n\textbf{k}}$. In Section \ref{sec:symm}, the projected Hamiltonian will be discussed and we will perform the change of basis on the creation/annihilation operators:
% \[
% \hat{\vf}^{\dag}_{m\vk} \to \sum_{n} [U(\vk)]_{mn} \hat{\vf}^{\dag}_{n\vk}.
% \]
% 
% On the other hand, $\ket{\Psi}$ represents the many-body wavefunction, which is a Slater determinant constructed from HF bands. In general, BM band basis is used to project the IBM Hamiltonian onto flat bands and it's generated from BM Hamiltonian, while HF solution is tested to see the spontaneous symmetry-broken and it's the ground state of IBM Hamiltonian.



\subsection{Subtraction Hamiltonian}\label{sec:subtraction}
 
%In order to observe the spontaneous symmetry breaking, we need to discuss the existence of symmetries in IBM model. Before the symmetry checking in Section~\ref{sec:symm}, we introduce 

%Using the Hartree--Fock potential, we can define the subtraction Hamiltonian in the quadratic part of the IBM model in \cref{eqn:ibm_quadratic}. 
Since the BM band energies already take the electron--electron interaction between the two layers of graphene into account, the double gate-screened Coulomb potential in the IBM model double counts said interactions.
As a remedy, Bultinck et al~\cite{BultinckKhalafLiuEtAl2020} have introduced $v_{\mathrm{hf}}[P^0](\vk)$, see Eq.~\cref{eq:hf-rho}, for a given reference density $P^0$ as the subtraction Hamiltonian $h_{\mathrm{sub}}(\vk)$.
Combining \cref{eqn:IBM_Ham,eqn:ibm_quadratic}, the IBM model is well-defined.
In particular, since the mapping $P \mapsto v_{\mathrm{hf}}[P]$ is linear, the Hartree--Fock Hamiltonian can be written as

% In \cite{BultinckKhalafLiuEtAl2020}, a subtraction Hamiltonian $h_{\mathrm{sub}}(\vk)$ is introduced to cancel out such effects at the Hartree--Fock level, defined as the Hartree--Fock potential \cref{eq:hf-rho} with respect to a reference density $P^0$, i.e., $h_{\mathrm{sub}}(\vk)=h_{\mathrm{hf}}[P_0](\vk)$. 
% Combining \cref{eqn:IBM_Ham,eqn:ibm_quadratic}, the IBM model is well defined. In particular, since the mapping $P \mapsto v_{\mathrm{hf}}[P]$ is linear, the Hartree--Fock Hamiltonian can be written as
\begin{equation}
\label{eqn:subtracted_HF}
\sum_{\vk\in\rm{mBZ}}\sum_{mn}\hat f^{\dagger}_{m\vk}[h_{\mathrm{BM}}(\vk)]_{mn}
\hat f_{n\vk} + \hat{V}_{\mathrm{HF}}[\delta P(\vk)],
\end{equation}
where $\delta P(\vk)=P(\vk)-P^{0}(\vk)$.



%\LL{ the following sentence should appear in the symmetry section?} Several special choices are discussed here to enforce different symmetries, such as particle-hole symmetry $\mc{P}$. 


% Given the reference density $P^0$, the quadratic subtraction Hamiltonian is defined as the Hartree--Fock potential  and
% 
% \begin{equation}
% \label{eqn:subtraction}
% \begin{split}
% h^0_s[P^0](\vk)= \frac{1}{|\Omega|N_{\vk}} 
% [&\sum_{\vG} V(\vG)\Lambda_{\vk}(G) \sum_{\vk'} \Tr[ \Lambda_{\vk'}(-\vG) P^0(\vk')] \\
% &-\sum_{\vG,\vq}V(\vG+\vq)\Lambda_{\vk}(\vq) P^0(\vk+\vq)\Lambda_{\vk+\vq}(-\vq)].
% \end{split}
% \end{equation}

% The single-particle Hamiltonian is then changed into $h(\vk)-h_s^0[P^0](\vk)$ and the corresponding Hartree--Fock Hamiltonian is
% \begin{equation}
% \begin{split}
% \label{eqn:subtracted_HF}
% \hat H_{HF}=&\sum_{\vk\in\rm{mBZ}}\hat f^{\dagger}_{\vk}[h(\vk)-h_s^0[P^0](\vk)]\hat f_{\vk} + \hat{H}_{\mathrm{h}}[P(\vk)]+\hat{H}_{\mathrm{f}}[P(\vk)],\\
% =&\sum_{\vk\in\rm{mBZ}}\hat f^{\dagger}_{\vk}h_s(\vk)\hat f_{\vk} + \hat{H}_{\mathrm{h}}[\delta P(\vk)]+\hat{H}_{\mathrm{f}}[\delta P(\vk)],
% \end{split}
% \end{equation}
% where $\delta P(\vk)=P(\vk)-\frac12I$, $\delta P^0(\vk)=P^0(\vk)-\frac12I$ and $h_s(\vk)=h(\vk)-h_s^0[\delta P^0](\vk)$. We further assume that $P^0(\vk)$ is a neutral projector arising from a $C_{2z}\mc{T}$ symmetric
% Hamiltonian, then the first term in \cref{eqn:subtraction} vanished for half-filling system (see Appendix~\ref{sec:supp}) and the subtracted single-particle Hamiltonian is
% \begin{equation}
% h_s(\vk)=h(\vk)+\frac{1}{|\Omega|N_{\vk}}\sum_{\vG,\vq}V(\vG+\vq)\Lambda_{\vk}(\vq) \delta P^0(\vk+\vq)\Lambda_{\vk+\vq}(-\vq).
% \end{equation}

Following \cref{eqn:1rdm}, $P^0(\vk)$ should be interpreted as the coefficients of the reference density matrix in the BM band basis.
The choice of a reference density matrix $P^0(\vk)$ is not unique and should also be viewed as part of the IBM model.
For instance, in Ref.~\cite{BernevigSongRegnaultEtAl2021}, the choice is $P^0(\vk)=\frac{1}{2}I$, which is called the \textit{average scheme}. 
In Ref.~\cite{BultinckKhalafLiuEtAl2020},\LL{ Mike/Tomo: cite the relevant papers from MacDonald's group?}  $P^0(\vk)$ is obtained by projecting the zero temperature limit of the density matrix corresponding to two decoupled graphene layers to the BM band basis of the TBG system. This is referred to as the \textit{decoupled scheme}. 
It is worth mentioning that in the decoupled scheme, the number of BM bands should be sufficiently large to preserve the trace of $P^0$ after the projection. The zero temperature limit ensures that $P^0$ is uniquely defined even if some of the band energies of the two decoupled graphene layers may become degenerate. Furthermore, the choice of $P^0$ does not change with respect to the filling factor $\nu$. \LL{ Mike/Tomo: can you add justification for the usage of exactly the same subtraction density matrix for non-integer fillings?}
Unless otherwise specified, we adopt the decoupled scheme in all the numerical results.
 


% In our implementation, without further notice, average scheme is used since it gives rise to the particle-hole symmetry $\mc{P}$ in the interaction term\cite{TBGIII}, preserves both $C_{2z}\mc{T}$ and $C_{3z}$ symmetry of our interests. The numerical difference between different schemes will also be discussed in \ref{sec:numerical}. 


==> Quantum chemistry TBG/sections/ibm_model.tex <==

\begin{figure*}
\begin{center}
\begin{subfigure}[c]{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/tbg_layers.pdf} 
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/mbz_num_lat.pdf} 
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/flat_bands.png}
\end{subfigure}
\begin{subfigure}[c]{.3\textwidth}
    \caption{}
    \label{fig:tbg_layers}
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \caption{}
    \label{fig:mbz_num_lattice}
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \caption{}
    \label{fig:flat_bands}
\end{subfigure}
\end{center}
\caption{
\FF{Note the hack! I did not know how to vertically align the figure and have the captions (a), (b), (c) at the bottom. Format fine tuning has to be done at some point.}
(\subref{fig:tbg_layers}) The graphic shows two monolayer graphene Brillouin zones (BZ) in red and blue, respectively, aligned by their $\Gamma$-point and twisted by an angle $\Theta$. 
The Dirac points of the individual layers are denoted by $K^+$ and $K^-$ for the red and blue BZ, respectively. 
Moreover, the graphic shows the corresponding moir\'e Brillouin zone of the twisted bilayer graphene shaded in grey and the $\Gamma$-point of the mBZ denoted $\Gamma_{\rm mBZ}$. 
(\subref{fig:mbz_num_lattice}) The graphic shows three mBZ. Furthermore, it shows the numerical $k$ grid encircle by the green dashed line. 
This rectangular choice of the mBZ $k$ grid follows the grid in Ref.~\cite{SoejimaParkerBultinckEtAl2020}
The Dirac points of the individual graphene layers $K^+$ and $K^-$ red and blue, respectively, are included as reference. 
(\subref{fig:flat_bands}) The graphic shows the band structure of the BM Hamiltonian in the mBZ, with the corresponding flat bands (red lines) and remote bands (grey lines). The interacting BM Hamiltonian is then projected onto the two flat band space (note that the labels should not touch the graphs).
\FF{Graphic (c) needs to be improved}
\LL{ I agree. A few more minor changes: 1) the fonts should be larger and lines should be thicker. 2) Not sure what the two vectors are for in the middle figure (we never used $Q_1,Q_2$. We should also say that the rectangular choice of the mBZ follows that in \cite{SoejimaParkerBultinckEtAl2020}. 3) The $\Gamma$ point in the rightmost figure should be $\Gamma_M$?}
}
\end{figure*}

% \begin{figure*}
% \centering
% \begin{subfigure}[b]{.74\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/mBZ.png} % KDS: The size of the subfigure is set to .74\textwidth above, \linewidth takes this change into account which is why it's \linewidth not .74\linewidth. 
%     \caption{}
%     \label{fig:mbz-picture}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/flat_bands.png}
%     \caption{}
%     \label{fig:flat_bands}
% \end{subfigure}
% \caption{(\subref{fig:mbz-picture}) Two monolayer graphene Brillouin zones twisted by an angle $\theta$ and the corresponding Moir\'e Brillouin zone of the twisted bilayer graphene. Zoomed view of the Moir\'e BZ shows the numerical $k$ grids using green dash. (\subref{fig:flat_bands}) The band structure of the BM Hamiltonian in the Moir\'e BZ, with the corresponding flat bands (red lines) and remote bands (grey lines). The interacting BM Hamiltonian is then projected onto the flat band space. \kds{Not an immediate issue but the y label in (b) is cut off}
% \FF{Maybe use three Figures (a), (b), and (c) to make this cleaner? What about a slight rephrasing: (a) The graphic shows two monolayer graphene Brillouin zones (in red and blue, respectively) aligned by their $\Gamma$-point and twisted by an angle $\theta$ ($\Theta$ should be larger in the Figure). The Dirac points of the individual layers are denoted by $K^+$ and $K^-$ for the red and blue BZ, respectively. Moreover, the graphic shows the corresponding Moir\'e Brillouin zone (mBZ) of the twisted bilayer graphene and the $\Gamma$-point of the mBZ ($\Gamma_M$). (b) The graphic shows three mBZ and the mBZ lattice vectors. Furthermore, it shows the numerical $k$ grid encircle by the green dashed line. (c) The graphic shows the band structure of the BM Hamiltonian in the mBZ, with the corresponding flat bands (red lines) and remote bands (grey lines). The interacting BM Hamiltonian is then projected onto the two flat band space (note that the labels should not touch the graphs).}\LL{ I agree. A few more minor changes: 1) the fonts should be larger and lines should be thicker. 2) Not sure what the two vectors are for in the middle figure (we never used $Q_1,Q_2$. We should also say that the rectangular choice of the mBZ follows that in \cite{SoejimaParkerBultinckEtAl2020}. 3) The $\Gamma$ point in the rightmost figure should be $\Gamma_M$?}
% }
% %\QZ{ somehow subcaption package doesn't work}}
% \end{figure*}



% 
% 
% 
% We first present a review of the monolayer and bilayer graphene to define our notations. Single layer graphene is a 2D structure with honeycomb lattice and it consists of a bipartite lattice of two triangular sublattices $\sigma=A/B$. Single layer graphene also has two Dirac points $\pm K$ in the single layer Brillouin zone and these two Dirac points are connected by the time-reversal symmetry. This two Dirac points are labelled with valley index $\pm1$ and equipped with the valley operator $\tau$. Then the twisted bilayer grapehene has two layers of graphene twisted by a small angle $\theta$ and this two layers are perfectly stacked with each other at one $AA$ lattice. When the twisted angle is small, each layer $l=\pm$ has two Dirac points $\pm K_{l}$ and the valley in the top layer is only coupled with the same valley in the bottom layer with a Moir\'e interlayer potential. The hopping parameters $w_0$ and $w_1$ represent the $AA$ hopping and $AB/BA$ hopping respectively. The original BM model has equal $AA$ and $AB/BA$ hopping with $w_0=w_1$. At the chiral limit $w_0=0$, $AA$ hopping is turned off and it gives us the exact zero flat bands.\cite{nam_2017}
% The special geometry and rich symmetries of graphene enable the unique band structure and interesting electronic phenomenon. In particular, there exist isolated flat bands in the BM band structure. Using these flat bands, we will introduce the projected IBM Hamiltonian with a double-gate screened Coulomb interaction. 

Unless otherwise specified, we restrict to the flat bands labeled by $n\in\{1,2\}$ \kds{I don't think choosing $n \in \{ 1,2 \}$ really makes sense here; we haven't defined what the band indexing is}\LL{ We talked about that (briefly) in the previous section? Please feel free to change.}  whose band energies are separated from the remaining band spectrum, as in Figure~\ref{fig:flat_bands}.
Throughout the discussion below, the band indices $m,n$ refer to the flat bands only. 
The Hamiltonian of the IBM model for the flat bands takes the form
\begin{equation}
\begin{split}
\hat{H}_{\mathrm{IBM}}
=& \hat{H}_0+\hat{H}_I\\
=&\sum_{\vk\in \Omega^*} \sum_{mn}\hat f_{m\vk}^{\dagger} [h(\vk)]_{mn} \hat f_{n\vk}\\
&+\frac{1}{2}
\sum_{\substack{\vk,\vk',\vk''\in \Omega^*\\\vk''' = \vk+\vk'-\vk''}} \sum_{mm'nn'}\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}\hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'\vk'''} \hat f_{n\vk''},
\end{split}
\label{eqn:IBM_Ham}
\end{equation}
%\kds{It looks a bit gross, but I added the crystal momentum conservation condition on $\vk'''$ in the sum above. At least for me, this significantly clarifies the discussion below}
where $\hat{H}_0$ and $\hat{H}_I$ are the quadratic term and the quartic term, respectively. 
The ground state of the IBM model is then defined as the solution to the eigenvalue problem
\begin{equation}
E_0=\min_{\substack{\ket{\Psi}\in\mc{F}, ~\braket{\Psi|\Psi}=1\\\braket{\Psi|\hat{N}|\Psi}=N_e}} \quad \braket{\Psi|\hat{H}|\Psi},
\end{equation}
where $N_e=\nu N_{\vk}$ is the total number of electrons, and $\hat{N}=\sum_{\vk}\sum_{n} \hat f_{n\vk}^{\dagger} \hat f_{n\vk}$ is the total number operator.
The number of electrons per $\vk$ point is denoted by $\nu$, called the \textit{filling factor}. 
Since there are only two bands per $\vk$ point, the only non-trivial integer value for the filling factor is $\nu=1$, which is called the half-filling case (or the particle-hole symmetric case) of the IBM model in the spin-less, valley-less regime.

The main object of interest in this work is the one-particle reduced density matrix (1-RDM) corresponding to the ground state $\ket{\Psi}$ defined as
\begin{equation}
\label{eqn:1rdm}
[P(\vk)]_{nm}=\braket{\Psi|\hat{f}_{m\vk}^{\dagger}\hat{f}_{n\vk}|\Psi}.
\end{equation}
We emphasize that the 1-RDM is well-defined in the entire moir\'e reciprocal space due to the periodic extension in \cref{eqn:period_f}.
Using the 1-RDM, we find that for any $\vk,\vk'$ in the moir\'e reciprocal space,
\begin{equation}
\braket{\Psi|\hat{f}_{m\vk}^{\dagger}\hat{f}_{n\vk'}|\Psi}
=P(\vk)\sum_{\vG\in\mathbb{L}^*}\delta_{\vk,\vk'+\vG}.
\label{eqn:average_f}
\end{equation}

The quartic term $\hat{H}_I$ describes the (screened) Coulomb interaction via the two electron repulsion integrals (ERI) denoted by $\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}$.
The coefficients of the quadratic term can be written as
\begin{equation}
h(\vk)=h_{\mathrm{BM}}(\vk)-h_{\mathrm{sub}}(\vk),
\label{eqn:ibm_quadratic}
\end{equation}
where $[h_{\mathrm{BM}}(\vk)]_{mn}=\varepsilon^{\mathrm{BM}}_n(\vk) \delta_{mn}$ is given by the BM band energy. The second term $h_{\mathrm{sub}}(\vk)$ is called the subtraction Hamiltonian, which removes the double counting of the Coulomb interaction within the flat bands, and is defined in terms of the Hartree--Fock potential. We focus on the Coulomb interaction term first and postpone the discussion of $h_{\mathrm{sub}}(\vk)$ to \cref{sec:subtraction}.

In the Coulomb interaction term, the summation is only over $\vk,\vk',\vk''\in\Omega^*$. This is due to the crystal momentum conservation, i.e., $\vk+\vk'-\vk''-\vk'''=\bm{0}$.
Here we follow the convention that the fourth momentum vector $\vk'''=\vk+\vk'-\vk''$ may be outside $\Omega^*$
\footnote{Many practical implementation restrict $\vk'''$ to be within the mBZ as well, and hence the crystal momentum conservation condition becomes $\vk+\vk'-\vk''-\vk'''=\vG$ for some $\vG\in\mathbb{L^*}$. We do not use this convention in this paper.}.
Another way to express the crystal momentum conservation condition is to write $\vk''=\vk+\vq$, $\vk'''=\vk'-\vq$. 
Note that in this convention, both $\vq$ and $\vk'''$ may be outside the mBZ.


In TBG, the flat bands not only interact via a screened Coulomb interaction (the screening is modeled by a dielectric constant $\epsilon$), but also feels the Coulomb screening from the top and bottom metallic gates.\FF{This is a weird phrase.}
\LL{ Mike/Tomo: what is a good reference to cite a picture for this double-gate setup for TBG?} Assume that the TBG sample is placed in a $x$\nobreakdash-$y$~plane that is of distance $d/2$ to the top and bottom metallic gate plates along the $z$ direction. 
Since the moir\'e length scale is much larger than the distance between the sublattice sites and the layers, we may assume that the Coulomb interaction depends only on the difference $\delta r= \vr-\vr'$, and does not depend on the sublattice and layer indices. 
The screened Coulomb interaction in the real space (called a double gate-screened Coulomb potential) can be written as
\begin{equation}
V(\vr)=U_{d} \sum_{n=-\infty}^{\infty} \frac{(-1)^{n}}{\sqrt{\abs{\vr}^2+(nd)^{2}}}.
\end{equation}
%Here $U_d=\frac{e^2}{4\pi\epsilon_0 \epsilon}$ is the interaction strength.
Here, $U_d=\epsilon^{-1}$ describes the strength of the screened Coulomb interaction. In the Fourier space, the Coulomb interaction takes the form
\begin{equation}
V(\vq)=\int V(\vr) e^{-\I \vq \cdot \vr}\ud \vr=2\pi U_d\frac{\tanh(\abs{\vq}d/2)}{\abs{\vq}},
\label{eqn:doublegate_q}
\end{equation}
see \cite[Appendix C]{BernevigSongRegnaultEtAl2021} for more details.
Note that under slight abuse of notation we here use $V(\vq)$ to denote the Fourier transform of $V(\vr)$).

The ERI take the form
\begin{equation}
\begin{split}
&\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}\\
\qquad&=\frac{1}{N_{\vk}^2}\sum_{\sigma,l,\sigma',l'}\int V(\vr-\vr')\psi^{*}_{m\vk}(\vr,\sigma,l)
\psi^{*}_{m'\vk'}(\vr,\sigma',l')\psi_{n\vk''}(\vr,\sigma,l)
\psi_{n'\vk'''}(\vr,\sigma',l') \ud \vr \ud \vr'\\
\qquad&=\frac{1}{N_{\vk}^2}
\,\int V(\vr-\vr') e^{\I \vq\cdot (\vr-\vr')}\varrho_{m\vk,n(\vk+\vq)}(\vr) \varrho_{m'\vk',n'(\vk'-\vq)}(\vr')\ud \vr \ud \vr',
\end{split}
\label{eqn:eri_realspace}
\end{equation}
Note that the integration is performed in the moir\'e supercell.
The pair product of the periodic components of the BM bands in the real space (summed over the sublattice and layer indices) is defined as
\begin{equation}
\varrho_{m\vk,n\vk''}(\vr)
=\sum_{\sigma,l}u^*_{m\vk}(\vr,\sigma,l)  u_{n\vk''}(\vr,\sigma,l).
\end{equation}
Expanding the periodic Bloch functions in terms of their Fourier coefficients, the pair product can be written as
\begin{equation}
\label{eq:pair-product}
    \varrho_{m\vk,n\vk''}(\vr) = \frac{1}{|\Omega|^2} \sum_{\vG, \vG' \in \mathbb{L}^*} \sum_{\sigma,l}u^*_{m\vk}(\vG,\sigma,l)  u_{n\vk''}(\vG',\sigma,l) e^{i (\vG' - \vG) \cdot r}.
\end{equation}
Recall that by definition of the periodic Bloch functions $\psi_{n\vk''}(\vr) = \psi_{n,(\vk'' + \vG)}(\vr)$ for all $\vG \in \mathbb{L}^*$.
Therefore, $u_{n\vk''}(\vr) = e^{i \vG \cdot \vr} u_{n,(\vk''+\vG)}(\vr)$ and consequently, 
% Observe that since for all $\vG \in \mathbb{L}^*$, $\psi_{n\vk''}(\vr) = \psi_{n,(\vk'' + \vG)}(\vr)$ by the definition of the periodic Bloch functions it is also true that $u_{n\vk''}(\vr) = e^{i \vG \cdot \vr} u_{n,(\vk''+\vG)}(\vr)$. 
% As a consequence of this 
\begin{equation}
\begin{split}
    & u_{n\vk''}(\vr) = e^{i \vG \cdot \vr} u_{n,(\vk''+\vG)}(\vr) \\[1ex]
    & \Rightarrow \sum_{\vG'} u_{n\vk''}(\vG') e^{i \vG' \cdot \vr} =  \sum_{\vG'} u_{n,(\vk''+\vG)}(\vG') e^{i (\vG' + \vG) \cdot \vr} \\[1ex]
    & \Rightarrow u_{n\vk''}(\vG') = u_{n,(\vk''+\vG)}(\vG' - \vG).
\end{split}
\end{equation}
Hence, 
\begin{equation}
    \varrho_{m\vk,n\vk''}(\vr) = \frac{1}{|\Omega|^2} \sum_{\vG, \vG' \in \mathbb{L}^*} \sum_{\sigma,l}u^*_{m\vk}(\vG,\sigma,l)  u_{n,\vk''+\vG}(\vG' - \vG,\sigma,l) e^{i (\vG' - \vG) \cdot r}.
\end{equation}
The Fourier coefficients of the pair product then satisfy
\begin{equation}
\varrho_{m \vk,n(\vk+\vq)}(\vG)=\frac{1}{\abs{\Omega}}
\sum_{\vG'\in\mathbb{L}^*} \sum_{\sigma,l}u^*_{m\vk}(\vG',\sigma,l) u_{n(\vk+\vq+\vG)}(\vG',\sigma,l)=[\Lambda_{\vk}(\vq+\vG)]_{mn},
\label{eqn:form_factor}
\end{equation}
where the matrix $\Lambda_{\vk}(\vq+\vG)$ is called the \textit{form factor}.
Note that due to a shift in $\vG$, the Fourier coefficients of the pair product can be written as an inner product opposed to the convolution that arises directly from Eq.~\eqref{eq:pair-product}.

From \cref{eqn:form_factor} we can verify that the form factor satisfies the symmetry condition
\begin{equation}
[\Lambda_{\vk}(\vq+\vG)]^*_{mn}=[\Lambda_{\vk+\vq}(-\vq-\vG)]_{nm}.
\label{eqn:form_factor_symmetry}
\end{equation}

Using the definitions of the Coulomb interaction $V(\vq)$ in Eq.~\ref{eqn:doublegate_q} and the form factor in Eq.~\eqref{eqn:form_factor}, the ERI can be expressed in the Fourier space as
\begin{equation}
\begin{split}
\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}=&\frac{1}{|\Omega| N_{\vk}} \sum_{\vG\in \mathbb{L}^*} V(\vq+\vG) \varrho_{m\vk,n(\vk+\vq)}(\vG)
\varrho_{m'\vk',n'(\vk'-\vq)}(-\vG)\\
=&\frac{1}{|\Omega| N_{\vk}} \sum_{\vG\in \mathbb{L}^*} V(\vq+\vG)  [\Lambda_{\vk}(\vq+\vG)]_{mn} [\Lambda_{\vk'}(-\vq-\vG)]_{m'n'}.
\end{split}
\label{eqn:IBM_ERI}
\end{equation}
Compared to \cref{eqn:eri_realspace}, we gained an extra factor $N_\vk$ due to the integration in the moir\'e supercell.
Hence, the interaction Hamiltonian is fully determined by the form factor and the screened Coulomb potential as
\begin{equation}
\begin{split}
\hat{H}_I=&\frac{1}{2} 
\sum_{\vk,\vk',\vk''\in \Omega^*}\sum_{mm'nn'}\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}\hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'\vk'''} \hat f_{n\vk''}\\
=& \frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk',\vk+\vq=\vk''\in  \Omega^*}\sum_{mm'nn'}
\sum_{\vG\in \mathbb{L}^*} V(\vq+\vG) \braket{u_{m\vk}|u_{n(\vk+\vq+\vG)}}\\
&
\times\braket{u_{m'\vk'}|u_{n'(\vk'-\vq-\vG)}} \hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq)} \hat f_{n(\vk+\vq)}\\
=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk',\vk+\vq=\vk''\in \Omega^*}\sum_{mm'nn'}
\sum_{\vG\in \mathbb{L}^*} V(\vq+\vG) [\Lambda_{\vk}(\vq+\vG)]_{mn}
\\
&
\times[\Lambda_{\vk'}(-\vq-\vG)]_{m'n'} \hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq)} \hat f_{n(\vk+\vq)}.
\end{split}
\label{eqn:interaction_comput}
\end{equation}
This can be further simplified by treating $\vq+\vG$ as a new variable $\vq'$, which takes the value from the entire reciprocal space.
Using \cref{eqn:period_f}, we have
\begin{equation}
\begin{split}
\hat{H}_I=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn}
\\
&
\times [\Lambda_{\vk'}(-\vq')]_{m'n'} \hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq')} \hat f_{n(\vk+\vq')}.
\end{split}
\end{equation} 
Defining a pseudo density operator
\begin{equation}
\hat{\rho}_{\vq}=\sum_{\vk\in \Omega^*} \sum_{mn} \hat f_{m\vk}^{\dagger} [\Lambda_{\vk}(\vq)]_{mn} \hat f_{n(\vk+\vq)},
\label{eqn:rho_operator}
\end{equation}
and using the normal ordering, i.e.,
\begin{equation}
:f_{m\vk}^{\dagger}  \hat f_{n(\vk+\vq)}f_{m'\vk'}^{\dagger}  \hat f_{n'(\vk'-\vq)}:\,
=f_{m\vk}^{\dagger}  f_{m'\vk'}^{\dagger}  \hat f_{n'(\vk'-\vq)}\hat f_{n(\vk+\vq)},
\end{equation}
we can further simplify $\hat{H}_I$ to 
\begin{equation}
\hat{H}_I=\frac{1}{2 \abs{\Omega}N_{\vk}} 
\sum_{\vq'} V(\vq'):\hat{\rho}_{\vq'}\hat{\rho}_{-\vq'}:.
\label{eqn:interaction_simplify}
\end{equation}
This form is reminiscent of the density--density Coulomb interaction in the reciprocal space. 
% \kds{Maybe bring this simplification up later? (in the symmetries section when we use it as part of the calculation?) I think keeping in this way will make it easier for people to compare to previous works} \LL{ Where do you think this should appear?} \kds{This formulation is better for the derviation of the HF theory so I think this is the right place to put it.}
The expression \eqref{eqn:interaction_simplify} has certain conceptual advantages, e.g., when writing down the Hartree--Fock potential, and to verify the symmetries of $\hat{H}_I$ in \cref{sec:symm_ham}. However, it does not simplify the implementation efforts compared to \cref{eqn:interaction_comput}.


==> Quantum chemistry TBG/sections/introduction.tex <==
\QZ{I am open to any advice in the introduction section.}\\
\FF{Maybe add a more general section introducing TBG here.}

The symmetry-breaking insulating phase is crucial in the superconductors\FF{This seems very general, and I am not sure if this is true. Maybe you can add a reference where this is stated?}, such as twisted bilayer graphene (TBG). At the first magic angles, twisted bilayer graphene has the extreme flat band structure, which gives rise to strongly-correlated interaction states and the corresponding superconductivity at charge neutrality.\cite{cao_2018,cao2_2018,lu_2019,yankowitz_2019} 
\FF{Maybe one can rephrase a bit like:
At the first magic angles, TBG exhibits a surprisingly flat band structure that gives rise to strongly-correlated interaction states and the experimentally observed superconductivity~\cite{cao_2018,cao2_2018,lu_2019,yankowitz_2019}.
}
On one hand, the isolation and degeneracy of the Moir\'e flat bands enable the implementation of the mean field method in the band space without breaking the symmetries.\cite{TBGIII,bultinck_2020,soejima_2020,TBGII} On the other hand, many recent work has suggested that strong correlations lead to symmetry breaking within the degenerate flat-band subspace.\cite{girvin_1999,kwan_2021,wang_2016} This spontaneous symmetry-breaking phase is close to a variety of novel phenomenon, such as superconductivity.


Many recent experiments have shown that the correlated insulating phases are well captured by a single $k$-space Slater determinant and Hartree-Fock approximation gives remarkably accurate ground state energy, up to the second perturbation theory.\cite{bultinck_2020}\cite{soejima_2020} The miniband structures and related symmetries of twisted bilayer graphene is close related to this level of accuracy. Many\cite{TBGIII}\cite{bultinck_2020} explained it using an enlarged $U(4)\times U(4)$ symmetry at the chiral limit $w_0=0$, derived the explicit form of the interacting Hamiltonian and proved Slater determinant can be the exact correlated states. Even away from the chiral limit, Hartree-Fock approximation is still remarkably accurate. The combination of two-fold rotation symmetry $C_{2z}$ and time-revesal symmetry  $\mc{T}$ in TBG keep the valley unchanged. The existence of such $C_{2z}\mc{T}$ symmetry in each valley doubles the degeneracy of the low energy bands. With the particle-hole symmetry $\mc{P}$ and chiral symmetry $\mc{S}$, it gives us a clear depiction of the band structures. 


The observations of superconductivity in twisted bilayer graphene has driven people to understand and explain its origin.\cite{girvin_1999}\cite{wang_2016} The flat bands are fragile topology protected by $C_{2z}\mc{T}$ symmetry, but several experiments have found a $C_{2z}\mc{T}$-breaking insulator at charge neutrality.\cite{chatterjee_2020}\cite{das_2021}\cite{liu_2021}\cite{saito_2021} and other symmetry-breaking insulators\cite{jiang_2019}\cite{liu_2021}\cite{wu_2020}. Some\cite{po_2018} has shown that the mean-field treatment necessarily breaks valley and other symmetries to remove the symmetry-enforced band interaction, but the origins are still under debate. In our experiments, we mainly observe two symmetry-breaking states: a) a $C_{2z}\mc{T}$-breaking insulater; b) a three-fold rotation symmetry $C_{3z}$-breaking nematic semimetal. A clear transition between two states is observed for different interlayer Moir\'e potential parameters $w_0/w_1$. 


In this work, we implement a ``careful'' Hartree-Fock approximation and discuss all the possible symmetry-breaking in the implementation. It gives us the ability to detect the spontaneous symmetry-breaking in the twisted bilayer graphene. Then we introduce a new order parameter $\mc{C}_{\vk}$, which can be used to measure the symmetry breaking for any given basis and unitary/antiunitary operators. Using this order parameter, a clear phase transition between quantum anomalous Hall (QAH) state and nematic semimetallic (SM) state is observed by detecting the $C_{2z}\mc{T}/C_{3z}$ symmetry breaking.


\section{Preliminaries}


The tight binding models for monolayer graphene, bilayer graphene, and the Bistritzer--Macdonald (BM) model for the twisted bilayer graphene have been extensively studied in the literature. 
We therefore only provide a minimal introduction to the BM model and the wavefunctions involved; we refer the reader to e.g.~\cite{BultinckKhalafLiuEtAl2020,BernevigSongRegnaultEtAl2021} and the references therein for a more detailed discussion.
Throughout the paper, we adopt atomic units, except for energies which are reported electron volt.

%The BM wavefunction defined in the moir\'e Brillouin zone (mBZ) has the same structure of a wavefunction defined by a non-interacting Hamiltonian with a periodic potential, except that the wavefunction carries additional indices, such as sublattice, layer, valley, and spin.
Subsequently, we denote the moir\'e unit cell by $\Omega$, its area by $|\Omega|$, and the moir\'e Bravais lattice by $\mathbb{L}$. 
Correspondingly, we denote the moir\'e reciprocal lattice $\mathbb{L}^*$, the mBZ by $\Omega^*$. 
The latter is discretized using a Monkhorst--Pack (MP) grid~\cite{MonkhorstPack1976} of size $N_{\vk}=N_{k_x}\cdot N_{k_y}$.
When the MP grid includes the $\Gamma$-point of the mBZ, the computation can be identified with a moir\'e supercell consisting of $N_{\vk}$ unit cells, and $N_{\vk}\abs{\Omega}$ is called the sample area. 
A given BM wavefunction, i.e., a BM band, can be labeled by a tuple $(n,\vk,\vG,\sigma,l,s,\tau)$, where $n$ is the band index, $\vk\in \mathrm{mBZ}$ is the $\vk$-point index, $\vG\in \mathbb{L}^*$ is the planewave index (also called the shell index),  $\sigma\in\{A=1,B=-1\}$ is the sublattice index, $l\in\{t=1,b=2\}$ is the layer index, $s\in\{\uparrow,\downarrow\}$ is the spin index, and $\tau\in\{\vK,\vK'\}$ is the valley index. 
For simplicity, we follow the assumptions in Ref.~\cite{SoejimaParkerBultinckEtAl2020}, and assume that the system is fully polarized along the spin and valley directions.
This is equivalent to dropping the indices $s,$ $\tau$ and assuming that the system is spin-less and valley-less.
If $\vG$ is replaced by the real space index $\vr$ in the moir\'e supercell, a BM wavefunction can be expressed as 
\begin{equation}
\psi_{n\vk}(\vr,\sigma,l)
=\frac{1}{\sqrt{N_{\vk}}}e^{\I \vk\cdot\vr}u_{n\vk}(\vr,\sigma,l)
=\frac{1}{\sqrt{N_{\vk}}\abs{\Omega}}\sum_{\vG} e^{\I(\vk+\vG)\cdot \vr}u_{n\vk}(\vG,\sigma,l),
\end{equation}
where $u_{n\vk}(\vr,\sigma,l)$ is periodic with respect to $\mathbb{L}$, i.e., $u_{n\vk}(\vr,\sigma,l)=u_{n\vk}(\vr+\vR,\sigma,l), \forall \vR\in\mathbb{L}$.
The normalization condition is chosen such that $u_{n\vk}$ is normalized within the moir\'e unit cell.
Moreover, the factor $\frac{1}{\sqrt{N_{\vk}}}$ ensures that $\psi_{n\vk}$ is normalized within the moir\'e supercell. 
With some abuse of notations, we use $u_{n\vk}(\vr,\sigma,l)$ and $u_{n\vk}(\vG,\sigma,l)$ to denote the coefficients of a BM wavefunction in the real space and reciprocal space, respectively. 
In practical calculations, the number of shell indices $\vG$ needs to be truncated to a finite size $N_{\vG}=N_{G_x}\cdot N_{G_y}$.
Note that throughout the paper, we omit the range of summation unless otherwise specified.
Subsequently, we refer to the set of all planewaves indexed by $\vG$ with sublattice index $\sigma$ and layer index $l$ as the primitive basis of the BM model, and denote the corresponding Fock space by $\mc{F}$.
Let $\hat{c}_{\vk}^{\dagger}(\vG,\sigma,l),\hat{c}_{\vk}(\vG,\sigma,l)$ be the creation and annihilation operators acting on $\mc{F}$, respectively. 
%\FF{The index alpha is not used again!}
%For the sake of brevity, we introduce the internal index $\alpha=(\vG,\sigma,l)$ and write $\hat{c}_{\vk}^{\dagger}(\alpha)=\hat{c}_{\vk}^{\dagger}(\vG,\sigma,l)$.
Then the creation and annihilation operators corresponding to the band $n\vk$ are
\begin{equation}
\label{eqn:creation-op-def}
\begin{split}
\hat{f}^{\dag}_{n\vk} 
=&\sum_{\vG,\sigma,l}\hat{c}_{\vk}^{\dagger}(\vG,\sigma,l)u_{n\vk}(\vG,\sigma,l)
%=\sum_{\alpha} \hat{c}_{\vk}^{\dagger}(\alpha)u_{n\vk}(\alpha)
,\\
\hat{f}_{n\vk} 
=&\sum_{\vG,\sigma,l}\hat{c}_{\vk}(\vG,\sigma,l)u^*_{n\vk}(\vG,\sigma,l)
%=\sum_{\alpha} \hat{c}_{\vk}(\alpha)u^*_{n\vk}(\alpha).
\end{split}
\end{equation}
Here $u_{n\vk}^*$ denotes the complex conjugation of $u_{n\vk}$.
The band creation and annihilation operators satisfy the canonical anticommutation relation $\{\hat{f}^{\dag}_{n\vk},\hat{f}_{n'\vk'}\}
= \delta_{nn'} \delta_{\vk\vk'}$, and define the band basis of the BM model.
Note that the definition of the band creation and annihilation operators can be periodically extended outside the mBZ according to 
\begin{equation}
\hat f^{\dag}_{n(\vk+\vG)}=\hat f^{\dag}_{n\vk}, \quad \hat f_{n(\vk+\vG)}=\hat f_{n\vk}, \quad \vG\in\mathbb{L}^*.
\label{eqn:period_f}
\end{equation}



==> Quantum chemistry TBG/sections/posthf.tex <==
\subsection{Coupled-cluster theory}


Coupled-cluster theory is one of the most widely used post-Hartree-Fock wavefunction methods in quantum chemistry~\cite{BartlettMusial2007}. 
It is built on the exponential ansatz which was independently introduced by Hubbard~\cite{Hubbard1957} and Hugenholtz~\cite{Hugenholtz1957} in 1957 as an alternative to summing many-body perturbation theory contributions order by order. 
In this ansatz the wavefunction takes the form
\begin{equation}
\label{eq:ExponentialParametrization}
|\Psi \rangle 
=
e^{T(\vt)}|\Phi_0 \rangle
\end{equation}
where 
\begin{equation}
\label{eq:ClusterOperator}
T(\vt)=\sum_\mu t_\mu X_\mu
\end{equation}
is the cluster operator determined by the cluster amplitudes $\vt$, and $|\Phi_0 \rangle$ is a chosen reference Slater determinant (most commonly the Hartree--Fock solution). 
The operators $X_\mu$ are the excitation operators with respect to the chosen reference $\Phi_0$, i.e., 
\begin{equation}
\label{eq:ExcitationOperator}
X_\mu
=
X_{i_1,...,i_k}^{a_1,...,a_k}
=
\hat{a}_{a_1}^\dagger...\hat{a}_{a_k}^\dagger \hat{a}_{i_k}...\hat{a}_{i_1}
\end{equation}
where for the sake of compactness we have combined the occupied orbital indices $\{i_l\}$ and virtual orbital indices $\{a_l\}$ in the multi-index $\mu$. 
The ground state energy can then be characterized by 
\begin{equation}
\label{eq:CCEnergy}
\mathcal{E}(\vt)
=
\langle\Phi_0|e^{-T(\vt)} H e^{T(\vt)}| \Phi_0 \rangle.
\end{equation}
The cluster amplitudes $\vt$ are determined by the coupled-cluster equations, i.e., a set of polynomial equations of at most degree four with respect to $\vt$:
\begin{equation}
\label{eq:CCEquations}
0
\overset{!}{=}
F_\mu(\vt)
=
\langle
\Phi_0|X_\mu^\dagger e^{-T(\vt)}H e^{T(\vt)} |\Phi_0
\rangle,\qquad \forall \mu.
\end{equation}
More compactly, Eq.~\eqref{eq:CCEnergy} and~\eqref{eq:CCEquations} can be combined in the coupled-cluster Lagrangian  
\begin{equation}
\label{eq:CCLagrangian}
\mathcal{L}(\vt, \boldsymbol\lambda)
=
\mathcal{E}(\vt)+\langle \lambda, \vF(\vt)\rangle
=
\langle \Phi_0|(I+\Lambda(\boldsymbol\lambda))e^{-T(\vt)}H e^{T(\vt)} |\Phi_0 \rangle
\end{equation}
where 
\begin{equation}
\label{eq:LambdaClusterOperator}
\Lambda(\boldsymbol\lambda)
=
\sum_\mu \lambda_\mu X^\dagger_\mu.
\end{equation}
The states $|e^{T(\vt)} \Phi_0 \rangle$ and $\langle \Phi_0(I+\Lambda(\lambda))e^{-T(\vt)}|$ are commonly referred to as the right and left coupled-cluster solution, respectively.
Due to the projective nature of Eq.~\eqref{eq:CCEnergy} and~\eqref{eq:CCEquations}, the $N$-RDM in coupled-cluster theory is given by 
%\LL{ This is the $N$-particle DM. The 1-RDM should involve traces with respect to the creation and annihilation operator.} 
%\FF{Very important, thanks!}
\begin{equation}
\label{eq:ccNrdm}
\varrho_{\rm CC}(\vt, \boldsymbol\lambda)
=
|e^{T(\vt)} \Phi_0 \rangle\langle
\Phi_0(I+\Lambda(\boldsymbol\lambda))e^{-T(\vt)}|
\end{equation}
ensuring that ${\rm Tr}[H\varrho_{\rm CC}(\vt, \boldsymbol\lambda)]= \mathcal{E}(\vt)$.
The corresponding 1-RDM is then given by
\begin{equation}
\label{eq:cc1rdm}
[P_{\rm CC}(\vt, \boldsymbol\lambda)]_{p, q}
=
\langle \Phi_0(I+\Lambda(\boldsymbol\lambda))e^{-T(\vt)}|
a_p^\dagger a_q
|e^{T(\vt)} \Phi_0 \rangle,
\end{equation}
see~\cite{Helgaker2014} for more details.
We emphasize that this ansatz---in its untruncated form---is equivalent to the full configuration interaction method (i.e., the exact diagonalization method)~\cite{LaestadiusFaulstich2019,Monkhorst1977,Schneider2009}\LL{ Is this the right citation?}\FF{Well, it is `a' reference towards which I am clearly biased. I added the other references, that show the essential parts for the individual directions (they are somewhat hidden though). However, I believe that Andre and I wrote the argument very clearly in this sanibel proceedings, which could be helpful for some readers?}, and is thus computationally infeasible. 
In the past decades, different level of approximations have been suggested to reduce the computational complexity~\cite{BartlettMusial2007,ChanKallayGauss2004,Piecuch2010}. The variant used in the subsequent simulations (and arguably one of the most widely used approximate versions of coupled-cluster theory) is the truncation of the cluster operator in Eq.~\eqref{eq:ClusterOperator} to only contain one-body and two-body excitations, also known as the coupled cluster singles and doubles (CCSD) method.
Note that due to the exponentiation of the cluster operator, the corresponding wavefunction expansion in Eq.~\eqref{eq:ExponentialParametrization} will still contain contributions from higher-body terms.  
One of the central benefits of the exponential ansatz is that it ensures that the energy is size consistent and size extensive, in particular, for (rank complete) truncations of $T$ such as in CCSD~\cite{Helgaker2014}.
The treatment of spin, i.e., restricted (R), unrestricted (U) and generalized (G), as in Hartree--Fock theory, carries on to coupled cluster calculations. 
%Here we shall employ a spin generalized treatment abbreviated GCCSD. 

\subsection{Implementation in PySCF}


The CCSD method is widely implemented in different electronic structure software packages. 
We here use the Python-based Simulations of Chemistry Framework (PySCF)~\cite{SunBerkelbachBluntEtAl2018, SunZhangBanerjeeEtAl2020}. 
The IBM model in \cref{eqn:IBM_Ham} can be defined as a ``customized Hamiltonian'' accessed through the one- and two-electron integrals, referred to as \texttt{h1e} and \texttt{eri}.
These integrals are complex valued, therefore, minor adjustments to PySCF need to be made to enable calculations using these customized Hamiltonians.
We also use the molecular formulation in PySCF, i.e., the \texttt{h1e} and \texttt{eri} are stored without taking advantage of the $\vk$-point symmetry~\cite{McClainSunChanEtAl2017}. This can increases the storage cost by a factor of $N_\vk$, and the computational cost by a polynomial of $N_\vk$.
However, PySCF for crystalline systems taking advantage of the $\vk$-point symmetry also requires further adjustments such as density fitting, which is not currently implemented for the IBM model.

%This goes beyond initial correlated calculations of the IBM model employing electronic structure software and shall consequently be postpone for future works.

Once \texttt{h1e} and \texttt{eri} are constructed, the use of the PySCF software packages allows us to perform GHF and GCCSD calculations on the same footing with a simple code structure.  Here is an example:

\begin{lstlisting}[language=Python, caption=Example code running GHF and GCCSD in PySCF from precomputed integrals.]
from pyscf import gto, scf, cc 

def get_veff(mol, dm, *args):       
    vj, vk= scf.hf.dot_eri_dm(eri, 
    return vj- vk                  
                                    
mol= gto.M()                       
mol.incore_anyway= True            
mol.nelectron= nelec 
                                    
ghf_mf= scf.GHF(mol)               
ghf_mf.get_hcore= lambda *args: h1e
ghf_mf.get_ovlp= lambda *args: ovlp
ghf_mf._eri= eri
ghf_mf.get_veff= get_veff          
                                    
# Running GHF
ghf_mf.kernel()

# Running GCCSD
gcc = cc.GCCSD(ghf_mf)  
gcc.kernel()            
\end{lstlisting}

After the calculations, PySCF also provides compact instructions to evalaute the 1-RDMs so that we can evalaute the observables to detect the symmetry breaking in  Section~\ref{sec:symm}.


==> Quantum chemistry TBG/sections/symmetries_old.tex <==
Both the BM model and the IBM model satisfy a large number of symmetries~\cite{BultinckKhalafLiuEtAl2020}, which can be written as a composition of operators from two different classes (1) Euclidean symmetries (i.e. translations, rotations, and reflections) and (2) complex conjugation.
In the spinless, valleyless regime, the symmetry operation must map the $\vK$ valley to itself, which significantly restricts the number of available symmetry operations. \cref{tab:symmetry} summarizes the relevant symmetry operations in this paper. 
In particular, we focus on the $C_{2 z} \mc{T}$ and $C_{3z}$ symmetries.
The BM model is a non-interacting theory. The 1-RDM satisfies both symmetries, and the corresponding ground state is a band metal. 
On the other hand, the 1-RDM of the IBM model solved at the Hatree-Fock level may spontaneously break such symmetries. 
Our main goal is to characterize the symmetry breaking of the 1-RDM in different parameter regimes. 
If the $C_{2 z} \mc{T}$ symmetry is broken but the $C_{3z}$ symmetry is satisfied, the system is in the quantum anomalous hall (QAH) state. If the $C_{2 z} \mc{T}$ symmetry is satisfied but the $C_{3z}$ symmetry is broken, the system is in the nematic metal (NM) state. 
It is interesting that in the IBM model, one and only one symmetry is observed to be broken at any given parameter regime~\cite{}. 

Although the IBM model is expected to satisfy both the $C_{2 z} \mc{T}$ and $C_{3z}$ symmetries in the continuous limit, such symmetries may be nonetheless weakly broken due to the finite number of shells, $\vk$-points, and the choice of the subtraction term in $\hat{H}_0$.
Therefore we would also like to numerically verify that the IBM Hamiltonian satisfies these symmetries, and/or the extent to which a symmetry is broken by the numerical schemes.  
For both purposes, it is desirable that the order parameters do not depend on the choice of the gauge of the bands.





\begin{table}[ht]
\begin{center}
\renewcommand{\arraystretch}{1.2} %% KDS Makes things a bit eaiser to read imo
\begin{tabular}{l|l|l|l}
\hline Symmetry & Real space & Momentum space &Type \\
\hline$C_{2 z}$ & swap sublattice & swap valleys; \\
& & $\mathbf{k} \rightarrow-\mathbf{k}$ & Unitary\\
\hline$C_{3z}$ & rotate by $120^{\circ}$ & $\mathbf{k} \rightarrow C_{3z}\mathbf{k}$ & Unitary\\
\hline $\mathcal{T}$ & & swap valley; \\
& & $\mathbf{k} \rightarrow-\mathbf{k}$ & Antiunitary\\
\hline $C_{2 z} \mc{T}$ & swap sublattice & $\vk\to\vk$ & Antiunitary\\
\hline
\end{tabular}
\end{center}
\caption{Relevant symmetry operations for the spinless, valleyless IBM model. }
\label{tab:symmetry}
\end{table}

\LL{ Give a picture depicing the action of $C2zT$ and $C3z$ in the real space} \kds{I will make beautiful pictures shortly}

In second quantization, a symmetry operation $g$ is defined by its action on the Fock space $\mc{F}$. By Wigner's theorem \FF{reference?}, any symmetry operation must either be unitary or antiunitary. 
If $g$ is unitary, then for any $a\in\CC$ and any $\ket{\Psi}\in\mc{F}$ $g(a\ket{\Psi})=a g\ket{\Psi}$. 
If $g$ is antiunitary, then $g(a\ket{\Psi})=a^* g\ket{\Psi}$. In particular, $g i g^{-1}=-i$. 
We recall that any anti-unitary symmetry $g$ can be written as $g=\wt{g} \mc{K}$, where $\wt{g}$ is a unitary symmetry and $\mc{K}$ is complex conjugation. \LL{ add a citation} 
Throughout the discussion of this section, we only consider unitary symmetries, we prove analogous results for antiunitary symmetries in Appendix \ref{sec:antiunitary} and summarize the results for both unitary and antiunitary symmetries in Table \ref{tab:symm-breaking}.

\subsection{Representation matrix and sewing matrix}

For any point group symmetry $g$, due to the properties of the Bloch transform, there exists a unitary $D(g)$, called the \textit{representation matrix}, so that the creation operators transform via the rule
\begin{equation}
\begin{split}
    (g \hat{c}_{\vk}^\dag g^{-1})(\alpha) & = \sum_{\alpha'} \hat{c}_{g\vk}^\dag(\alpha') [D(g)]_{\alpha',\alpha} \\
    (g \hat{c}_{\vk} g^{-1})(\alpha) & = \sum_{\alpha'} \hat{c}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha}^{*}
\end{split}
\end{equation}
where $g\vk$ denotes the action of the symmetry $g$ in $\vk$-space and $\hat{c}_{\vk}$ are the primitive creation operators defined in Section \ref{sec:ibm_model}. 
In particular, note that the representation matrix does not depend on $\vk$. 


To study the symmetries of IBM model, we will need to understand how the symmetry $g$ transforms the annihilation operators $f_{n\vk}^\dagger$. We consider the action of $g$ on the BM Hamiltonian and show can be written in terms of the representation matrix $D(g)$.
Suppose we have the quadratic Hamiltonian in the primitive basis $\hat{H}=\sum_{\vk}\sum_{\alpha,\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)$. 
 If $g$ is a unitary symmetry with corresponding representation matrix $D(g)$, then
\begin{equation}
\begin{split}
g\hat{H} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
=& \sum_{\vk} [D(g)h(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
\end{split}
\end{equation}

If $\hat{H}$ is invariant under $g$, i.e., $g\hat{H}g^{-1}=\hat{H}$, then this calculation shows that at the matrix level:
\begin{equation}
D(g) h(\vk)=h(g\vk) D(g).
\end{equation}
In other words, 
\begin{equation}
h(g\vk)D(g)u_{n\vk}=D(g)h(\vk)u_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk},
\end{equation}
or equivalently $D(g)u_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$.

This allows us to define a ``sewing matrix'', $[B(g)]_{\vk}$,
\begin{equation}
\label{eqn:matrix_representation}
(D(g) u_{n\vk})(\alpha)=
\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}(\alpha')=
\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
\end{equation}
Here
\begin{equation}
\label{sec:sewing-def}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk} | D(g) | u_{n\vk}},
%[B(g)]_{\vk,mn} := \sum_{\alpha,\alpha'} u_{m,g\vk}(\alpha) [D(g)]_{\alpha,\alpha'} u_{n\vk}(\alpha').
\end{equation}
where the bra-ket notation denotes contraction over the internal indices
$\alpha,\alpha'$. When the system is gapped, $[B(g)]_{\vk}$ is a unitary matrix
(using a contour integral argument, see Appendix \ref{sec:contour-argument}).
Given the definition of sewing matrices, for unitary operator $g$, one can
calculate that:

%\QZ{ The original representation matrix $D(g)$ is defined in the space of combined indices $\alpha$, while sewing matrix $[B(g)]_{\vk}$ is defined in the band space. It's obvious that the symmetry operation is complete using the representation matrix. Using sewing matrix, the symmetry operation is also complete when all the bands are used. In practice, the number of bands is limited. Therefore, our goal is that the symmetry operations of our interests are ``closed'' and ``complete'' using the corresponding sewing matrices: Given a set of bands $\{u_{n\vk}\}_{n,\vk}$, a)``closed'':  for any unitary/antiunitary operator $g$ of interest, $\sum_{m}  u_{m,g\vk} [B(g)]_{\vk,mn}\in\{u_{n\vk}\}_{n,\vk}$; b) ``complete'': for any $u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ and unitary (antiunitary) operator $g$ of interest, $D(g)u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ ($D(g)u^*_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$) and $D(g)u_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$ ($D(g)u^*_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$). In this note, we are particularly interested in the spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetry. In a single-valley, spinless system, one pair of flat bands with different sublattice index $\sigma=\pm$ is enough to satisfy the conditions above. More details are in Section \ref{sec:ibm-symm}}
%\LL{ It seems that a projection operator approach might be a better way to go than the abstract "closed" and "complete" concepts. Let us discuss this.} 
\begin{equation}
\begin{split}
g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}(\alpha')\\
=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
u_{n\vk}(\alpha)\\
=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
\end{split}
\label{eqn:sewing_transf_unitary}
\end{equation}
Hence the sewing matrices encode how $\hat{f}^{\dag}_{n\vk}$ transforms under the symmetry action.

%
%\LL{ Appendix?} \kds{I'd like to keep the formula for the sewing matrix in the main text so people implementing this don't need to look at the appendix, but otherwise let's move the rest to the appendix?}
%Now to turn to consider antiunitary symmetries. Since any antiunitary transformation can be written as $g \mc{K}$ where $g$ is a unitary transform and $\mc{K}$ is complex conjugation, similar calculations show that if $\hat{H}_{\mathrm{BM}}$ is invariant under an antiunitary symmetry then the corresponding matrix equation is:
%\begin{equation}
%D(g) h(\vk)=h(g\vk)^* D(g).
%\end{equation}
%From this matrix relation, one can check that the corresponding sewing matrix can be defined by the relations:
%\begin{equation}
%\begin{split}
%(D(g) u_{n\vk})(\alpha) & =
%\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}^*(\alpha')=
%\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]^{\text{anti}}_{\vk,mn} \\
%[B(g)]^{\text{anti}}_{\vk,mn} & = \braket{u_{m,g\vk} | D(g) | u^*_{n\vk}}.
%\end{split}
%\end{equation}
%Using these definitions, we can now calculate how $f^\dag_{n\vk}$ transforms under antiunitary symmetry: 
%\[
%\begin{split}
%(g \mc{K}) \hat{f}^{\dag}_{n\vk} (g \mc{K})^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}^*(\alpha')\\
%=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
%u_{n\vk}^*(\alpha)\\
%=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]^{\text{anti}}_{\vk,mn} \\
%=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]^{\text{anti}}_{\vk,mn}.
%\end{split}
%\]
%


%\QZ{Maybe move the antiunitary case to the Appendix.}
%
%The case when $g$ is antiunitary is similar. 
%Here
%\begin{equation}
%\begin{split}
%g\hat{H}_{\mathrm{BM}} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
%=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]^*_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
%=& \sum_{\vk} [D(g)h^*(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
%\end{split}
%\end{equation}
%So
%\begin{equation}
%D(g) h^*(\vk)=h(g\vk) D(g).
%\end{equation}
%Hence
%\begin{equation}
%h(g\vk)D(g) u^*_{n\vk}=D(g) h^*(\vk)u^*_{n\vk}=\varepsilon^*_{n\vk} D(g)u^*_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk}.
%\end{equation}
%In other words, $D(g)u^*_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$. 
%The sewing matrix is then given by 
%\begin{equation}
%(D(g) u^{*}_{n\vk})(\alpha)=
%\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u^{*}_{n\vk}(\alpha')=
%\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
%\end{equation}
%Here 
%\[
%[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u^*_{n\vk}}
%\]
%and $[B(g)]_{\vk}$ is a unitary matrix. The transformation rule remains the same
%\begin{equation}
%\begin{split}
%g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u^*_{n\vk}(\alpha')\\
%=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
%u^*_{n\vk}(\alpha)\\
%=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
%=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
%\end{split}
%\end{equation}

\subsection{Gauge-invariant detection of symmetry breaking in the 1-RDM}
\label{sec:symm-broken}

Suppose that $\hat{H}_{\mathrm{IBM}}$ indeed satisfies a unitary symmetry $g$, and we are interested in whether the symmetry is spontaneously broken in the mean-field solutions.
If the many-body wavefunction $\ket{\Psi}$ satisfies the symmetry $g$, then
\[
g\ket{\Psi}\bra{\Psi}g^{-1}=\ket{\Psi}\bra{\Psi}.
\]
Here $g$ acting on $\ket{\Psi}$ is implemented by $g$ acting on each individual creation operators, and the vaccum is an eigenfunction of any symmetry $g\ket{0}=\ket{0}$.
Therefore the 1-RDM should satisfy
\begin{equation}
\begin{split}
[P(\vk)]_{nm}=&\braket{\Psi|\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}|\Psi}=\Tr[\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}\ket{\Psi}\bra{\Psi}]\\
=&\Tr[g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}g\ket{\Psi}\bra{\Psi}g^{-1}]\\
=&\braket{\Psi|g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}|\Psi}\\
=&\sum_{pq} [B(g)]_{\vk,pm} [B(g)]^*_{\vk,qn}\braket{\Psi|\hat{f}^{\dag}_{p,g\vk} \hat{f}_{q,g\vk}|\Psi}\\
=&([B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk})_{nm}.
\end{split}
\end{equation}
Therefore we can check the norm 
\begin{equation}
\label{eqn:order-parameter}
\mc{C}_{\vk}(g)=\norm{[B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk}-P(\vk)}=\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}
\end{equation}
to detect broken symmetry.

Next, we will show that $\mc{C}_{\vk}(g)$ is invariant under arbitrary unitary rotation. We perform an unitary rotation $U(\vk)$ on the original basis. Towards these ends, suppose that we perform the mapping
\[
\hat{f}^{\dagger}_{n\vk} \mapsto \sum_{n'}\hat{f}^{\dagger}_{n'\vk}[U(\vk)]_{n'n}.
\]

Under this unitary rotation, the 1-RDM is
\begin{equation}
\begin{split}
\label{eq:1rdm-gauge}
[P(\vk)]_{nm}\mapsto&\braket{\Psi|\sum_{m'}\hat{f}^{\dagger}_{m'\vk}[U(\vk)]_{m'm} \sum_{n'}[U(\vk)]^*_{n'n}\hat{f}_{n'\vk}|\Psi}\\
=&\sum_{m'n'}[U(\vk)]_{m'm}[U(\vk)]^*_{n'n}\braket{\Psi|\hat{f}^{\dagger}_{m'\vk} \hat{f}_{n'\vk}|\Psi},\\
=&(U^{\dagger}(\vk)P(\vk)U(\vk))_{nm}.
\end{split}
\end{equation}
By a similar calculation, it can be checked that the sewing matrices transform as:
\begin{equation}
[B(g)]_{\vk,mn} \mapsto (U^{\dagger}(g\vk)B(g)_{\vk}U(\vk))_{mn}
\end{equation}
Therefore, for unitary operator, the norm is
\begin{equation}
\begin{split}
\mc{C}_{\vk}(g)\mapsto&\norm{U^{\dagger}(g\vk)P(g\vk)U(g\vk)U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)-U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)U^{\dagger}(\vk)P(\vk)U(\vk)},\\
=&\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)},
\end{split}
\end{equation}
Hence $\mc{C}_{\vk}(g)$ is gauge invariant. 

One can repeat similar calculations for anti-unitary symmetries to derive a gauge-invariant order parameter, we go through such calculations in Appendix \ref{sec:antiunitary} and summarize the results in Table \ref{tab:symm-breaking}.
\begin{center}
\begin{table}[ht]
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{c|cc}
     & Sewing Matrix $[B(g)]_{\vk,mn}$ & Order Parameter $\mc{C}_{\vk}(g)$ \\
     \hline 
    Unitary & $\braket{u_{m,g\vk} | D(g) | u_{n\vk}}$ & $\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}$ \\
    Anti-Unitary & $\braket{u_{m,g\vk} | D(g) | u^*_{n\vk}}$ & $\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)^*}$
\end{tabular}
\caption{\kds{Summary of Results}}
\label{tab:symm-breaking}
\end{table}
\end{center}
\kds{We need to decide about notation for $\mc{C}_{\vk}(g)$. I originally put $\mc{C}_{\vk}(g)$ and $\mc{C}_{\vk}^{\text{anti}}(g)$, but I realize now it's a little inelegant.} \LL{ I sort of agree. Since $g$ already carries the information of unitary/anti-unitary, maybe we do not need the superscript ``anti''?} \kds{We're kind of abusing notation above. If $g$ is anti-unitary then $D(g)$ should be the representation matrix for $g \mc{K}$ (i.e. the unitary component of $g$). This doesn't really change the overall story, but it's important to be consistent}

\subsection{Connection with the order parameter in the Chern band basis}

Let us also show the connection between $\mc{C}_{\vk}(\mc{C}_{2z}\mc{T})$ and the order parameter used in \cite{SoejimaParkerBultinckEtAl2020} using a particular gauge fixing called the Chern band basis. 
According to the gauge choice of the Chern band basis, the sewing matrix takes the form
\[
[B(C_{2z}\mc{T})]^{\text{anti}}_{\vk}=\sigma_x  e^{\I \theta(\vk)}
\]
for some $\vk$-dependent phase $\theta(\vk)$. 
In this basis, the $C_{2z}\mc{T}$ symmetry breaking is detected by computing
\begin{equation}
\gamma_z(\vk)=\Tr[P(\vk)\sigma_z]=P_{11}(\vk)-P_{22}(\vk).
\end{equation}

On the other hand, the commutator satisfies
\[
P(\vk)[B(C_{2z}\mc{T})]^{\text{anti}}_{\vk}-[B(C_{2z}\mc{T})]^{\text{anti}}_{\vk}P(\vk)=e^{\I \theta(\vk)}
\begin{pmatrix}
P_{21}(\vk)-P_{12}(\vk) & P_{22}(\vk)-P_{11}(\vk)\\
P_{11}(\vk)-P_{22}(\vk) & P_{12}(\vk)-P_{21}(\vk)
\end{pmatrix}
\]
Therefore $\gamma_z(\vk)$ can be interpreted as checking the magnitude of the off-diagonal element of commutator in the Chern band basis. However, the order parameter $\gamma_z(\vk)$ is designed specifically for the Chern band basis and $C_{2z}\mathcal{T}$ symmetry, which is unable to generalize to the other band basis and other symmetries. On the other hand, the commutator is designed for any symmetries of our interests and works for any band basis. Using the norm of commutator, a clear spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetries is observed for both BM band basis and Chern band basis in Section \ref{sec:numerical}.



%When the energy band basis $\hat{f}^{\dagger}_{n\vk}$ is fixed, the matrix representations of unitary/antiunitary operators are also fixed. In the other word, sewing matrices are the same up to a arbitrary unitary rotation and explicit forms of sewing matrices can be obtained only when this unitary rotation is fixed.


\subsection{Generalization and multi-band case}
\label{sec:multi-band}

In our previous sections, two flat bands $u_{\pm1,\vk}$ with different sublattice index $\sigma=\pm$ are used to project the Hamiltonian and compute the corresponding sewing matrices. Meanwhile, we make the assumption that all the states with band index $n<-1$ ($n>1$) are fully occupied (unoccupied). 
This assumption is valid for the first magic angle $\theta=1.1^{\circ}$, where the two flat bands are isolated from the other energy bands in the band structure of BM model. 
For the other magic angles, there may not exist such isolated flat bands\LL{ cite}. 
\LL{ Even for the first magic angle, it may be desirable to include more bands to systematically improve the accuracy of the IBM model.} 
Therefore, we need to include more bands in our projection in order to get numerically accurate results. Generally, we assume that $2N_{\max}$ bands are used and all the states with band index $n<-N_{\max}$ ($n>N_{\max}$) are full (empty). Away from the flat band case, the band energies are also relatively away from zero. One more symmetry needs to be defined here for the multi-band case, which is unitary ``particle-hole symmetry'' $\mc{P}$\cite{song_2019,TBGII,TBGIII}:
\begin{equation}
[D(\mc{P})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',-\vG} \delta_{l',-l} \delta_{\sigma',\sigma}\zeta_l,
\end{equation}
where $\mc{P}\vk=-\vk$ and $\zeta_l=\pm1$ for $l=\pm$. Note that $\mc{P}$ anticommutes with the BM Hamiltonian and $\mc{P}$ maps creation operators to creation operators (rather than annihilation operators)\LL{ cite} . Therefore, ``particle-hole symmetry'' is mainly a map from positive energy band $u_{n\vk}$ to negative energy band $u_{-n\vk}$. Using the particle-hole symmetry $\mc{P}$ and rotation symmetry $C_{2z}$, the band structure of the BM Hamiltonian has the property:
\begin{equation}
    \epsilon_{n,\vk}=-\epsilon_{-n,-\vk},\ \epsilon_{n,\vk}=\epsilon_{n,-\vk}\ \to\ \epsilon_{n,\vk}=-\epsilon_{-n,\vk}.
\end{equation}

\LL{Can we say how to choose these additional bands to satisfy the particle hole symmetry? The easiest way is probably to cite some paper saying that for some $N_{max}>1$ there is another gap separating the bands away from other bands.} 
This band structure also implicitly reflects that $\epsilon_{1,\vk}=\epsilon_{-1,\vk}=0$ in the two flat band case. Away from the flat band case, one pair of bands with positive/negative energies should be included in our set of bands and this pair is connected by the ``particle-hole symmetry''. \LL{ This part seems out of date now.} Besides that, in order to ensure the ``completeness'' of the symmetry operation, $u_{n\vk}$ and $D(g)u_{n\vk}$ should also be included. with this setup, our norm of the commutator can be generalized to the multi-band case by defining
\begin{equation}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u_{n\vk}},\ \ \ m,n\in[-N_{\max},N_{\max}].
\end{equation}


% This is enough for our discussion about $C_{2z}\mc{T}$ and $C_{3z}$ symmetry in the single-valley, spinless system. However, if we want to further discuss about other symmetries, more bands are needed. One example is the rotation symmetry $C_{2x}$:
% \begin{equation}
% [D(C_{2x})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',C_{2x}\vG} \delta_{l',-l} \left(\sigma_x\right)_{\sigma',\sigma},
% \end{equation}
% where $C_{2x}\vk=C_{2x}\left(k_x,k_y\right)=\left(k_x,-k_y\right)$.

% The sewing matrices are $[B(C_{2x})]_{\vk,mn}=[B(C_{2z})]_{\vk,mn}$ if only two flat bands are used. Moreover, the ``completeness'' is broken since $D(C_{2z})$

\subsection{Symmetries of the IBM Model}
\label{sec:ibm-symm}

\LL{ Extra thing: for $\hat{H}_I$ it is sufficient to check that $\hat{\rho}_{\vq}$ satisfies the symmetry} 

For the interacting BM Hamiltonian, it's sufficient to verify  \LL{small thing: there is normal ordering involved} 
\begin{equation}
\begin{split}
g\hat{H}_Ig^{-1}&=\frac{1}{2 \abs{\Omega}N_{\vk}} 
\sum_{\vq} V(\vq)g\hat{\rho}_{\vq}g^{-1}g\hat{\rho}_{-\vq}g^{-1},\\
\Longleftrightarrow&\\
g\hat{\rho}_{\vq}g^{-1}&=g\sum_{\vk\in \Omega^*} \sum_{mn} \hat f_{m\vk}^{\dagger} [\Lambda_{\vk}(\vq)]_{mn} \hat f_{n(\vk+\vq)}g^{-1},\\
&=\sum_{\vk}\sum_{mn}\sum_{m'n'}[\Lambda_{\vk}(\vq)]_{mn}\hat{f}^{\dag}_{m',g\vk}[B(g)]_{\vk,m'm}\hat{f}_{n,g(\vk+\vq)}[B(g)]^*_{\vk,}
\end{split}
\end{equation}





==> Quantum chemistry TBG/tikzlibraryquantikz.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.6
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.6:
%	changed packaging so there isn't a compile warning any more
%	modified the meter command so that \meter[draw=blue]{} colours everything blue, not just outline.
%	added trash command
%	added \ctrlbundle command so that \ctrl works well with \qwbundle[alternate]. If you supple \ctrlbundle[2]{}, then the bundle only contains 2 wires instead of the default of 3
%	\qwbundle[alternate] now also works with the parameter \qwbundle[alternate=2] to only have 2 wires in the bundle.
%	added \midstick. Works a bit like rstick and lstick, but reserves space for the text. Can choose to have brackets=none|left|right|both (default is both). Gives better method for circuit identities and other things.
%	added "align equals at" key for setting circuit identities (specifies wire number that should line up with equals. can be non-integer)
%	added makeebit command. accepts one parameter which is the text. Haven't got tyling and different angles of the split working yet.
%   added bundle option to supplement nwires and cwires.
%	fixed bug where you couldn't put a wire command after the declaration of a multi-qubit gate command.
%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

%\ProvidesPackage{quantikz}[2020/04/27 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools,pgfmath}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings,math}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\pgfkeysgetvalue{/quantikz/bundle}{\bundle}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\IfInList{1}{\bundle}{\qwbundle[alternate]{}}{\qw}}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomc{\noexpand\vqbundleexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\IfInList{\val}{\bundle}{\newcomc}{\newcomb}}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}%
 		\dotikzset%
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}%
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}%
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1%
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}%
 		   \dotikzset%
 		   \globaldefs=0%
%		
 	}
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%import options
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}

\newcommand\midstick[2][]{%
	\hphantom{\text{gg#2gg}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\mn{\the\numexpr\m-1\relax}
	\edef\k{\the\numexpr\n+\quantwires-1\relax}
	\settowidth{\myl}{gg#2gg}
	%if more than 1 wire, need to reserve space for each wire
	\ifthenelse{\quantwires=1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={\the\myl}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
      	\globaldefs=0
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@mid\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
	}{
	\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[anchor=mid,#2]center:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(midgr-\row-\col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\row-\col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(midgr-\row-\col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\row-\col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

\DeclareDocumentCommand{\makeebit}{O{-45}O{}m}{
	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(#1)}!#1:(\tikztotarget)$) node [anchor=east,style={#2}]{#3} -- (\tikztotarget) }]{d}
}

% \newcommand{\makeebit}[2][-45]{
% 	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!0.707!#1:(\tikztotarget)$) node [anchor=east]{#2} -- (\tikztotarget) }]{d}
% }

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals\globaldefs=0}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.base)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}
}}
%\show\temp
\temp
}
}

%initialise all the pgfkeys for key=value parameter passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}},/tikz/align equals at/.code={\setmiddle{#1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.default=1,alternate/.code={\def\helper{#1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1},bundle/.initial={-1},brackets/.is choice,brackets/.initial=both}
\pgfkeys{/quantikz,brackets/.cd,none/.code={\def\leftbrace{0}\def\rightbrace{0}},left/.code={\def\leftbrace{1}\def\rightbrace{0}},right/.code={\def\leftbrace{0}\def\rightbrace{1}},both/.code={\def\leftbrace{1}\def\rightbrace{1}}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {} \qw}


%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
\newcommand{\vqbundleexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper>0}{
		\arrow[arrows,yshift=0.1cm]{l}
		\ifthenelse{\helper=1}{\arrow[arrows]{l}}{}
		\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}\qw
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
	trash/.style={path picture={\draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},minimum height=2.5em,minimum width=2em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}

==> backup/comutator_norm.tex <==
Now that we have discussed how symmetry acts on our initial choice of creation and annihilation operators, will derive two gauge independent quantities, $\mc{C}_{\vk}$ and $\mc{C}_{\vk}^{\text{anti}}$, which check for symmetry breaking for unitary and antiunitary symmetries respectively.

Suppose that $\hat{H}_{\mathrm{IBM}}$ indeed satisfies a unitary symmetry $g$, and we are interested in whether the symmetry is spontaneously broken in the mean-field solutions \kds{I think we can use this to check whether the symmetry is broken using any method?}.\QZ{I agree.} 
If the many-body wavefunction $\ket{\Psi}$ satisfies the symmetry $g$, then
\[
g\ket{\Psi}\bra{\Psi}g^{-1}=\ket{\Psi}\bra{\Psi}.
\]
Here $g$ acting on $\ket{\Psi}$ is implemented by $g$ acting on each individual creation operators, and the vaccum is an eigenfunction of any symmetry $g\ket{0}=\ket{0}$.
Therefore the 1-RDM should satisfy
\begin{equation}
\begin{split}
[P(\vk)]_{nm}=&\braket{\Psi|\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}|\Psi}=\Tr[\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}\ket{\Psi}\bra{\Psi}]\\
=&\Tr[g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}g\ket{\Psi}\bra{\Psi}g^{-1}]\\
=&\braket{\Psi|g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}|\Psi}\\
=&\sum_{pq} [B(g)]_{\vk,pm} [B(g)]^*_{\vk,qn}\braket{\hat{f}^{\dag}_{p,g\vk} \hat{f}_{q,g\vk}}=([B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk})_{nm}.
\end{split}
\end{equation}
Therefore we can check the norm 
\begin{equation}
\label{eqn:order-parameter}
\mc{C}_{\vk}(g)=\norm{[B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk}-P(\vk)}=\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}
\end{equation}
to detect broken symmetry.

Similarly, for antiunitary symmetries we can check the norm
\begin{equation}
\label{eqn:order-parameter-anti}
\mc{C}^{\text{anti}}_{\vk}(g)=\norm{[B(g)]_{\vk}^{\dag}P(-g\vk)[B(g)]_{\vk}-P(\vk)^*}=\norm{P(-g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)^*}.
\end{equation}

Let us also show the connection between $\mc{C}_{\vk}(\mc{C}_{2z}\mc{T})$ and the order parameter used in \cite{SoejimaParkerBultinckEtAl2020} using a particular gauge fixing called the Chern band basis. In the Chern band basis, we have
\[
[B(C_{2z}\mc{T})]_{\vk}=\sigma_x  e^{\I \theta(\vk)}
\]
for some $\vk$-dependent phase $\theta(\vk)$. 
In this basis, the $C_{2z}\mc{T}$ symmetry breaking is detected by computing
\begin{equation}
\gamma_z(\vk)=\Tr[P(\vk)\sigma_z]=P_{11}(\vk)-P_{22}(\vk).
\end{equation}

\QZ{Should $C_{2z}\mc{T}$ be antiunitary?}

On the other hand, the commutator satisfies
\[
P(\vk)[B(C_{2z}\mc{T})]_{\vk}-[B(C_{2z}\mc{T})]_{\vk}P(\vk)=e^{\I \theta(\vk)}
\begin{pmatrix}
P_{21}(\vk)-P_{12}(\vk) & P_{22}(\vk)-P_{11}(\vk)\\
P_{11}(\vk)-P_{22}(\vk) & P_{12}(\vk)-P_{21}(\vk)
\end{pmatrix}
\]
Therefore $\gamma_z(\vk)$ can be interpreted as checking the magnitude of the off-diagonal element of commutator in the Chern band basis. \QZ{However, the order parameter $\gamma_z(\vk)$ is designed specifically for the Chern band basis and $C_{2z}\mathcal{T}$ symmetry, which is unable to generalize to the other band basis and other symmetries. On the other hand, the commutator is designed for any symmetries of our interests and works for any band basis. Using the norm of commutator, a clear spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetries is observed for both BM band basis and Chern band basis in Section \ref{sec:numerical}.}



==> backup/multi_band.tex <==
In our previous sections, two flat bands $u_{\pm1,\vk}$ with different sublattice index $\sigma=\pm$ are used to project the Hamiltonian and compute the corresponding sewing matrices. Meanwhile, we make the assumption that all the states with band index $n<-1$ ($n>1$) are full (empty). This is enough for the first magic angle $\theta=1.1^{\circ}$, since this two flat bands are isolated from the other energy bands in the band structure of BM model. However, for the other magic angles, there doesn't exist such isolated flat bands. Therefore, we need to include more bands in our projection in order to get numerically accurate results. Generally, we assume that $2N_{\max}$ bands are used and all the states with band index $n<-N_{\max}$ ($n>N_{\max}$) are full (empty). Away from the flat band case, the band energies are also relatively away from zero. One more symmetry needs to be defined here for the multi-band case, which is unitary ``particle-hole symmetry'' $\mc{P}$\cite{song_2019}\cite{TBGII}\cite{TBGIII}:
\begin{equation}
[D(P)]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',-\vG} \delta_{l',-l} \delta_{\sigma',\sigma}\zeta_l,
\end{equation}
where $\mc{P}\vk=-\vk$ and $\zeta_l=\pm1$ for $l=\pm$. Note that $\mc{P}$ anticommutes with the BM Hamiltonian and $\mc{P}$ maps creation operators to creation operators (rather than annihilation operators). Therefore, ``particle-hole symmetry'' is mainly a map from positive energy band $u_{n\vk}$ to negative energy band $u_{-n\vk}$. Using the particle-hole symmetry $\mc{P}$ and rotation symmetry $C_{2z}$, the band structure of the BM Hamiltonian has the property:
\begin{equation}
    \epsilon_{n,\vk}=-\epsilon_{-n,-\vk},\ \epsilon_{n,\vk}=\epsilon_{n,-\vk}\ \to\ \epsilon_{n,\vk}=-\epsilon_{-n,\vk}.
\end{equation}

This band structure also implicitly reflects that $\epsilon_{1,\vk}=\epsilon_{-1,\vk}=0$ in the two flat band case. Away from the flat band case, one pair of bands with positive/negative energies should be included in our set of bands and this pair is connected by the ``particle-hole symmetry''. Besides that, in order to ensure the ``completeness'' of the symmetry operation, $u_{n\vk}$ and $D(g)u_{n\vk}$ should also be included. with this setup, our norm of the commutator can be generalized to the multi-band case by defining
\begin{equation}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u_{n\vk}},\ \ \ m,n\in[-N_{\max},N_{\max}].
\end{equation}


% This is enough for our discussion about $C_{2z}\mc{T}$ and $C_{3z}$ symmetry in the single-valley, spinless system. However, if we want to further discuss about other symmetries, more bands are needed. One example is the rotation symmetry $C_{2x}$:
% \begin{equation}
% [D(C_{2x})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',C_{2x}\vG} \delta_{l',-l} \left(\sigma_x\right)_{\sigma',\sigma},
% \end{equation}
% where $C_{2x}\vk=C_{2x}\left(k_x,k_y\right)=\left(k_x,-k_y\right)$.

% The sewing matrices are $[B(C_{2x})]_{\vk,mn}=[B(C_{2z})]_{\vk,mn}$ if only two flat bands are used. Moreover, the ``completeness'' is broken since $D(C_{2z})$


==> backup/symm_bm.tex <==


\QZ{In this section, we introduce the matrix representation of the symmetry operation and discuss the discrete symmetries of the non-interacting BM model. These definitions help us get prepared for the following discussion about the projected IBM Hamiltonian in Section \ref{sec:ibm-symm} and the spontaneous symmetry breaking in Section \ref{sec:symm-broken}.}

%\QZ{In the single-valley, spinless system, we abbreviate the valley and spin dimension.} We introduce a multi-index $\alpha=(\vG,\sigma,l)$ to denote the ``internal variables'', i.e., the BM wavefunction is $u_{n\vk}(\alpha)$, and the total number of internal variables is $N_{\alpha}$. The action of a discrete symmetry operator $g$ on the fermion basis $\hat c^{\dag}_{\vk}(\alpha)$ is
%\begin{equation}
%g\hat{c}^{\dag}_{\vk}(\alpha)g^{-1} = \sum_{\alpha'} 
%\hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha}.
%\end{equation}
%The unitary matrix $D(g)\in \CC^{N_{\alpha}\times N_{\alpha}}$ is called the representation matrix.
%Similarly $g$ acting on the annihilation operators 
%\begin{equation}
%g\hat{c}_{\vk}(\alpha)g^{-1} = \sum_{\alpha'} 
%\hat{c}_{g\vk}(\alpha') [D(g)]^*_{\alpha',\alpha}.
%\end{equation}
%A symmetry $g$ is unitary if for any $c\in \CC$, $gcg^{-1}=c$. 
%A symmetry $g$ is antiunitary if for any $c\in \CC$, $gcg^{-1}=c^*$. 

For example, the $C_{3z}$ symmetry is unitary which maps the $\vK$ valley into an equivalent $\vK$ valley. Specifically, it maps $\vK+\vk\to \vK+C_{3z}\vk$.
So
\begin{equation}
(C_{3z})\hat{c}^{\dag}_{\vk}(\vG,\sigma,l)(C_{3z})^{-1} = \sum_{\alpha'}
\hat{c}^{\dag}_{C_{3z}\vk}(\vG',\sigma',l') [D(C_{3z})]_{\alpha',\alpha}.
\end{equation}
with
\begin{equation}
[D(C_{3z})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',C_{3z}\vG} \delta_{l',l} \left(e^{\I \frac{2\pi}{3} \sigma_z}\right)_{\sigma',\sigma}.
\end{equation}
The $C_{2z}\mc{T}$ symmetry is antiunitary which maps $\vk\to \vk$
\begin{equation}
(C_{2z}\mc{T})\hat{c}^{\dag}_{\vk}(\vG,\sigma,l)(C_{2z}\mc{T})^{-1} = \sum_{\alpha'}
\hat{c}^{\dag}_{\vk}(\vG',\sigma',l') [D(C_{2z}\mc{T})]_{\alpha',\alpha}.
\end{equation}
with
\begin{equation}
[D(C_{2z}\mc{T})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',\vG} \delta_{l',l} (\sigma_x)_{\sigma',\sigma}.
\end{equation}
 
The BM Hamiltonian commutes with both $C_{2z}\mc{T}$ and $C_{3z}$. 




==> backup/symm_broken.tex <==
\QZ{I adjusted the indices in this follwing content.}


%When the energy band basis $\hat{f}^{\dagger}_{n\vk}$ is fixed, the matrix representations of unitary/antiunitary operators are also fixed. In the other word, sewing matrices are the same up to a arbitrary unitary rotation and explicit forms of sewing matrices can be obtained only when this unitary rotation is fixed.
Next, we will show that $\mc{C}_{\vk}(g)$ is invariant under arbitrary unitary rotation. We perform an unitary rotation $U(\vk)$ on the original basis. Towards these ends, suppose that we perform the mapping
%In particular, we are able to map the original basis into the Chern band basis using the unitary rotation defined in \cite{SoejimaParkerBultinckEtAl2020}.
\[
\hat{f}^{\dagger}_{n\vk} \mapsto \sum_{n'}\hat{f}^{\dagger}_{n'\vk}[U(\vk)]_{n'n}.
\]

Under this unitary rotation, the 1-RDM is
\begin{equation}
\begin{split}
[P(\vk)]_{nm}\to&\braket{\Psi|\sum_{m'}\hat{f}^{\dagger}_{m'\vk}[U(\vk)]_{m'm} \sum_{n'}[U(\vk)]^*_{n'n}\hat{f}_{n'\vk}|\Psi}\\
=&\sum_{m'n'}[U(\vk)]_{m'm}[U(\vk)]^*_{n'n}\braket{\Psi|\hat{f}^{\dagger}_{m'\vk} \hat{f}_{n'\vk}|\Psi},\\
=&(U^{\dagger}(\vk)P(\vk)U(\vk))_{nm}.
\end{split}
\end{equation}
By a similar calculation, it can be checked that the sewing matrices transform as:
\begin{equation}
[B(g)]_{\vk,mn} \mapsto (U^{\dagger}(g\vk)B(g)_{\vk}U(\vk))_{mn}
\end{equation}
Therefore, the norm is
\begin{equation}
\begin{split}
\mc{C}_{\vk}(g)\to&\norm{U^{\dagger}(g\vk)P(g\vk)U(g\vk)U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)-U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)U^{\dagger}(\vk)P(\vk)U(\vk)},\\
=&\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}.
\end{split}
\end{equation}

\LL{ The antiunitary case requires separate treatment.} 

==> backup/symm_ibm.tex <==
In order to check the symmetries of the interacting BM model, we need to discuss the interacting term in \cref{eqn:interaction_simplify}. For unitary/antiunitary operator, it is sufficient to verify the symmetries of form factors:
$$
[\Lambda_{\vk}(\vq)]_{mn}=\braket{u_{m\vk}|u_{n,\vk+\vq}},
$$
where $u_{m\vk}$, $u_{n,\vk+\vq}$ are the flat bands in the BM band structure. It has been proven that the BM model has $C_{2z}\mc{T}$ symmetry. Given a flat band $u_{m\vk}$, another band $D[g]u_{m\vk}$ is also a flat band. For example, two flat bands can be chosen as $u_{1,\vk}$ and $u_{-1,\vk}=\sigma_xu^*_{1,\vk}$. With this kind of setup, the flat bands always include the pairs of bands and each pair is connected by one specific symmetry. In this case, the symmetry operation using sewing matrix can also be ``closed'' and ``complete''. In Chern band basis $u_{\pm,\vk}=u_{\pm1,\vk}$, the sewing matrix is defined as $[B(C_{2z}\mathcal{T})]_{\vk,mn}=\braket{u_{m\vk}|\sigma_x|u^*_{n\vk}}=\braket{u_{m\vk}|u_{-n\vk}}=\delta_{m,-n}$. In random band basis $u_{\pm,\vk}=c_{\pm,1,\vk}u_{1,\vk}+c_{\pm,-1,\vk}u_{-1,\vk}$, the sewing matrix is $[B(C_{2z}\mathcal{T})]_{\vk,mn}=c^*_{m,-1,\vk}c^*_{n,1,\vk}+c^*_{m,1,\vk}c^*_{n,-1,\vk}$. It's easy to verify that these sewing matrices are ``closed'' and ``complete''.


Then for unitary operator, we have

\begin{equation}
\begin{split}
[[B(g)]^{\dag}_{\vk} \Lambda_{g\vk}(\vq) [B(g)]_{\vk+\vq}]_{mn}&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'} [\Lambda_{g\vk}(\vq)]_{n'm'}[B(g)]_{\vk+\vq,m'n},\\
&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'}\braket{u_{n',g\vk}|u_{m',g\vk+g\vq}}[B(g)]_{\vk+\vq,m'n}\\
&=\braket{u_{m\vk}|D^{\dag}(g)D(g)|u_{n,\vk+\vq}},\\
&=\braket{u_{m\vk}|u_{n,\vk+\vq}}=[\Lambda_{\vk}(\vq)]_{mn},
\end{split}
\end{equation}
and for antiunitary operator: 
\begin{equation}
\begin{split}
[[B(g)]^{\dag}_{\vk} \Lambda_{g\vk}(\vq) [B(g)]_{\vk+\vq}]_{mn}&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'} [\Lambda_{g\vk}(\vq)]_{n'm'}[B(g)]_{\vk+\vq,m'n},\\
&=\sum_{m'n'}[B(g)]^{\dag}_{\vk,mn'}\braket{u_{n',g\vk}|u_{m',g\vk+g\vq}}[B(g)]_{\vk+\vq,m'n}\\
&=\braket{u^*_{m\vk}|D^{\dag}(g)D(g)|u^*_{n,\vk+\vq}},\\
&=\braket{u^*_{m\vk}|u^*_{n,\vk+\vq}}=[\Lambda^*_{\vk}(\vq)]_{mn}.
\end{split}
\end{equation}

This holds for both BM and Chern band basis. To summarize, the flat bands connected by the desired symmetry should be included to form a complete set of basis in the projected space.

For the subtraction term in \cref{eqn:subtracted_HF}, it can be verified using
\begin{equation}
[B(g)]^{\dag}_{\vk}h_s(g\vk)[B(g)]_{\vk}=h_s(\vk),
\end{equation}
which is equivalent to verify that $[B(g)]^{\dag}_{\vk}\delta P^0(g\vk+g\vq)[B(g)]_{\vk}=\delta P^0(\vk+\vq)$ for unitary operator. Therefore, the symmetries of the subtracted Hamiltonian still holds if the reference density also have the same symmetries. Some common choice of the reference density includes: (i) the ground state density of the BM model; (ii) the ground state density of the decoupled BM model; (iii) the charge neural point ($\delta P^0=0$). All these choice share the same symmetries with BM model.

==> backup/symm_notation.tex <==
\QZ{ For the eigenstates $u_{n\vk}$, we have $u_{n\vk}=u_{n\vk}(\alpha)$.}

Symmetries play an important role in both the theoretical understanding of the Bistrizter MacDonald Hamiltonian as well as in numerical simulations. In this work, we consider symmetries which can be written as a composition of operators from two different classes (1) Euclidean symmetries (i.e. translations, rotations, and reflections) and (2) complex conjugation. While these \kds{first few sections. (depends on how the rest of the section is written)} will focus on studying symmetries at a very abstract level, in Section \ref{sec:bm-symm} we will explicitly show how $C_{2z} \mc{T}$ and $C_{3z}$ can be realized in our parameterization of the IBM.

Given a choice of creation and annihilation operations, any symmetry operation can be completely determined by how it acts on the Fock space. For unitary symmetries, it suffices to describe how the symmetry acts on a basis of creation and annilhilation operators. In particular, for any Euclidean symmetry $g$, due to the properties of the Bloch transform, there exists a unitary $D(g)$, called the representation matrix, so that the creation operators transform via the rule
\begin{equation}
\begin{split}
    (g \hat{\vc}_{\vk}^\dag g^{-1})(\alpha) & = \sum_{\alpha'} \hat{\vc}_{g\vk}^\dag(\alpha') [D(g)]_{\alpha',\alpha} \\
    (g \hat{\vc}_{\vk} g^{-1})(\alpha) & = \sum_{\alpha'} \hat{\vc}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha}^{*}
\end{split}
\end{equation}
where $g\vk$ denotes the action of the symmetry $g$ in $\vk$-space and $\hat{\vc}_{\vk}$ are the creation operators \kds{defined in Section III}. 

In contrast to unitary symmetries, the action of complex conjugation must be defined with respect to a fixed choice of creation and annihilation operators. Throughout this section, we will define complex conjugation with respect to creation operators $\{ \hat{\vc}_{\vk}^\dag \}$ so that if $\mc{K}$ denote complex conjugation, then any linear combination of creation operators transforms as:
\begin{equation}
\begin{split}
    \mc{K} \left( \sum_{\alpha} a_{\alpha} \hat{\vc}_{\vk}^\dag(\alpha)  \right) \mc{K} =  \sum_{\alpha} a_{\alpha}^{*} \hat{\vc}_{-\vk}^\dag(\alpha) \\
    \mc{K} \left( \sum_{\alpha} a_{\alpha} \hat{\vc}_{\vk}(\alpha)  \right) \mc{K} =  \sum_{\alpha} a_{\alpha}^{*} \hat{\vc}_{-\vk}(\alpha) 
\end{split}
\end{equation}


As a first step toward studying symmetries in the Bistrizter Macdonald model, we will first show how we can write the action of $g$ in terms of its representation matrix $D(g)$. If $g$ is a unitary symmetry with corresponding representation matrix $D(g)$, then
\begin{equation}
\begin{split}
g\hat{H}_{\mathrm{BM}} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
=& \sum_{\vk} [D(g)h(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
\end{split}
\end{equation}
If $\hat{H}_{\mathrm{BM}}$ is invariant under $g$, then this calculation shows that at the matrix level:
\begin{equation}
D(g) h(\vk)=h(g\vk) D(g).
\end{equation}
In other words, 
\begin{equation}
h(g\vk)D(g)u_{n\vk}=D(g)h(\vk)u_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk},
\end{equation}
or equivalently $D(g)u_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$.

This allows us to define a ``sewing matrix'', $[B(g)]_{\vk}$,
\begin{equation}
\label{eqn:matrix_representation}
(D(g) u_{n\vk})(\alpha)=
\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}(\alpha')=
\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
\end{equation}
\kds{It is critical here that the system is gapped. If the bands are entangled, we are no longer guaranteed that $\{ \ket{u_{n,g\vk}} \}_{n \in \mc{I}}$ spans the same space as $\{ D(g) \ket{u_{n,\vk}} \}_{n \in \mc{I}}$ where $\mc{I}$ is an arbitrary index set. Not sure how to explain this...} Here 
\begin{equation}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk} | D(g) | u_{n\vk}},
\end{equation}
and $[B(g)]_{\vk}$ is a unitary matrix. \kds{Note that $D(g)$ isn't Hermitian, perhaps we should use different notation here?} \QZ{ The original representation matrix $D(g)$ is defined in the space of combined indices $\alpha$, while sewing matrix $[B(g)]_{\vk}$ is defined in the band space. It's obvious that the symmetry operation is complete using the representation matrix. Using sewing matrix, the symmetry operation is also complete when all the bands are used. In practice, the number of bands is limited. Therefore, our goal is that the symmetry operations of our interests are ``closed'' and ``complete'' using the corresponding sewing matrices: Given a set of bands $\{u_{n\vk}\}_{n,\vk}$, a)``closed'':  for any unitary/antiunitary operator $g$ of interest, $\sum_{m}  u_{m,g\vk} [B(g)]_{\vk,mn}\in\{u_{n\vk}\}_{n,\vk}$; b) ``complete'': for any $u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ and unitary (antiunitary) operator $g$ of interest, $D(g)u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ ($D(g)u^*_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$) and $D(g)u_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$ ($D(g)u^*_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$). In this note, we are particularly interested in the spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetry. In a single-valley, spinless system, one pair of flat bands with different sublattice index $\sigma=\pm$ is enough to satisfy the conditions above. More details are in Section \ref{sec:ibm-symm}}


Given the definition of sewing matrices, for unitary operator $g$, one can calculate that:
\[
\begin{split}
g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}(\alpha')\\
=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
u_{n\vk}(\alpha)\\
=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
\end{split}
\]
Hence the sewing matrices define how $\hat{f}^{\dag}_{n\vk}$ transforms under the symmetry action.

Now to turn to consider antiunitary symmetries. Since any antiunitary transformation can be written as $g \mc{K}$ where $g$ is a unitary transform and $\mc{K}$ is complex conjugation, similar calculations show that if $\hat{H}_{\mathrm{BM}}$ is invariant under an antiunitary symmetry then the corresponding matrix equation is:
\begin{equation}
D(g) h(\vk)=h(-g\vk)^* D(g).
\end{equation}
From this matrix relation, one can check that the corresponding sewing matrix can be defined by the relations:
\begin{equation}
\begin{split}
(D(g) u_{n\vk})(\alpha) & =
\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}^*(\alpha')=
\sum_{m}  u_{m,-g\vk}(\alpha) [B(g)]_{\vk,mn} \\
[B(g)]_{\vk,mn} & = \braket{u_{m,-g\vk} | D(g) | u^*_{n\vk}}.
\end{split}
\end{equation}
Using these definitions, we can now calculate how $f^\dag_{n\vk}$ transforms under antiunitary symmetry: 
\[
\begin{split}
(g \mc{K}) \hat{f}^{\dag}_{n\vk} (g \mc{K})^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}^*(\alpha')\\
=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
u_{n\vk}^*(\alpha)\\
=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,-g\vk}(\alpha') [B(g)]_{\vk,mn} \\
=& \sum_{m} \hat{f}^{\dag}_{m,-g\vk}  [B(g)]_{\vk,mn}.
\end{split}
\]



%\QZ{Maybe move the antiunitary case to the Appendix.}
%
%The case when $g$ is antiunitary is similar. 
%Here
%\begin{equation}
%\begin{split}
%g\hat{H}_{\mathrm{BM}} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
%=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]^*_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
%=& \sum_{\vk} [D(g)h^*(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
%\end{split}
%\end{equation}
%So
%\begin{equation}
%D(g) h^*(\vk)=h(g\vk) D(g).
%\end{equation}
%Hence
%\begin{equation}
%h(g\vk)D(g) u^*_{n\vk}=D(g) h^*(\vk)u^*_{n\vk}=\varepsilon^*_{n\vk} D(g)u^*_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk}.
%\end{equation}
%In other words, $D(g)u^*_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$. 
%The sewing matrix is then given by 
%\begin{equation}
%(D(g) u^{*}_{n\vk})(\alpha)=
%\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u^{*}_{n\vk}(\alpha')=
%\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
%\end{equation}
%Here 
%\[
%[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u^*_{n\vk}}
%\]
%and $[B(g)]_{\vk}$ is a unitary matrix. The transformation rule remains the same
%\begin{equation}
%\begin{split}
%g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u^*_{n\vk}(\alpha')\\
%=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
%u^*_{n\vk}(\alpha)\\
%=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
%=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
%\end{split}
%\end{equation}
%


With the transformation rule set by the sewing matrices, we can check whether a quadratic Hamiltonian 
$\hat{A}=\sum_{\vk}\sum_{mn}[A(\vk)]_{mn} \hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}$
commutes with the symmetry $g$. 
If $g\hat{A}g^{-1}=\hat{A}$, and assume that the Monkhorst-Pack grid discretizing the mBZ is invariant under $g$, then
\begin{equation}
\begin{split}
g\hat{A}g^{-1}=&\sum_{\vk}\sum_{mn} [A(\vk)]_{mn}\sum_{pq} [B(g)]_{\vk,pm} [B(g)]^*_{\vk,qn} \hat{f}^{\dag}_{p,g\vk}\hat{f}_{q,g\vk}\\
=&\sum_{g\vk} \sum_{pq} \left([B(g)]_{\vk} A(\vk) [B(g)]_{\vk}^{\dag}\right)_{pq}\hat{f}^{\dag}_{p,g\vk}\hat{f}_{q,g\vk}.
\end{split}
\end{equation}
Therefore we have the relation 
\begin{equation}
[B(g)]_{\vk} A(\vk) [B(g)]^{\dag}_{\vk}-A(g\vk)=0.
\end{equation}
Similarly, if $g$ is antiunitary, then
\begin{equation}
[B(g)]_{\vk} A^*(\vk) [B(g)]^{\dag}_{\vk}-A(-g\vk)=0.
\end{equation}

The same procedure can be used to check whether the quartic Hamiltonian commutes with $g$. \QZ{ As in \cref{eqn:subtracted_HF}, the single-particle term in the subtracted Hamiltonian is a quartic term. Therefore, the symmetries will be verified by setting $A(\vk)=h_s(\vk)$ in Section \ref{sec:ibm-symm}.}

\QZ{ For the coulomb interaction term,} due to the structure in \cref{eqn:interaction_simplify}, it is sufficient to verify that $g$ commutes with the pseudo-density operator $\hat{\rho}_{\vq}$ in \cref{eqn:rho_operator}, which is a quadratic operator.
Direct computation shows that if $g$ is unitary and commutes with $\hat{\rho}_{\vq}$,
then
\begin{equation}
[B(g)]_{\vk} \Lambda_{\vk}(\vq) [B(g)]^{\dag}_{\vk+\vq}-\Lambda_{g\vk}(g\vq)=0.
\end{equation}
If $g$ is antiunitary, then
\begin{equation}
[B(g)]_{\vk} \Lambda^*_{\vk}(\vq) [B(g)]^{\dag}_{\vk+\vq}-\Lambda_{g\vk}(g\vq)=0.
\end{equation}

Using the strategy above, we can verify that $g\hat{H}_{\mathrm{IBM}}g^{-1}=\hat{H}_{\mathrm{IBM}}$ for $g=C_{2z}\mc{T},C_{3z}$ in the continuous limit. \QZ{ More details are in Section \ref{sec:ibm-symm}.} However, in a calculation with a finite number of $\vk$ points, the symmetry may be slightly broken. 
Therefore we need to check the norm of the commutators above to verify that the magnitude of the broken symmetry is sufficiently small. \QZ{ The definition of the norm and the discussion of symmetry breaking are discussed in Section \ref{sec:symm-broken}.}



% KDS: I think what you have below is good, but the operators $\hat{\vc}$ are already defined in Section III
%\QZ{ $\hat{\vc}_{n\vk}^\dag/\hat{\vc}_{n\vk}$ is the creation/annihilation operator defined in the space of combined indices $\alpha=(\vG, s,\sigma,\tau,l)$, including the Moir\'e reciprocal lattice vector, spin, sublattice, valley, layer, and $n$ represents the unique band index. Note that the combined indices $\alpha$ and band indices $n$ are correlated with each other.} Unlike unitary symmetries, the action of complex conjugation is defined with respect to a choice of basis. Recalling


==> sections/hartree_fock.tex <==
\subsection{Hartree--Fock theory}

The Hartree--Fock approximation is the starting point for various high-accuracy electronic-structure methods~\cite{Helgaker2014}. 
The underlying assumption is that the many-body wavefunction takes the form of a Slater determinant, i.e., 
\begin{equation}
\ket{\Psi_S}=\prod_{\vk}\prod_{i\in\mathrm{occ}} b_{i\vk}^{\dag}\ket{\mathrm{vac}},
\end{equation}
where $\ket{\mathrm{vac}}$ is the vacuum state, and 
\begin{equation}
b_{i\vk}^{\dag}=\sum_{n}f_{n\vk}^{\dag} \Xi_{ni}(\vk)
\end{equation}
defines the creation operator for the Hartree--Fock orbitals for each $\vk\in\Omega^*$.
For integer filling, the number of occupied orbitals per $\vk$ point is $\nu$ (indexed by $\mathrm{occ}$). 
The 1-RDM associated with a given Slater determinant $\ket{\Psi_S}$ is then
\begin{equation}
[P(\vk)]_{nm}=\braket{\Psi_S|\hat{f}_{m\vk}^{\dagger}\hat{f}_{n\vk}|\Psi_S}=
\sum_{i\in\mathrm{occ}} \Xi_{ni}(\vk)\Xi_{mi}^*(\vk).
\end{equation}
Following the standard derivation of Hartree--Fock theory (see e.g.,~\cite{SzaboOstlund1989,MartinReiningCeperley2016}), we begin with the characterization of the Hartree--Fock energy, i.e., 
\begin{equation}
\label{eq:e_hf}
E_{\rm HF}
=
\min_{P\in \mathcal{M}}{\rm Tr}[PH],
\end{equation}
where $\mathcal{M}$ is the set of 1-RDMs associated with the possible single Slater determinants of the system.
A common way to seek the solution to Eq.~\eqref{eq:e_hf} is by finding a stationary point, which is equivalent to diagonalizing the Fock operator~\cite{SzaboOstlund1989}, i.e., 
\begin{equation}
\hat{F}[P]=\hat{H}_0+ \hat{J}[P] - \hat{K}[P]= \hat{H}_0+ \hat{V}_{HF}[P].
\end{equation}
We here employ quantum chemistry notation where $H_0$ is the core Hamiltonian, $\hat{J}[\cdot]$ and $\hat{K}[\cdot]$ are the Coulomb and exchange operator, respectively, and $\hat{V}_{HF}[\cdot]$ is the Hartree--Fock potential.
This non-linear eigenvalue problem is determined by self-consistently evaluating the 1-RDM~\cite{Lehtola2020}.

For an explicit definition of the Coulomb term, we apply Wick's theorem to the interaction term~\eqref{eqn:interaction_simplify}, and use the relation in \cref{eqn:average_f}. 
This yields
%can be obtained using , which replaces $\hat{\rho}_{-\vq}$ by its mean-field %average. Replacing $\hat{\rho}_{\vq}$ by its mean-field average gives an %identical contribution, which cancels the factor $\frac12$ in the interaction %Hamiltonian.
%The Hartree potential is 
% \begin{equation}
% \begin{split}
% \hat{H}_{\mathrm{h}}[P]=&\frac{1}{ |\Omega|} 
% \sum_{\vq} V(\vq)\hat{\rho}_{\vq}\frac{1}{N_{\vk}}\braket{\Psi_S|\hat{\rho}_{-\vq}|\Psi_S}\\
% =&\frac{1}{|\Omega|} 
% \sum_{\vG} V(\vG)\hat{\rho}_{\vG} \left(\frac{1}{N_{\vk}}\sum_{\vk'\in \Omega^*} \Tr[ \Lambda_{\vk'}(-\vG) P(\vk')]\right)\\
% =:&\frac{1}{|\Omega|} 
% \sum_{\vG} V(\vG)\hat{\rho}_{\vG} \varrho(-\vG).
% \end{split}
% \end{equation}
%\kds{I think $\Lambda_{k'}$ needs a transpose above?}

\begin{equation}
\label{eq:Coulomb_op_long}
\begin{split}
\hat{J}[P]=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}
\\
&
\times \left(\braket{\Psi_S|\hat f_{m\vk}^{\dagger}\hat f_{n(\vk+\vq')}|\Psi_S} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq')}+ \braket{\Psi_S|\hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq')}|\Psi_S} \hat f_{m\vk}^{\dagger}\hat f_{n(\vk+\vq')}\right)\\
=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}\\
&
\times \sum_{\vG\in\mathbb{L}^*} \left([P(\vk)]_{nm}\delta_{\vq',-\vG}\hat f_{m'\vk'}^{\dagger} \hat f_{n'\vk'}+[P(\vk')]_{n'm'}\delta_{\vq',\vG}\hat f_{m\vk}^{\dagger}\hat f_{n\vk}\right)\\
=&\frac{1}{|\Omega|} 
\sum_{\vG\in\mathbb{L}^*} V(\vG)\left(\frac{1}{N_{\vk}}\sum_{\vk'\in \Omega^*} \Tr[ \Lambda_{\vk'}(-\vG) P(\vk')]\right)\left(\sum_{\vk\in \Omega^*} \sum_{mn} [\Lambda_{\vk}(\vG)]_{mn}\hat f_{m\vk}^{\dagger}  \hat f_{n\vk}\right).
\end{split}
\end{equation}
In the last step we have used the fact that $V(\vq')=V(-\vq')$. 
To simplify the expression in Eq.~\eqref{eq:Coulomb_op_long}, we can define the electron density $\wt{\rho}$, i.e., 
\begin{equation}
\wt{\rho}[P](\vG)=\frac{1}{N_{\vk}} 
\sum_{\vk'\in \Omega^*}\Tr[ \Lambda_{\vk'}(\vG) P(\vk')],
\end{equation}
which is periodic with respect to the moir\'e unit cell.  
Using the definition of the pseudo-density operator in~\cref{eqn:rho_operator}, the expression of the Coulomb operator can be simplified into the standard density--density form 
\begin{equation}
\hat{J}[P]=\frac{1}{|\Omega|} \sum_{\vG} V(\vG) \wt{\rho}[P](-\vG)\hat{\rho}_{\vG}.
\end{equation}


We proceed similarly for the exchange operator; using Wick's theorem yields
\begin{equation}
\begin{split}
\hat{K}[P]=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}
\\
&
\times\left(\braket{\Psi_S|\hat f_{m\vk}^{\dagger}\hat f_{n'(\vk'-\vq')}|\Psi_S} \hat f_{m'\vk'}^{\dagger}\hat f_{n(\vk+\vq')} + \braket{\Psi_S|\hat f_{m'\vk'}^{\dagger}\hat f_{n(\vk+\vq')}|\Psi_S} \hat f_{m\vk}^{\dagger}\hat f_{n'(\vk'-\vq')}\right)\\
=&
\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [\Lambda_{\vk'}(-\vq')]_{m'n'}\\
&
\times \sum_{\vG\in\mathbb{L}^*} \left([P(\vk)]_{n'm}\delta_{\vk,\vk'-\vq'+\vG}
\hat f_{m'\vk'}^{\dagger}\hat f_{n(\vk+\vq')}+[P(\vk')]_{nm'}\delta_{\vk',\vk+\vq'+\vG}
\hat f_{n'(\vk'-\vq')}\right)\\
=&
\frac{1}{ |\Omega| N_{\vk}} \sum_{\vq'}\sum_{\vk\in \Omega^*}
\sum_{mm'nn'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn} [P(\vk+\vq')]_{nm'}[\Lambda_{\vk+\vq'}(-\vq')]_{m'n'}
\hat f_{m\vk}^{\dagger}\hat f_{n'\vk}. 
\end{split}
\end{equation}
In summary, the Hartree--Fock potential can be written as
\begin{equation}
\hat{V}_{\mathrm{HF}}[P]
=\hat{J}[P]- \hat{K}[P]
=\sum_{\vk\in \Omega^*} \hat f_{m\vk}^{\dagger}[v_{\mathrm{hf}}[P](\vk)]_{mn}
\hat f_{n\vk},
\end{equation}
where
\begin{equation}
\label{eq:hf-rho}
\begin{split}
[v_{\mathrm{hf}}[P](\vk)]_{mn}=&\frac{1}{|\Omega|} 
\sum_{\vG\in\mathbb{L}^*} V(\vG) \left(\frac{1}{N_{\vk}}\sum_{\vk'\in \Omega^*} \Tr[ \Lambda_{\vk'}(-\vG) P(\vk')]\right)[\Lambda_{\vk}(\vG)]_{mn}\\
&-\frac{1}{ |\Omega| N_{\vk}} \sum_{\vq'} \sum_{m'n'}
 V(\vq') [\Lambda_{\vk}(\vq')]_{mn'} [P(\vk+\vq')]_{n'm'}[\Lambda_{\vk+\vq'}(-\vq')]_{m'n}.
\end{split}
\end{equation}

% 
% Note that BM bands are different from HF bands here. $\hat{f}^{\dagger}_{n\vk}$ represents the creation operator corresponding to the BM band basis $u_{n\vk}=\hat{f}^{\dagger}_{n\vk}\ket{0}$, where $u_{n\vk}$ is an eigenfunction of the first quantized single-particle Hamiltonian $h(\textbf{k})$ with the eigenvalue $\epsilon_{n\textbf{k}}$. In Section \ref{sec:symm}, the projected Hamiltonian will be discussed and we will perform the change of basis on the creation/annihilation operators:
% \[
% \hat{\vf}^{\dag}_{m\vk} \to \sum_{n} [U(\vk)]_{mn} \hat{\vf}^{\dag}_{n\vk}.
% \]
% 
% On the other hand, $\ket{\Psi}$ represents the many-body wavefunction, which is a Slater determinant constructed from HF bands. In general, BM band basis is used to project the IBM Hamiltonian onto flat bands and it's generated from BM Hamiltonian, while HF solution is tested to see the spontaneous symmetry-broken and it's the ground state of IBM Hamiltonian.



\subsection{Subtraction Hamiltonian}\label{sec:subtraction}
 
%In order to observe the spontaneous symmetry breaking, we need to discuss the existence of symmetries in IBM model. Before the symmetry checking in Section~\ref{sec:symm}, we introduce 

%Using the Hartree--Fock potential, we can define the subtraction Hamiltonian in the quadratic part of the IBM model in \cref{eqn:ibm_quadratic}. 
Since the BM band energies already take the electron--electron interaction between the two layers of graphene into account, the double gate-screened Coulomb potential in the IBM model double counts said interactions.
As a remedy, Bultinck et al~\cite{BultinckKhalafLiuEtAl2020} have introduced $v_{\mathrm{hf}}[P^0](\vk)$, see Eq.~\cref{eq:hf-rho}, for a given reference density $P^0$ as the subtraction Hamiltonian $h_{\mathrm{sub}}(\vk)$.
Combining \cref{eqn:IBM_Ham,eqn:ibm_quadratic}, the IBM model is well-defined.
In particular, since the mapping $P \mapsto v_{\mathrm{hf}}[P]$ is linear, the Hartree--Fock Hamiltonian can be written as

% In \cite{BultinckKhalafLiuEtAl2020}, a subtraction Hamiltonian $h_{\mathrm{sub}}(\vk)$ is introduced to cancel out such effects at the Hartree--Fock level, defined as the Hartree--Fock potential \cref{eq:hf-rho} with respect to a reference density $P^0$, i.e., $h_{\mathrm{sub}}(\vk)=h_{\mathrm{hf}}[P_0](\vk)$. 
% Combining \cref{eqn:IBM_Ham,eqn:ibm_quadratic}, the IBM model is well defined. In particular, since the mapping $P \mapsto v_{\mathrm{hf}}[P]$ is linear, the Hartree--Fock Hamiltonian can be written as
\begin{equation}
\label{eqn:subtracted_HF}
\sum_{\vk\in\rm{mBZ}}\sum_{mn}\hat f^{\dagger}_{m\vk}[h_{\mathrm{BM}}(\vk)]_{mn}
\hat f_{n\vk} + \hat{V}_{\mathrm{HF}}[\delta P(\vk)],
\end{equation}
where $\delta P(\vk)=P(\vk)-P^{0}(\vk)$.



%\LL{ the following sentence should appear in the symmetry section?} Several special choices are discussed here to enforce different symmetries, such as particle-hole symmetry $\mc{P}$. 


% Given the reference density $P^0$, the quadratic subtraction Hamiltonian is defined as the Hartree--Fock potential  and
% 
% \begin{equation}
% \label{eqn:subtraction}
% \begin{split}
% h^0_s[P^0](\vk)= \frac{1}{|\Omega|N_{\vk}} 
% [&\sum_{\vG} V(\vG)\Lambda_{\vk}(G) \sum_{\vk'} \Tr[ \Lambda_{\vk'}(-\vG) P^0(\vk')] \\
% &-\sum_{\vG,\vq}V(\vG+\vq)\Lambda_{\vk}(\vq) P^0(\vk+\vq)\Lambda_{\vk+\vq}(-\vq)].
% \end{split}
% \end{equation}

% The single-particle Hamiltonian is then changed into $h(\vk)-h_s^0[P^0](\vk)$ and the corresponding Hartree--Fock Hamiltonian is
% \begin{equation}
% \begin{split}
% \label{eqn:subtracted_HF}
% \hat H_{HF}=&\sum_{\vk\in\rm{mBZ}}\hat f^{\dagger}_{\vk}[h(\vk)-h_s^0[P^0](\vk)]\hat f_{\vk} + \hat{H}_{\mathrm{h}}[P(\vk)]+\hat{H}_{\mathrm{f}}[P(\vk)],\\
% =&\sum_{\vk\in\rm{mBZ}}\hat f^{\dagger}_{\vk}h_s(\vk)\hat f_{\vk} + \hat{H}_{\mathrm{h}}[\delta P(\vk)]+\hat{H}_{\mathrm{f}}[\delta P(\vk)],
% \end{split}
% \end{equation}
% where $\delta P(\vk)=P(\vk)-\frac12I$, $\delta P^0(\vk)=P^0(\vk)-\frac12I$ and $h_s(\vk)=h(\vk)-h_s^0[\delta P^0](\vk)$. We further assume that $P^0(\vk)$ is a neutral projector arising from a $C_{2z}\mc{T}$ symmetric
% Hamiltonian, then the first term in \cref{eqn:subtraction} vanished for half-filling system (see Appendix~\ref{sec:supp}) and the subtracted single-particle Hamiltonian is
% \begin{equation}
% h_s(\vk)=h(\vk)+\frac{1}{|\Omega|N_{\vk}}\sum_{\vG,\vq}V(\vG+\vq)\Lambda_{\vk}(\vq) \delta P^0(\vk+\vq)\Lambda_{\vk+\vq}(-\vq).
% \end{equation}

Following \cref{eqn:1rdm}, $P^0(\vk)$ should be interpreted as the coefficients of the reference density matrix in the BM band basis.
The choice of a reference density matrix $P^0(\vk)$ is not unique and should also be viewed as part of the IBM model.
For instance, in Ref.~\cite{BernevigSongRegnaultEtAl2021}, the choice is $P^0(\vk)=\frac{1}{2}I$, which is called the \textit{average scheme}. 
In Ref.~\cite{BultinckKhalafLiuEtAl2020},\LL{ Mike/Tomo: cite the relevant papers from MacDonald's group?}  $P^0(\vk)$ is obtained by projecting the zero temperature limit of the density matrix corresponding to two decoupled graphene layers to the BM band basis of the TBG system. This is referred to as the \textit{decoupled scheme}. 
It is worth mentioning that in the decoupled scheme, the number of BM bands should be sufficiently large to preserve the trace of $P^0$ after the projection. The zero temperature limit ensures that $P^0$ is uniquely defined even if some of the band energies of the two decoupled graphene layers may become degenerate. Furthermore, the choice of $P^0$ does not change with respect to the filling factor $\nu$. \LL{ Mike/Tomo: can you add justification for the usage of exactly the same subtraction density matrix for non-integer fillings?}
Unless otherwise specified, we adopt the decoupled scheme in all the numerical results.
 


% In our implementation, without further notice, average scheme is used since it gives rise to the particle-hole symmetry $\mc{P}$ in the interaction term\cite{TBGIII}, preserves both $C_{2z}\mc{T}$ and $C_{3z}$ symmetry of our interests. The numerical difference between different schemes will also be discussed in \ref{sec:numerical}. 


==> sections/ibm_model.tex <==

\begin{figure*}
\begin{center}
\begin{subfigure}[c]{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/tbg_layers.pdf} 
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/mbz_num_lat.pdf} 
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/flat_bands.png}
\end{subfigure}
\begin{subfigure}[c]{.3\textwidth}
    \caption{}
    \label{fig:tbg_layers}
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \caption{}
    \label{fig:mbz_num_lattice}
\end{subfigure}
\hfill
\begin{subfigure}[c]{.3\textwidth}
    \caption{}
    \label{fig:flat_bands}
\end{subfigure}
\end{center}
\caption{
\FF{Note the hack! I did not know how to vertically align the figure and have the captions (a), (b), (c) at the bottom. Format fine tuning has to be done at some point.}
(\subref{fig:tbg_layers}) The graphic shows two monolayer graphene Brillouin zones (BZ) in red and blue, respectively, aligned by their $\Gamma$-point and twisted by an angle $\Theta$. 
The Dirac points of the individual layers are denoted by $K^+$ and $K^-$ for the red and blue BZ, respectively. 
Moreover, the graphic shows the corresponding moir\'e Brillouin zone of the twisted bilayer graphene shaded in grey and the $\Gamma$-point of the mBZ denoted $\Gamma_{\rm mBZ}$. 
(\subref{fig:mbz_num_lattice}) The graphic shows three mBZ. Furthermore, it shows the numerical $k$ grid encircle by the green dashed line. 
This rectangular choice of the mBZ $k$ grid follows the grid in Ref.~\cite{SoejimaParkerBultinckEtAl2020}
The Dirac points of the individual graphene layers $K^+$ and $K^-$ red and blue, respectively, are included as reference. 
(\subref{fig:flat_bands}) The graphic shows the band structure of the BM Hamiltonian in the mBZ, with the corresponding flat bands (red lines) and remote bands (grey lines). The interacting BM Hamiltonian is then projected onto the two flat band space (note that the labels should not touch the graphs).
\FF{Graphic (c) needs to be improved}
\LL{ I agree. A few more minor changes: 1) the fonts should be larger and lines should be thicker. 2) Not sure what the two vectors are for in the middle figure (we never used $Q_1,Q_2$. We should also say that the rectangular choice of the mBZ follows that in \cite{SoejimaParkerBultinckEtAl2020}. 3) The $\Gamma$ point in the rightmost figure should be $\Gamma_M$?}
}
\end{figure*}

% \begin{figure*}
% \centering
% \begin{subfigure}[b]{.74\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/mBZ.png} % KDS: The size of the subfigure is set to .74\textwidth above, \linewidth takes this change into account which is why it's \linewidth not .74\linewidth. 
%     \caption{}
%     \label{fig:mbz-picture}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/flat_bands.png}
%     \caption{}
%     \label{fig:flat_bands}
% \end{subfigure}
% \caption{(\subref{fig:mbz-picture}) Two monolayer graphene Brillouin zones twisted by an angle $\theta$ and the corresponding Moir\'e Brillouin zone of the twisted bilayer graphene. Zoomed view of the Moir\'e BZ shows the numerical $k$ grids using green dash. (\subref{fig:flat_bands}) The band structure of the BM Hamiltonian in the Moir\'e BZ, with the corresponding flat bands (red lines) and remote bands (grey lines). The interacting BM Hamiltonian is then projected onto the flat band space. \kds{Not an immediate issue but the y label in (b) is cut off}
% \FF{Maybe use three Figures (a), (b), and (c) to make this cleaner? What about a slight rephrasing: (a) The graphic shows two monolayer graphene Brillouin zones (in red and blue, respectively) aligned by their $\Gamma$-point and twisted by an angle $\theta$ ($\Theta$ should be larger in the Figure). The Dirac points of the individual layers are denoted by $K^+$ and $K^-$ for the red and blue BZ, respectively. Moreover, the graphic shows the corresponding Moir\'e Brillouin zone (mBZ) of the twisted bilayer graphene and the $\Gamma$-point of the mBZ ($\Gamma_M$). (b) The graphic shows three mBZ and the mBZ lattice vectors. Furthermore, it shows the numerical $k$ grid encircle by the green dashed line. (c) The graphic shows the band structure of the BM Hamiltonian in the mBZ, with the corresponding flat bands (red lines) and remote bands (grey lines). The interacting BM Hamiltonian is then projected onto the two flat band space (note that the labels should not touch the graphs).}\LL{ I agree. A few more minor changes: 1) the fonts should be larger and lines should be thicker. 2) Not sure what the two vectors are for in the middle figure (we never used $Q_1,Q_2$. We should also say that the rectangular choice of the mBZ follows that in \cite{SoejimaParkerBultinckEtAl2020}. 3) The $\Gamma$ point in the rightmost figure should be $\Gamma_M$?}
% }
% %\QZ{ somehow subcaption package doesn't work}}
% \end{figure*}



% 
% 
% 
% We first present a review of the monolayer and bilayer graphene to define our notations. Single layer graphene is a 2D structure with honeycomb lattice and it consists of a bipartite lattice of two triangular sublattices $\sigma=A/B$. Single layer graphene also has two Dirac points $\pm K$ in the single layer Brillouin zone and these two Dirac points are connected by the time-reversal symmetry. This two Dirac points are labelled with valley index $\pm1$ and equipped with the valley operator $\tau$. Then the twisted bilayer grapehene has two layers of graphene twisted by a small angle $\theta$ and this two layers are perfectly stacked with each other at one $AA$ lattice. When the twisted angle is small, each layer $l=\pm$ has two Dirac points $\pm K_{l}$ and the valley in the top layer is only coupled with the same valley in the bottom layer with a Moir\'e interlayer potential. The hopping parameters $w_0$ and $w_1$ represent the $AA$ hopping and $AB/BA$ hopping respectively. The original BM model has equal $AA$ and $AB/BA$ hopping with $w_0=w_1$. At the chiral limit $w_0=0$, $AA$ hopping is turned off and it gives us the exact zero flat bands.\cite{nam_2017}
% The special geometry and rich symmetries of graphene enable the unique band structure and interesting electronic phenomenon. In particular, there exist isolated flat bands in the BM band structure. Using these flat bands, we will introduce the projected IBM Hamiltonian with a double-gate screened Coulomb interaction. 

Unless otherwise specified, we restrict to the flat bands labeled by $n\in\{1,2\}$ \kds{I don't think choosing $n \in \{ 1,2 \}$ really makes sense here; we haven't defined what the band indexing is}\LL{ We talked about that (briefly) in the previous section? Please feel free to change.}  whose band energies are separated from the remaining band spectrum, as in Figure~\ref{fig:flat_bands}.
Throughout the discussion below, the band indices $m,n$ refer to the flat bands only. 
The Hamiltonian of the IBM model for the flat bands takes the form
\begin{equation}
\begin{split}
\hat{H}_{\mathrm{IBM}}
=& \hat{H}_0+\hat{H}_I\\
=&\sum_{\vk\in \Omega^*} \sum_{mn}\hat f_{m\vk}^{\dagger} [h(\vk)]_{mn} \hat f_{n\vk}\\
&+\frac{1}{2}
\sum_{\substack{\vk,\vk',\vk''\in \Omega^*\\\vk''' = \vk+\vk'-\vk''}} \sum_{mm'nn'}\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}\hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'\vk'''} \hat f_{n\vk''},
\end{split}
\label{eqn:IBM_Ham}
\end{equation}
%\kds{It looks a bit gross, but I added the crystal momentum conservation condition on $\vk'''$ in the sum above. At least for me, this significantly clarifies the discussion below}
where $\hat{H}_0$ and $\hat{H}_I$ are the quadratic term and the quartic term, respectively. 
The ground state of the IBM model is then defined as the solution to the eigenvalue problem
\begin{equation}
E_0=\min_{\substack{\ket{\Psi}\in\mc{F}, ~\braket{\Psi|\Psi}=1\\\braket{\Psi|\hat{N}|\Psi}=N_e}} \quad \braket{\Psi|\hat{H}|\Psi},
\end{equation}
where $N_e=\nu N_{\vk}$ is the total number of electrons, and $\hat{N}=\sum_{\vk}\sum_{n} \hat f_{n\vk}^{\dagger} \hat f_{n\vk}$ is the total number operator.
The number of electrons per $\vk$ point is denoted by $\nu$, called the \textit{filling factor}. 
Since there are only two bands per $\vk$ point, the only non-trivial integer value for the filling factor is $\nu=1$, which is called the half-filling case (or the particle-hole symmetric case) of the IBM model in the spin-less, valley-less regime.

The main object of interest in this work is the one-particle reduced density matrix (1-RDM) corresponding to the ground state $\ket{\Psi}$ defined as
\begin{equation}
\label{eqn:1rdm}
[P(\vk)]_{nm}=\braket{\Psi|\hat{f}_{m\vk}^{\dagger}\hat{f}_{n\vk}|\Psi}.
\end{equation}
We emphasize that the 1-RDM is well-defined in the entire moir\'e reciprocal space due to the periodic extension in \cref{eqn:period_f}.
Using the 1-RDM, we find that for any $\vk,\vk'$ in the moir\'e reciprocal space,
\begin{equation}
\braket{\Psi|\hat{f}_{m\vk}^{\dagger}\hat{f}_{n\vk'}|\Psi}
=P(\vk)\sum_{\vG\in\mathbb{L}^*}\delta_{\vk,\vk'+\vG}.
\label{eqn:average_f}
\end{equation}

The quartic term $\hat{H}_I$ describes the (screened) Coulomb interaction via the two electron repulsion integrals (ERI) denoted by $\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}$.
The coefficients of the quadratic term can be written as
\begin{equation}
h(\vk)=h_{\mathrm{BM}}(\vk)-h_{\mathrm{sub}}(\vk),
\label{eqn:ibm_quadratic}
\end{equation}
where $[h_{\mathrm{BM}}(\vk)]_{mn}=\varepsilon^{\mathrm{BM}}_n(\vk) \delta_{mn}$ is given by the BM band energy. The second term $h_{\mathrm{sub}}(\vk)$ is called the subtraction Hamiltonian, which removes the double counting of the Coulomb interaction within the flat bands, and is defined in terms of the Hartree--Fock potential. We focus on the Coulomb interaction term first and postpone the discussion of $h_{\mathrm{sub}}(\vk)$ to \cref{sec:subtraction}.

In the Coulomb interaction term, the summation is only over $\vk,\vk',\vk''\in\Omega^*$. This is due to the crystal momentum conservation, i.e., $\vk+\vk'-\vk''-\vk'''=\bm{0}$.
Here we follow the convention that the fourth momentum vector $\vk'''=\vk+\vk'-\vk''$ may be outside $\Omega^*$
\footnote{Many practical implementation restrict $\vk'''$ to be within the mBZ as well, and hence the crystal momentum conservation condition becomes $\vk+\vk'-\vk''-\vk'''=\vG$ for some $\vG\in\mathbb{L^*}$. We do not use this convention in this paper.}.
Another way to express the crystal momentum conservation condition is to write $\vk''=\vk+\vq$, $\vk'''=\vk'-\vq$. 
Note that in this convention, both $\vq$ and $\vk'''$ may be outside the mBZ.


In TBG, the flat bands not only interact via a screened Coulomb interaction (the screening is modeled by a dielectric constant $\epsilon$), but also feels the Coulomb screening from the top and bottom metallic gates.\FF{This is a weird phrase.}
\LL{ Mike/Tomo: what is a good reference to cite a picture for this double-gate setup for TBG?} Assume that the TBG sample is placed in a $x$\nobreakdash-$y$~plane that is of distance $d/2$ to the top and bottom metallic gate plates along the $z$ direction. 
Since the moir\'e length scale is much larger than the distance between the sublattice sites and the layers, we may assume that the Coulomb interaction depends only on the difference $\delta r= \vr-\vr'$, and does not depend on the sublattice and layer indices. 
The screened Coulomb interaction in the real space (called a double gate-screened Coulomb potential) can be written as
\begin{equation}
V(\vr)=U_{d} \sum_{n=-\infty}^{\infty} \frac{(-1)^{n}}{\sqrt{\abs{\vr}^2+(nd)^{2}}}.
\end{equation}
%Here $U_d=\frac{e^2}{4\pi\epsilon_0 \epsilon}$ is the interaction strength.
Here, $U_d=\epsilon^{-1}$ describes the strength of the screened Coulomb interaction. In the Fourier space, the Coulomb interaction takes the form
\begin{equation}
V(\vq)=\int V(\vr) e^{-\I \vq \cdot \vr}\ud \vr=2\pi U_d\frac{\tanh(\abs{\vq}d/2)}{\abs{\vq}},
\label{eqn:doublegate_q}
\end{equation}
see \cite[Appendix C]{BernevigSongRegnaultEtAl2021} for more details.
Note that under slight abuse of notation we here use $V(\vq)$ to denote the Fourier transform of $V(\vr)$).

The ERI take the form
\begin{equation}
\begin{split}
&\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}\\
\qquad&=\frac{1}{N_{\vk}^2}\sum_{\sigma,l,\sigma',l'}\int V(\vr-\vr')\psi^{*}_{m\vk}(\vr,\sigma,l)
\psi^{*}_{m'\vk'}(\vr,\sigma',l')\psi_{n\vk''}(\vr,\sigma,l)
\psi_{n'\vk'''}(\vr,\sigma',l') \ud \vr \ud \vr'\\
\qquad&=\frac{1}{N_{\vk}^2}
\,\int V(\vr-\vr') e^{\I \vq\cdot (\vr-\vr')}\varrho_{m\vk,n(\vk+\vq)}(\vr) \varrho_{m'\vk',n'(\vk'-\vq)}(\vr')\ud \vr \ud \vr',
\end{split}
\label{eqn:eri_realspace}
\end{equation}
Note that the integration is performed in the moir\'e supercell.
The pair product of the periodic components of the BM bands in the real space (summed over the sublattice and layer indices) is defined as
\begin{equation}
\varrho_{m\vk,n\vk''}(\vr)
=\sum_{\sigma,l}u^*_{m\vk}(\vr,\sigma,l)  u_{n\vk''}(\vr,\sigma,l).
\end{equation}
Expanding the periodic Bloch functions in terms of their Fourier coefficients, the pair product can be written as
\begin{equation}
\label{eq:pair-product}
    \varrho_{m\vk,n\vk''}(\vr) = \frac{1}{|\Omega|^2} \sum_{\vG, \vG' \in \mathbb{L}^*} \sum_{\sigma,l}u^*_{m\vk}(\vG,\sigma,l)  u_{n\vk''}(\vG',\sigma,l) e^{i (\vG' - \vG) \cdot r}.
\end{equation}
Recall that by definition of the periodic Bloch functions $\psi_{n\vk''}(\vr) = \psi_{n,(\vk'' + \vG)}(\vr)$ for all $\vG \in \mathbb{L}^*$.
Therefore, $u_{n\vk''}(\vr) = e^{i \vG \cdot \vr} u_{n,(\vk''+\vG)}(\vr)$ and consequently, 
% Observe that since for all $\vG \in \mathbb{L}^*$, $\psi_{n\vk''}(\vr) = \psi_{n,(\vk'' + \vG)}(\vr)$ by the definition of the periodic Bloch functions it is also true that $u_{n\vk''}(\vr) = e^{i \vG \cdot \vr} u_{n,(\vk''+\vG)}(\vr)$. 
% As a consequence of this 
\begin{equation}
\begin{split}
    & u_{n\vk''}(\vr) = e^{i \vG \cdot \vr} u_{n,(\vk''+\vG)}(\vr) \\[1ex]
    & \Rightarrow \sum_{\vG'} u_{n\vk''}(\vG') e^{i \vG' \cdot \vr} =  \sum_{\vG'} u_{n,(\vk''+\vG)}(\vG') e^{i (\vG' + \vG) \cdot \vr} \\[1ex]
    & \Rightarrow u_{n\vk''}(\vG') = u_{n,(\vk''+\vG)}(\vG' - \vG).
\end{split}
\end{equation}
Hence, 
\begin{equation}
    \varrho_{m\vk,n\vk''}(\vr) = \frac{1}{|\Omega|^2} \sum_{\vG, \vG' \in \mathbb{L}^*} \sum_{\sigma,l}u^*_{m\vk}(\vG,\sigma,l)  u_{n,\vk''+\vG}(\vG' - \vG,\sigma,l) e^{i (\vG' - \vG) \cdot r}.
\end{equation}
The Fourier coefficients of the pair product then satisfy
\begin{equation}
\varrho_{m \vk,n(\vk+\vq)}(\vG)=\frac{1}{\abs{\Omega}}
\sum_{\vG'\in\mathbb{L}^*} \sum_{\sigma,l}u^*_{m\vk}(\vG',\sigma,l) u_{n(\vk+\vq+\vG)}(\vG',\sigma,l)=[\Lambda_{\vk}(\vq+\vG)]_{mn},
\label{eqn:form_factor}
\end{equation}
where the matrix $\Lambda_{\vk}(\vq+\vG)$ is called the \textit{form factor}.
Note that due to a shift in $\vG$, the Fourier coefficients of the pair product can be written as an inner product opposed to the convolution that arises directly from Eq.~\eqref{eq:pair-product}.

From \cref{eqn:form_factor} we can verify that the form factor satisfies the symmetry condition
\begin{equation}
[\Lambda_{\vk}(\vq+\vG)]^*_{mn}=[\Lambda_{\vk+\vq}(-\vq-\vG)]_{nm}.
\label{eqn:form_factor_symmetry}
\end{equation}

Using the definitions of the Coulomb interaction $V(\vq)$ in Eq.~\ref{eqn:doublegate_q} and the form factor in Eq.~\eqref{eqn:form_factor}, the ERI can be expressed in the Fourier space as
\begin{equation}
\begin{split}
\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}=&\frac{1}{|\Omega| N_{\vk}} \sum_{\vG\in \mathbb{L}^*} V(\vq+\vG) \varrho_{m\vk,n(\vk+\vq)}(\vG)
\varrho_{m'\vk',n'(\vk'-\vq)}(-\vG)\\
=&\frac{1}{|\Omega| N_{\vk}} \sum_{\vG\in \mathbb{L}^*} V(\vq+\vG)  [\Lambda_{\vk}(\vq+\vG)]_{mn} [\Lambda_{\vk'}(-\vq-\vG)]_{m'n'}.
\end{split}
\label{eqn:IBM_ERI}
\end{equation}
Compared to \cref{eqn:eri_realspace}, we gained an extra factor $N_\vk$ due to the integration in the moir\'e supercell.
Hence, the interaction Hamiltonian is fully determined by the form factor and the screened Coulomb potential as
\begin{equation}
\begin{split}
\hat{H}_I=&\frac{1}{2} 
\sum_{\vk,\vk',\vk''\in \Omega^*}\sum_{mm'nn'}\braket{m\vk, m'\vk'|n\vk'', n' \vk'''}\hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'\vk'''} \hat f_{n\vk''}\\
=& \frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk',\vk+\vq=\vk''\in  \Omega^*}\sum_{mm'nn'}
\sum_{\vG\in \mathbb{L}^*} V(\vq+\vG) \braket{u_{m\vk}|u_{n(\vk+\vq+\vG)}}\\
&
\times\braket{u_{m'\vk'}|u_{n'(\vk'-\vq-\vG)}} \hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq)} \hat f_{n(\vk+\vq)}\\
=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk',\vk+\vq=\vk''\in \Omega^*}\sum_{mm'nn'}
\sum_{\vG\in \mathbb{L}^*} V(\vq+\vG) [\Lambda_{\vk}(\vq+\vG)]_{mn}
\\
&
\times[\Lambda_{\vk'}(-\vq-\vG)]_{m'n'} \hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq)} \hat f_{n(\vk+\vq)}.
\end{split}
\label{eqn:interaction_comput}
\end{equation}
This can be further simplified by treating $\vq+\vG$ as a new variable $\vq'$, which takes the value from the entire reciprocal space.
Using \cref{eqn:period_f}, we have
\begin{equation}
\begin{split}
\hat{H}_I=&\frac{1}{2 |\Omega| N_{\vk}} \sum_{\vk,\vk'\in \Omega^*}\sum_{mm'nn'}
\sum_{\vq'} V(\vq') [\Lambda_{\vk}(\vq')]_{mn}
\\
&
\times [\Lambda_{\vk'}(-\vq')]_{m'n'} \hat f_{m\vk}^{\dagger} \hat f_{m'\vk'}^{\dagger} \hat f_{n'(\vk'-\vq')} \hat f_{n(\vk+\vq')}.
\end{split}
\end{equation} 
Defining a pseudo density operator
\begin{equation}
\hat{\rho}_{\vq}=\sum_{\vk\in \Omega^*} \sum_{mn} \hat f_{m\vk}^{\dagger} [\Lambda_{\vk}(\vq)]_{mn} \hat f_{n(\vk+\vq)},
\label{eqn:rho_operator}
\end{equation}
and using the normal ordering, i.e.,
\begin{equation}
:f_{m\vk}^{\dagger}  \hat f_{n(\vk+\vq)}f_{m'\vk'}^{\dagger}  \hat f_{n'(\vk'-\vq)}:\,
=f_{m\vk}^{\dagger}  f_{m'\vk'}^{\dagger}  \hat f_{n'(\vk'-\vq)}\hat f_{n(\vk+\vq)},
\end{equation}
we can further simplify $\hat{H}_I$ to 
\begin{equation}
\hat{H}_I=\frac{1}{2 \abs{\Omega}N_{\vk}} 
\sum_{\vq'} V(\vq'):\hat{\rho}_{\vq'}\hat{\rho}_{-\vq'}:.
\label{eqn:interaction_simplify}
\end{equation}
This form is reminiscent of the density--density Coulomb interaction in the reciprocal space. 
% \kds{Maybe bring this simplification up later? (in the symmetries section when we use it as part of the calculation?) I think keeping in this way will make it easier for people to compare to previous works} \LL{ Where do you think this should appear?} \kds{This formulation is better for the derviation of the HF theory so I think this is the right place to put it.}
The expression \eqref{eqn:interaction_simplify} has certain conceptual advantages, e.g., when writing down the Hartree--Fock potential, and to verify the symmetries of $\hat{H}_I$ in \cref{sec:symm_ham}. However, it does not simplify the implementation efforts compared to \cref{eqn:interaction_comput}.


==> sections/introduction.tex <==
\QZ{I am open to any advice in the introduction section.}\\
\FF{Maybe add a more general section introducing TBG here.}

The symmetry-breaking insulating phase is crucial in the superconductors\FF{This seems very general, and I am not sure if this is true. Maybe you can add a reference where this is stated?}, such as twisted bilayer graphene (TBG). At the first magic angles, twisted bilayer graphene has the extreme flat band structure, which gives rise to strongly-correlated interaction states and the corresponding superconductivity at charge neutrality.\cite{cao_2018,cao2_2018,lu_2019,yankowitz_2019} 
\FF{Maybe one can rephrase a bit like:
At the first magic angles, TBG exhibits a surprisingly flat band structure that gives rise to strongly-correlated interaction states and the experimentally observed superconductivity~\cite{cao_2018,cao2_2018,lu_2019,yankowitz_2019}.
}
On one hand, the isolation and degeneracy of the Moir\'e flat bands enable the implementation of the mean field method in the band space without breaking the symmetries.\cite{TBGIII,bultinck_2020,soejima_2020,TBGII} On the other hand, many recent work has suggested that strong correlations lead to symmetry breaking within the degenerate flat-band subspace.\cite{girvin_1999,kwan_2021,wang_2016} This spontaneous symmetry-breaking phase is close to a variety of novel phenomenon, such as superconductivity.


Many recent experiments have shown that the correlated insulating phases are well captured by a single $k$-space Slater determinant and Hartree-Fock approximation gives remarkably accurate ground state energy, up to the second perturbation theory.\cite{bultinck_2020}\cite{soejima_2020} The miniband structures and related symmetries of twisted bilayer graphene is close related to this level of accuracy. Many\cite{TBGIII}\cite{bultinck_2020} explained it using an enlarged $U(4)\times U(4)$ symmetry at the chiral limit $w_0=0$, derived the explicit form of the interacting Hamiltonian and proved Slater determinant can be the exact correlated states. Even away from the chiral limit, Hartree-Fock approximation is still remarkably accurate. The combination of two-fold rotation symmetry $C_{2z}$ and time-revesal symmetry  $\mc{T}$ in TBG keep the valley unchanged. The existence of such $C_{2z}\mc{T}$ symmetry in each valley doubles the degeneracy of the low energy bands. With the particle-hole symmetry $\mc{P}$ and chiral symmetry $\mc{S}$, it gives us a clear depiction of the band structures. 


The observations of superconductivity in twisted bilayer graphene has driven people to understand and explain its origin.\cite{girvin_1999}\cite{wang_2016} The flat bands are fragile topology protected by $C_{2z}\mc{T}$ symmetry, but several experiments have found a $C_{2z}\mc{T}$-breaking insulator at charge neutrality.\cite{chatterjee_2020}\cite{das_2021}\cite{liu_2021}\cite{saito_2021} and other symmetry-breaking insulators\cite{jiang_2019}\cite{liu_2021}\cite{wu_2020}. Some\cite{po_2018} has shown that the mean-field treatment necessarily breaks valley and other symmetries to remove the symmetry-enforced band interaction, but the origins are still under debate. In our experiments, we mainly observe two symmetry-breaking states: a) a $C_{2z}\mc{T}$-breaking insulater; b) a three-fold rotation symmetry $C_{3z}$-breaking nematic semimetal. A clear transition between two states is observed for different interlayer Moir\'e potential parameters $w_0/w_1$. 


In this work, we implement a ``careful'' Hartree-Fock approximation and discuss all the possible symmetry-breaking in the implementation. It gives us the ability to detect the spontaneous symmetry-breaking in the twisted bilayer graphene. Then we introduce a new order parameter $\mc{C}_{\vk}$, which can be used to measure the symmetry breaking for any given basis and unitary/antiunitary operators. Using this order parameter, a clear phase transition between quantum anomalous Hall (QAH) state and nematic semimetallic (SM) state is observed by detecting the $C_{2z}\mc{T}/C_{3z}$ symmetry breaking.


\section{Preliminaries}


The tight binding models for monolayer graphene, bilayer graphene, and the Bistritzer--Macdonald (BM) model for the twisted bilayer graphene have been extensively studied in the literature. 
We therefore only provide a minimal introduction to the BM model and the wavefunctions involved; we refer the reader to e.g.~\cite{BultinckKhalafLiuEtAl2020,BernevigSongRegnaultEtAl2021} and the references therein for a more detailed discussion.
Throughout the paper, we adopt atomic units, except for energies which are reported electron volt.

%The BM wavefunction defined in the moir\'e Brillouin zone (mBZ) has the same structure of a wavefunction defined by a non-interacting Hamiltonian with a periodic potential, except that the wavefunction carries additional indices, such as sublattice, layer, valley, and spin.
Subsequently, we denote the moir\'e unit cell by $\Omega$, its area by $|\Omega|$, and the moir\'e Bravais lattice by $\mathbb{L}$. 
Correspondingly, we denote the moir\'e reciprocal lattice $\mathbb{L}^*$, the mBZ by $\Omega^*$. 
The latter is discretized using a Monkhorst--Pack (MP) grid~\cite{MonkhorstPack1976} of size $N_{\vk}=N_{k_x}\cdot N_{k_y}$.
When the MP grid includes the $\Gamma$-point of the mBZ, the computation can be identified with a moir\'e supercell consisting of $N_{\vk}$ unit cells, and $N_{\vk}\abs{\Omega}$ is called the sample area. 
A given BM wavefunction, i.e., a BM band, can be labeled by a tuple $(n,\vk,\vG,\sigma,l,s,\tau)$, where $n$ is the band index, $\vk\in \mathrm{mBZ}$ is the $\vk$-point index, $\vG\in \mathbb{L}^*$ is the planewave index (also called the shell index),  $\sigma\in\{A=1,B=-1\}$ is the sublattice index, $l\in\{t=1,b=2\}$ is the layer index, $s\in\{\uparrow,\downarrow\}$ is the spin index, and $\tau\in\{\vK,\vK'\}$ is the valley index. 
For simplicity, we follow the assumptions in Ref.~\cite{SoejimaParkerBultinckEtAl2020}, and assume that the system is fully polarized along the spin and valley directions.
This is equivalent to dropping the indices $s,$ $\tau$ and assuming that the system is spin-less and valley-less.
If $\vG$ is replaced by the real space index $\vr$ in the moir\'e supercell, a BM wavefunction can be expressed as 
\begin{equation}
\psi_{n\vk}(\vr,\sigma,l)
=\frac{1}{\sqrt{N_{\vk}}}e^{\I \vk\cdot\vr}u_{n\vk}(\vr,\sigma,l)
=\frac{1}{\sqrt{N_{\vk}}\abs{\Omega}}\sum_{\vG} e^{\I(\vk+\vG)\cdot \vr}u_{n\vk}(\vG,\sigma,l),
\end{equation}
where $u_{n\vk}(\vr,\sigma,l)$ is periodic with respect to $\mathbb{L}$, i.e., $u_{n\vk}(\vr,\sigma,l)=u_{n\vk}(\vr+\vR,\sigma,l), \forall \vR\in\mathbb{L}$.
The normalization condition is chosen such that $u_{n\vk}$ is normalized within the moir\'e unit cell.
Moreover, the factor $\frac{1}{\sqrt{N_{\vk}}}$ ensures that $\psi_{n\vk}$ is normalized within the moir\'e supercell. 
With some abuse of notations, we use $u_{n\vk}(\vr,\sigma,l)$ and $u_{n\vk}(\vG,\sigma,l)$ to denote the coefficients of a BM wavefunction in the real space and reciprocal space, respectively. 
In practical calculations, the number of shell indices $\vG$ needs to be truncated to a finite size $N_{\vG}=N_{G_x}\cdot N_{G_y}$.
Note that throughout the paper, we omit the range of summation unless otherwise specified.
Subsequently, we refer to the set of all planewaves indexed by $\vG$ with sublattice index $\sigma$ and layer index $l$ as the primitive basis of the BM model, and denote the corresponding Fock space by $\mc{F}$.
Let $\hat{c}_{\vk}^{\dagger}(\vG,\sigma,l),\hat{c}_{\vk}(\vG,\sigma,l)$ be the creation and annihilation operators acting on $\mc{F}$, respectively. 
%\FF{The index alpha is not used again!}
%For the sake of brevity, we introduce the internal index $\alpha=(\vG,\sigma,l)$ and write $\hat{c}_{\vk}^{\dagger}(\alpha)=\hat{c}_{\vk}^{\dagger}(\vG,\sigma,l)$.
Then the creation and annihilation operators corresponding to the band $n\vk$ are
\begin{equation}
\label{eqn:creation-op-def}
\begin{split}
\hat{f}^{\dag}_{n\vk} 
=&\sum_{\vG,\sigma,l}\hat{c}_{\vk}^{\dagger}(\vG,\sigma,l)u_{n\vk}(\vG,\sigma,l)
%=\sum_{\alpha} \hat{c}_{\vk}^{\dagger}(\alpha)u_{n\vk}(\alpha)
,\\
\hat{f}_{n\vk} 
=&\sum_{\vG,\sigma,l}\hat{c}_{\vk}(\vG,\sigma,l)u^*_{n\vk}(\vG,\sigma,l)
%=\sum_{\alpha} \hat{c}_{\vk}(\alpha)u^*_{n\vk}(\alpha).
\end{split}
\end{equation}
Here $u_{n\vk}^*$ denotes the complex conjugation of $u_{n\vk}$.
The band creation and annihilation operators satisfy the canonical anticommutation relation $\{\hat{f}^{\dag}_{n\vk},\hat{f}_{n'\vk'}\}
= \delta_{nn'} \delta_{\vk\vk'}$, and define the band basis of the BM model.
Note that the definition of the band creation and annihilation operators can be periodically extended outside the mBZ according to 
\begin{equation}
\hat f^{\dag}_{n(\vk+\vG)}=\hat f^{\dag}_{n\vk}, \quad \hat f_{n(\vk+\vG)}=\hat f_{n\vk}, \quad \vG\in\mathbb{L}^*.
\label{eqn:period_f}
\end{equation}



==> sections/posthf.tex <==
\subsection{Coupled-cluster theory}


Coupled-cluster theory is one of the most widely used post-Hartree-Fock wavefunction methods in quantum chemistry~\cite{BartlettMusial2007}. 
It is built on the exponential ansatz which was independently introduced by Hubbard~\cite{Hubbard1957} and Hugenholtz~\cite{Hugenholtz1957} in 1957 as an alternative to summing many-body perturbation theory contributions order by order. 
In this ansatz the wavefunction takes the form
\begin{equation}
\label{eq:ExponentialParametrization}
|\Psi \rangle 
=
e^{T(\vt)}|\Phi_0 \rangle
\end{equation}
where 
\begin{equation}
\label{eq:ClusterOperator}
T(\vt)=\sum_\mu t_\mu X_\mu
\end{equation}
is the cluster operator determined by the cluster amplitudes $\vt$, and $|\Phi_0 \rangle$ is a chosen reference Slater determinant (most commonly the Hartree--Fock solution). 
The operators $X_\mu$ are the excitation operators with respect to the chosen reference $\Phi_0$, i.e., 
\begin{equation}
\label{eq:ExcitationOperator}
X_\mu
=
X_{i_1,...,i_k}^{a_1,...,a_k}
=
\hat{a}_{a_1}^\dagger...\hat{a}_{a_k}^\dagger \hat{a}_{i_k}...\hat{a}_{i_1}
\end{equation}
where for the sake of compactness we have combined the occupied orbital indices $\{i_l\}$ and virtual orbital indices $\{a_l\}$ in the multi-index $\mu$. 
The ground state energy can then be characterized by 
\begin{equation}
\label{eq:CCEnergy}
\mathcal{E}(\vt)
=
\langle\Phi_0|e^{-T(\vt)} H e^{T(\vt)}| \Phi_0 \rangle.
\end{equation}
The cluster amplitudes $\vt$ are determined by the coupled-cluster equations, i.e., a set of polynomial equations of at most degree four with respect to $\vt$:
\begin{equation}
\label{eq:CCEquations}
0
\overset{!}{=}
F_\mu(\vt)
=
\langle
\Phi_0|X_\mu^\dagger e^{-T(\vt)}H e^{T(\vt)} |\Phi_0
\rangle,\qquad \forall \mu.
\end{equation}
More compactly, Eq.~\eqref{eq:CCEnergy} and~\eqref{eq:CCEquations} can be combined in the coupled-cluster Lagrangian  
\begin{equation}
\label{eq:CCLagrangian}
\mathcal{L}(\vt, \boldsymbol\lambda)
=
\mathcal{E}(\vt)+\langle \lambda, \vF(\vt)\rangle
=
\langle \Phi_0|(I+\Lambda(\boldsymbol\lambda))e^{-T(\vt)}H e^{T(\vt)} |\Phi_0 \rangle
\end{equation}
where 
\begin{equation}
\label{eq:LambdaClusterOperator}
\Lambda(\boldsymbol\lambda)
=
\sum_\mu \lambda_\mu X^\dagger_\mu.
\end{equation}
The states $|e^{T(\vt)} \Phi_0 \rangle$ and $\langle \Phi_0(I+\Lambda(\lambda))e^{-T(\vt)}|$ are commonly referred to as the right and left coupled-cluster solution, respectively.
Due to the projective nature of Eq.~\eqref{eq:CCEnergy} and~\eqref{eq:CCEquations}, the $N$-RDM in coupled-cluster theory is given by 
%\LL{ This is the $N$-particle DM. The 1-RDM should involve traces with respect to the creation and annihilation operator.} 
%\FF{Very important, thanks!}
\begin{equation}
\label{eq:ccNrdm}
\varrho_{\rm CC}(\vt, \boldsymbol\lambda)
=
|e^{T(\vt)} \Phi_0 \rangle\langle
\Phi_0(I+\Lambda(\boldsymbol\lambda))e^{-T(\vt)}|
\end{equation}
ensuring that ${\rm Tr}[H\varrho_{\rm CC}(\vt, \boldsymbol\lambda)]= \mathcal{E}(\vt)$.
The corresponding 1-RDM is then given by
\begin{equation}
\label{eq:cc1rdm}
[P_{\rm CC}(\vt, \boldsymbol\lambda)]_{p, q}
=
\langle \Phi_0(I+\Lambda(\boldsymbol\lambda))e^{-T(\vt)}|
a_p^\dagger a_q
|e^{T(\vt)} \Phi_0 \rangle,
\end{equation}
see~\cite{Helgaker2014} for more details.
We emphasize that this ansatz---in its untruncated form---is equivalent to the full configuration interaction method (i.e., the exact diagonalization method)~\cite{LaestadiusFaulstich2019,Monkhorst1977,Schneider2009}\LL{ Is this the right citation?}\FF{Well, it is `a' reference towards which I am clearly biased. I added the other references, that show the essential parts for the individual directions (they are somewhat hidden though). However, I believe that Andre and I wrote the argument very clearly in this sanibel proceedings, which could be helpful for some readers?}, and is thus computationally infeasible. 
In the past decades, different level of approximations have been suggested to reduce the computational complexity~\cite{BartlettMusial2007,ChanKallayGauss2004,Piecuch2010}. The variant used in the subsequent simulations (and arguably one of the most widely used approximate versions of coupled-cluster theory) is the truncation of the cluster operator in Eq.~\eqref{eq:ClusterOperator} to only contain one-body and two-body excitations, also known as the coupled cluster singles and doubles (CCSD) method.
Note that due to the exponentiation of the cluster operator, the corresponding wavefunction expansion in Eq.~\eqref{eq:ExponentialParametrization} will still contain contributions from higher-body terms.  
One of the central benefits of the exponential ansatz is that it ensures that the energy is size consistent and size extensive, in particular, for (rank complete) truncations of $T$ such as in CCSD~\cite{Helgaker2014}.
The treatment of spin, i.e., restricted (R), unrestricted (U) and generalized (G), as in Hartree--Fock theory, carries on to coupled cluster calculations. 
%Here we shall employ a spin generalized treatment abbreviated GCCSD. 

\subsection{Implementation in PySCF}


The CCSD method is widely implemented in different electronic structure software packages. 
We here use the Python-based Simulations of Chemistry Framework (PySCF)~\cite{SunBerkelbachBluntEtAl2018, SunZhangBanerjeeEtAl2020}. 
The IBM model in \cref{eqn:IBM_Ham} can be defined as a ``customized Hamiltonian'' accessed through the one- and two-electron integrals, referred to as \texttt{h1e} and \texttt{eri}.
These integrals are complex valued, therefore, minor adjustments to PySCF need to be made to enable calculations using these customized Hamiltonians.
We also use the molecular formulation in PySCF, i.e., the \texttt{h1e} and \texttt{eri} are stored without taking advantage of the $\vk$-point symmetry~\cite{McClainSunChanEtAl2017}. This can increases the storage cost by a factor of $N_\vk$, and the computational cost by a polynomial of $N_\vk$.
However, PySCF for crystalline systems taking advantage of the $\vk$-point symmetry also requires further adjustments such as density fitting, which is not currently implemented for the IBM model.

%This goes beyond initial correlated calculations of the IBM model employing electronic structure software and shall consequently be postpone for future works.

Once \texttt{h1e} and \texttt{eri} are constructed, the use of the PySCF software packages allows us to perform GHF and GCCSD calculations on the same footing with a simple code structure.  Here is an example:

\begin{lstlisting}[language=Python, caption=Example code running GHF and GCCSD in PySCF from precomputed integrals.]
from pyscf import gto, scf, cc 

def get_veff(mol, dm, *args):       
    vj, vk= scf.hf.dot_eri_dm(eri, 
    return vj- vk                  
                                    
mol= gto.M()                       
mol.incore_anyway= True            
mol.nelectron= nelec 
                                    
ghf_mf= scf.GHF(mol)               
ghf_mf.get_hcore= lambda *args: h1e
ghf_mf.get_ovlp= lambda *args: ovlp
ghf_mf._eri= eri
ghf_mf.get_veff= get_veff          
                                    
# Running GHF
ghf_mf.kernel()

# Running GCCSD
gcc = cc.GCCSD(ghf_mf)  
gcc.kernel()            
\end{lstlisting}

After the calculations, PySCF also provides compact instructions to evalaute the 1-RDMs so that we can evalaute the observables to detect the symmetry breaking in  Section~\ref{sec:symm}.


==> sections/symmetries_old.tex <==
Both the BM model and the IBM model satisfy a large number of symmetries~\cite{BultinckKhalafLiuEtAl2020}, which can be written as a composition of operators from two different classes (1) Euclidean symmetries (i.e. translations, rotations, and reflections) and (2) complex conjugation.
In the spinless, valleyless regime, the symmetry operation must map the $\vK$ valley to itself, which significantly restricts the number of available symmetry operations. \cref{tab:symmetry} summarizes the relevant symmetry operations in this paper. 
In particular, we focus on the $C_{2 z} \mc{T}$ and $C_{3z}$ symmetries.
The BM model is a non-interacting theory. The 1-RDM satisfies both symmetries, and the corresponding ground state is a band metal. 
On the other hand, the 1-RDM of the IBM model solved at the Hatree-Fock level may spontaneously break such symmetries. 
Our main goal is to characterize the symmetry breaking of the 1-RDM in different parameter regimes. 
If the $C_{2 z} \mc{T}$ symmetry is broken but the $C_{3z}$ symmetry is satisfied, the system is in the quantum anomalous hall (QAH) state. If the $C_{2 z} \mc{T}$ symmetry is satisfied but the $C_{3z}$ symmetry is broken, the system is in the nematic metal (NM) state. 
It is interesting that in the IBM model, one and only one symmetry is observed to be broken at any given parameter regime~\cite{}. 

Although the IBM model is expected to satisfy both the $C_{2 z} \mc{T}$ and $C_{3z}$ symmetries in the continuous limit, such symmetries may be nonetheless weakly broken due to the finite number of shells, $\vk$-points, and the choice of the subtraction term in $\hat{H}_0$.
Therefore we would also like to numerically verify that the IBM Hamiltonian satisfies these symmetries, and/or the extent to which a symmetry is broken by the numerical schemes.  
For both purposes, it is desirable that the order parameters do not depend on the choice of the gauge of the bands.





\begin{table}[ht]
\begin{center}
\renewcommand{\arraystretch}{1.2} %% KDS Makes things a bit eaiser to read imo
\begin{tabular}{l|l|l|l}
\hline Symmetry & Real space & Momentum space &Type \\
\hline$C_{2 z}$ & swap sublattice & swap valleys; \\
& & $\mathbf{k} \rightarrow-\mathbf{k}$ & Unitary\\
\hline$C_{3z}$ & rotate by $120^{\circ}$ & $\mathbf{k} \rightarrow C_{3z}\mathbf{k}$ & Unitary\\
\hline $\mathcal{T}$ & & swap valley; \\
& & $\mathbf{k} \rightarrow-\mathbf{k}$ & Antiunitary\\
\hline $C_{2 z} \mc{T}$ & swap sublattice & $\vk\to\vk$ & Antiunitary\\
\hline
\end{tabular}
\end{center}
\caption{Relevant symmetry operations for the spinless, valleyless IBM model. }
\label{tab:symmetry}
\end{table}

\LL{ Give a picture depicing the action of $C2zT$ and $C3z$ in the real space} \kds{I will make beautiful pictures shortly}

In second quantization, a symmetry operation $g$ is defined by its action on the Fock space $\mc{F}$. By Wigner's theorem \FF{reference?}, any symmetry operation must either be unitary or antiunitary. 
If $g$ is unitary, then for any $a\in\CC$ and any $\ket{\Psi}\in\mc{F}$ $g(a\ket{\Psi})=a g\ket{\Psi}$. 
If $g$ is antiunitary, then $g(a\ket{\Psi})=a^* g\ket{\Psi}$. In particular, $g i g^{-1}=-i$. 
We recall that any anti-unitary symmetry $g$ can be written as $g=\wt{g} \mc{K}$, where $\wt{g}$ is a unitary symmetry and $\mc{K}$ is complex conjugation. \LL{ add a citation} 
Throughout the discussion of this section, we only consider unitary symmetries, we prove analogous results for antiunitary symmetries in Appendix \ref{sec:antiunitary} and summarize the results for both unitary and antiunitary symmetries in Table \ref{tab:symm-breaking}.

\subsection{Representation matrix and sewing matrix}

For any point group symmetry $g$, due to the properties of the Bloch transform, there exists a unitary $D(g)$, called the \textit{representation matrix}, so that the creation operators transform via the rule
\begin{equation}
\begin{split}
    (g \hat{c}_{\vk}^\dag g^{-1})(\alpha) & = \sum_{\alpha'} \hat{c}_{g\vk}^\dag(\alpha') [D(g)]_{\alpha',\alpha} \\
    (g \hat{c}_{\vk} g^{-1})(\alpha) & = \sum_{\alpha'} \hat{c}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha}^{*}
\end{split}
\end{equation}
where $g\vk$ denotes the action of the symmetry $g$ in $\vk$-space and $\hat{c}_{\vk}$ are the primitive creation operators defined in Section \ref{sec:ibm_model}. 
In particular, note that the representation matrix does not depend on $\vk$. 


To study the symmetries of IBM model, we will need to understand how the symmetry $g$ transforms the annihilation operators $f_{n\vk}^\dagger$. We consider the action of $g$ on the BM Hamiltonian and show can be written in terms of the representation matrix $D(g)$.
Suppose we have the quadratic Hamiltonian in the primitive basis $\hat{H}=\sum_{\vk}\sum_{\alpha,\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)$. 
 If $g$ is a unitary symmetry with corresponding representation matrix $D(g)$, then
\begin{equation}
\begin{split}
g\hat{H} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
=& \sum_{\vk} [D(g)h(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
\end{split}
\end{equation}

If $\hat{H}$ is invariant under $g$, i.e., $g\hat{H}g^{-1}=\hat{H}$, then this calculation shows that at the matrix level:
\begin{equation}
D(g) h(\vk)=h(g\vk) D(g).
\end{equation}
In other words, 
\begin{equation}
h(g\vk)D(g)u_{n\vk}=D(g)h(\vk)u_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk},
\end{equation}
or equivalently $D(g)u_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$.

This allows us to define a ``sewing matrix'', $[B(g)]_{\vk}$,
\begin{equation}
\label{eqn:matrix_representation}
(D(g) u_{n\vk})(\alpha)=
\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}(\alpha')=
\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
\end{equation}
Here
\begin{equation}
\label{sec:sewing-def}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk} | D(g) | u_{n\vk}},
%[B(g)]_{\vk,mn} := \sum_{\alpha,\alpha'} u_{m,g\vk}(\alpha) [D(g)]_{\alpha,\alpha'} u_{n\vk}(\alpha').
\end{equation}
where the bra-ket notation denotes contraction over the internal indices
$\alpha,\alpha'$. When the system is gapped, $[B(g)]_{\vk}$ is a unitary matrix
(using a contour integral argument, see Appendix \ref{sec:contour-argument}).
Given the definition of sewing matrices, for unitary operator $g$, one can
calculate that:

%\QZ{ The original representation matrix $D(g)$ is defined in the space of combined indices $\alpha$, while sewing matrix $[B(g)]_{\vk}$ is defined in the band space. It's obvious that the symmetry operation is complete using the representation matrix. Using sewing matrix, the symmetry operation is also complete when all the bands are used. In practice, the number of bands is limited. Therefore, our goal is that the symmetry operations of our interests are ``closed'' and ``complete'' using the corresponding sewing matrices: Given a set of bands $\{u_{n\vk}\}_{n,\vk}$, a)``closed'':  for any unitary/antiunitary operator $g$ of interest, $\sum_{m}  u_{m,g\vk} [B(g)]_{\vk,mn}\in\{u_{n\vk}\}_{n,\vk}$; b) ``complete'': for any $u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ and unitary (antiunitary) operator $g$ of interest, $D(g)u_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$ ($D(g)u^*_{n\vk}\in\{u_{n\vk}\}_{n,\vk}$) and $D(g)u_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$ ($D(g)u^*_{n\vk}=\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}$). In this note, we are particularly interested in the spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetry. In a single-valley, spinless system, one pair of flat bands with different sublattice index $\sigma=\pm$ is enough to satisfy the conditions above. More details are in Section \ref{sec:ibm-symm}}
%\LL{ It seems that a projection operator approach might be a better way to go than the abstract "closed" and "complete" concepts. Let us discuss this.} 
\begin{equation}
\begin{split}
g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}(\alpha')\\
=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
u_{n\vk}(\alpha)\\
=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
\end{split}
\label{eqn:sewing_transf_unitary}
\end{equation}
Hence the sewing matrices encode how $\hat{f}^{\dag}_{n\vk}$ transforms under the symmetry action.

%
%\LL{ Appendix?} \kds{I'd like to keep the formula for the sewing matrix in the main text so people implementing this don't need to look at the appendix, but otherwise let's move the rest to the appendix?}
%Now to turn to consider antiunitary symmetries. Since any antiunitary transformation can be written as $g \mc{K}$ where $g$ is a unitary transform and $\mc{K}$ is complex conjugation, similar calculations show that if $\hat{H}_{\mathrm{BM}}$ is invariant under an antiunitary symmetry then the corresponding matrix equation is:
%\begin{equation}
%D(g) h(\vk)=h(g\vk)^* D(g).
%\end{equation}
%From this matrix relation, one can check that the corresponding sewing matrix can be defined by the relations:
%\begin{equation}
%\begin{split}
%(D(g) u_{n\vk})(\alpha) & =
%\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u_{n\vk}^*(\alpha')=
%\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]^{\text{anti}}_{\vk,mn} \\
%[B(g)]^{\text{anti}}_{\vk,mn} & = \braket{u_{m,g\vk} | D(g) | u^*_{n\vk}}.
%\end{split}
%\end{equation}
%Using these definitions, we can now calculate how $f^\dag_{n\vk}$ transforms under antiunitary symmetry: 
%\[
%\begin{split}
%(g \mc{K}) \hat{f}^{\dag}_{n\vk} (g \mc{K})^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u_{n\vk}^*(\alpha')\\
%=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
%u_{n\vk}^*(\alpha)\\
%=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]^{\text{anti}}_{\vk,mn} \\
%=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]^{\text{anti}}_{\vk,mn}.
%\end{split}
%\]
%


%\QZ{Maybe move the antiunitary case to the Appendix.}
%
%The case when $g$ is antiunitary is similar. 
%Here
%\begin{equation}
%\begin{split}
%g\hat{H}_{\mathrm{BM}} g^{-1}=&g \sum_{\vk} \sum_{\alpha\beta}[h(\vk)]_{\alpha\beta} \hat{c}^{\dag}_{\vk}(\alpha) \hat{c}_{\vk}(\beta)g^{-1}\\
%=& \sum_{\vk} \sum_{\alpha\beta} \sum_{\alpha'\beta'}[h(\vk)]^*_{\alpha\beta} \hat{c}^{\dag}_{g\vk}(\alpha') [D(g)]_{\alpha',\alpha} \hat{c}_{g\vk}(\beta') [D(g)]^*_{\beta',\beta}\\
%=& \sum_{\vk} [D(g)h^*(\vk)D^{\dag}(g)]_{\alpha'\beta'}\hat{c}^{\dag}_{g\vk}(\alpha') \hat{c}_{g\vk}(\beta').
%\end{split}
%\end{equation}
%So
%\begin{equation}
%D(g) h^*(\vk)=h(g\vk) D(g).
%\end{equation}
%Hence
%\begin{equation}
%h(g\vk)D(g) u^*_{n\vk}=D(g) h^*(\vk)u^*_{n\vk}=\varepsilon^*_{n\vk} D(g)u^*_{n\vk}=\varepsilon_{n\vk} D(g)u_{n\vk}.
%\end{equation}
%In other words, $D(g)u^*_{n\vk}$ is an eigenfunction of $h(g\vk)$ with the eigenvalue $\varepsilon_{n,g\vk}=\varepsilon_{n\vk}$. 
%The sewing matrix is then given by 
%\begin{equation}
%(D(g) u^{*}_{n\vk})(\alpha)=
%\sum_{\alpha'} [D(g)]_{\alpha,\alpha'} u^{*}_{n\vk}(\alpha')=
%\sum_{m}  u_{m,g\vk}(\alpha) [B(g)]_{\vk,mn}.
%\end{equation}
%Here 
%\[
%[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u^*_{n\vk}}
%\]
%and $[B(g)]_{\vk}$ is a unitary matrix. The transformation rule remains the same
%\begin{equation}
%\begin{split}
%g \hat{f}^{\dag}_{n\vk} g^{-1}=&\sum_{\alpha}  g\hat{c}_{\vk}^{\dagger}(\alpha) g^{-1}u^*_{n\vk}(\alpha')\\
%=&\sum_{\alpha,\alpha'}  \hat{c}^{\dag}_{g\vk}(\alpha')[D(g)]_{\alpha',\alpha}
%u^*_{n\vk}(\alpha)\\
%=& \sum_{\alpha'} \hat{c}^{\dag}_{g\vk}(\alpha') \sum_{m} u_{m,g\vk}(\alpha') [B(g)]_{\vk,mn} \\
%=& \sum_{m} \hat{f}^{\dag}_{m,g\vk}  [B(g)]_{\vk,mn}.
%\end{split}
%\end{equation}

\subsection{Gauge-invariant detection of symmetry breaking in the 1-RDM}
\label{sec:symm-broken}

Suppose that $\hat{H}_{\mathrm{IBM}}$ indeed satisfies a unitary symmetry $g$, and we are interested in whether the symmetry is spontaneously broken in the mean-field solutions.
If the many-body wavefunction $\ket{\Psi}$ satisfies the symmetry $g$, then
\[
g\ket{\Psi}\bra{\Psi}g^{-1}=\ket{\Psi}\bra{\Psi}.
\]
Here $g$ acting on $\ket{\Psi}$ is implemented by $g$ acting on each individual creation operators, and the vaccum is an eigenfunction of any symmetry $g\ket{0}=\ket{0}$.
Therefore the 1-RDM should satisfy
\begin{equation}
\begin{split}
[P(\vk)]_{nm}=&\braket{\Psi|\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}|\Psi}=\Tr[\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}\ket{\Psi}\bra{\Psi}]\\
=&\Tr[g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}g\ket{\Psi}\bra{\Psi}g^{-1}]\\
=&\braket{\Psi|g\hat{f}^{\dag}_{m\vk} \hat{f}_{n\vk}g^{-1}|\Psi}\\
=&\sum_{pq} [B(g)]_{\vk,pm} [B(g)]^*_{\vk,qn}\braket{\Psi|\hat{f}^{\dag}_{p,g\vk} \hat{f}_{q,g\vk}|\Psi}\\
=&([B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk})_{nm}.
\end{split}
\end{equation}
Therefore we can check the norm 
\begin{equation}
\label{eqn:order-parameter}
\mc{C}_{\vk}(g)=\norm{[B(g)]_{\vk}^{\dag}P(g\vk)[B(g)]_{\vk}-P(\vk)}=\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}
\end{equation}
to detect broken symmetry.

Next, we will show that $\mc{C}_{\vk}(g)$ is invariant under arbitrary unitary rotation. We perform an unitary rotation $U(\vk)$ on the original basis. Towards these ends, suppose that we perform the mapping
\[
\hat{f}^{\dagger}_{n\vk} \mapsto \sum_{n'}\hat{f}^{\dagger}_{n'\vk}[U(\vk)]_{n'n}.
\]

Under this unitary rotation, the 1-RDM is
\begin{equation}
\begin{split}
\label{eq:1rdm-gauge}
[P(\vk)]_{nm}\mapsto&\braket{\Psi|\sum_{m'}\hat{f}^{\dagger}_{m'\vk}[U(\vk)]_{m'm} \sum_{n'}[U(\vk)]^*_{n'n}\hat{f}_{n'\vk}|\Psi}\\
=&\sum_{m'n'}[U(\vk)]_{m'm}[U(\vk)]^*_{n'n}\braket{\Psi|\hat{f}^{\dagger}_{m'\vk} \hat{f}_{n'\vk}|\Psi},\\
=&(U^{\dagger}(\vk)P(\vk)U(\vk))_{nm}.
\end{split}
\end{equation}
By a similar calculation, it can be checked that the sewing matrices transform as:
\begin{equation}
[B(g)]_{\vk,mn} \mapsto (U^{\dagger}(g\vk)B(g)_{\vk}U(\vk))_{mn}
\end{equation}
Therefore, for unitary operator, the norm is
\begin{equation}
\begin{split}
\mc{C}_{\vk}(g)\mapsto&\norm{U^{\dagger}(g\vk)P(g\vk)U(g\vk)U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)-U^{\dagger}(g\vk)[B(g)]_{\vk}U(\vk)U^{\dagger}(\vk)P(\vk)U(\vk)},\\
=&\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)},
\end{split}
\end{equation}
Hence $\mc{C}_{\vk}(g)$ is gauge invariant. 

One can repeat similar calculations for anti-unitary symmetries to derive a gauge-invariant order parameter, we go through such calculations in Appendix \ref{sec:antiunitary} and summarize the results in Table \ref{tab:symm-breaking}.
\begin{center}
\begin{table}[ht]
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{c|cc}
     & Sewing Matrix $[B(g)]_{\vk,mn}$ & Order Parameter $\mc{C}_{\vk}(g)$ \\
     \hline 
    Unitary & $\braket{u_{m,g\vk} | D(g) | u_{n\vk}}$ & $\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)}$ \\
    Anti-Unitary & $\braket{u_{m,g\vk} | D(g) | u^*_{n\vk}}$ & $\norm{P(g\vk)[B(g)]_{\vk}-[B(g)]_{\vk}P(\vk)^*}$
\end{tabular}
\caption{\kds{Summary of Results}}
\label{tab:symm-breaking}
\end{table}
\end{center}
\kds{We need to decide about notation for $\mc{C}_{\vk}(g)$. I originally put $\mc{C}_{\vk}(g)$ and $\mc{C}_{\vk}^{\text{anti}}(g)$, but I realize now it's a little inelegant.} \LL{ I sort of agree. Since $g$ already carries the information of unitary/anti-unitary, maybe we do not need the superscript ``anti''?} \kds{We're kind of abusing notation above. If $g$ is anti-unitary then $D(g)$ should be the representation matrix for $g \mc{K}$ (i.e. the unitary component of $g$). This doesn't really change the overall story, but it's important to be consistent}

\subsection{Connection with the order parameter in the Chern band basis}

Let us also show the connection between $\mc{C}_{\vk}(\mc{C}_{2z}\mc{T})$ and the order parameter used in \cite{SoejimaParkerBultinckEtAl2020} using a particular gauge fixing called the Chern band basis. 
According to the gauge choice of the Chern band basis, the sewing matrix takes the form
\[
[B(C_{2z}\mc{T})]^{\text{anti}}_{\vk}=\sigma_x  e^{\I \theta(\vk)}
\]
for some $\vk$-dependent phase $\theta(\vk)$. 
In this basis, the $C_{2z}\mc{T}$ symmetry breaking is detected by computing
\begin{equation}
\gamma_z(\vk)=\Tr[P(\vk)\sigma_z]=P_{11}(\vk)-P_{22}(\vk).
\end{equation}

On the other hand, the commutator satisfies
\[
P(\vk)[B(C_{2z}\mc{T})]^{\text{anti}}_{\vk}-[B(C_{2z}\mc{T})]^{\text{anti}}_{\vk}P(\vk)=e^{\I \theta(\vk)}
\begin{pmatrix}
P_{21}(\vk)-P_{12}(\vk) & P_{22}(\vk)-P_{11}(\vk)\\
P_{11}(\vk)-P_{22}(\vk) & P_{12}(\vk)-P_{21}(\vk)
\end{pmatrix}
\]
Therefore $\gamma_z(\vk)$ can be interpreted as checking the magnitude of the off-diagonal element of commutator in the Chern band basis. However, the order parameter $\gamma_z(\vk)$ is designed specifically for the Chern band basis and $C_{2z}\mathcal{T}$ symmetry, which is unable to generalize to the other band basis and other symmetries. On the other hand, the commutator is designed for any symmetries of our interests and works for any band basis. Using the norm of commutator, a clear spontaneous symmetry breaking between $C_{2z}\mc{T}$ and $C_{3z}$ symmetries is observed for both BM band basis and Chern band basis in Section \ref{sec:numerical}.



%When the energy band basis $\hat{f}^{\dagger}_{n\vk}$ is fixed, the matrix representations of unitary/antiunitary operators are also fixed. In the other word, sewing matrices are the same up to a arbitrary unitary rotation and explicit forms of sewing matrices can be obtained only when this unitary rotation is fixed.


\subsection{Generalization and multi-band case}
\label{sec:multi-band}

In our previous sections, two flat bands $u_{\pm1,\vk}$ with different sublattice index $\sigma=\pm$ are used to project the Hamiltonian and compute the corresponding sewing matrices. Meanwhile, we make the assumption that all the states with band index $n<-1$ ($n>1$) are fully occupied (unoccupied). 
This assumption is valid for the first magic angle $\theta=1.1^{\circ}$, where the two flat bands are isolated from the other energy bands in the band structure of BM model. 
For the other magic angles, there may not exist such isolated flat bands\LL{ cite}. 
\LL{ Even for the first magic angle, it may be desirable to include more bands to systematically improve the accuracy of the IBM model.} 
Therefore, we need to include more bands in our projection in order to get numerically accurate results. Generally, we assume that $2N_{\max}$ bands are used and all the states with band index $n<-N_{\max}$ ($n>N_{\max}$) are full (empty). Away from the flat band case, the band energies are also relatively away from zero. One more symmetry needs to be defined here for the multi-band case, which is unitary ``particle-hole symmetry'' $\mc{P}$\cite{song_2019,TBGII,TBGIII}:
\begin{equation}
[D(\mc{P})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',-\vG} \delta_{l',-l} \delta_{\sigma',\sigma}\zeta_l,
\end{equation}
where $\mc{P}\vk=-\vk$ and $\zeta_l=\pm1$ for $l=\pm$. Note that $\mc{P}$ anticommutes with the BM Hamiltonian and $\mc{P}$ maps creation operators to creation operators (rather than annihilation operators)\LL{ cite} . Therefore, ``particle-hole symmetry'' is mainly a map from positive energy band $u_{n\vk}$ to negative energy band $u_{-n\vk}$. Using the particle-hole symmetry $\mc{P}$ and rotation symmetry $C_{2z}$, the band structure of the BM Hamiltonian has the property:
\begin{equation}
    \epsilon_{n,\vk}=-\epsilon_{-n,-\vk},\ \epsilon_{n,\vk}=\epsilon_{n,-\vk}\ \to\ \epsilon_{n,\vk}=-\epsilon_{-n,\vk}.
\end{equation}

\LL{Can we say how to choose these additional bands to satisfy the particle hole symmetry? The easiest way is probably to cite some paper saying that for some $N_{max}>1$ there is another gap separating the bands away from other bands.} 
This band structure also implicitly reflects that $\epsilon_{1,\vk}=\epsilon_{-1,\vk}=0$ in the two flat band case. Away from the flat band case, one pair of bands with positive/negative energies should be included in our set of bands and this pair is connected by the ``particle-hole symmetry''. \LL{ This part seems out of date now.} Besides that, in order to ensure the ``completeness'' of the symmetry operation, $u_{n\vk}$ and $D(g)u_{n\vk}$ should also be included. with this setup, our norm of the commutator can be generalized to the multi-band case by defining
\begin{equation}
[B(g)]_{\vk,mn}=\braket{u_{m,g\vk}|D(g)|u_{n\vk}},\ \ \ m,n\in[-N_{\max},N_{\max}].
\end{equation}


% This is enough for our discussion about $C_{2z}\mc{T}$ and $C_{3z}$ symmetry in the single-valley, spinless system. However, if we want to further discuss about other symmetries, more bands are needed. One example is the rotation symmetry $C_{2x}$:
% \begin{equation}
% [D(C_{2x})]_{\vG'\sigma'l',\vG\sigma l} = \delta_{\vG',C_{2x}\vG} \delta_{l',-l} \left(\sigma_x\right)_{\sigma',\sigma},
% \end{equation}
% where $C_{2x}\vk=C_{2x}\left(k_x,k_y\right)=\left(k_x,-k_y\right)$.

% The sewing matrices are $[B(C_{2x})]_{\vk,mn}=[B(C_{2z})]_{\vk,mn}$ if only two flat bands are used. Moreover, the ``completeness'' is broken since $D(C_{2z})$

\subsection{Symmetries of the IBM Model}
\label{sec:ibm-symm}

\LL{ Extra thing: for $\hat{H}_I$ it is sufficient to check that $\hat{\rho}_{\vq}$ satisfies the symmetry} 

For the interacting BM Hamiltonian, it's sufficient to verify  \LL{small thing: there is normal ordering involved} 
\begin{equation}
\begin{split}
g\hat{H}_Ig^{-1}&=\frac{1}{2 \abs{\Omega}N_{\vk}} 
\sum_{\vq} V(\vq)g\hat{\rho}_{\vq}g^{-1}g\hat{\rho}_{-\vq}g^{-1},\\
\Longleftrightarrow&\\
g\hat{\rho}_{\vq}g^{-1}&=g\sum_{\vk\in \Omega^*} \sum_{mn} \hat f_{m\vk}^{\dagger} [\Lambda_{\vk}(\vq)]_{mn} \hat f_{n(\vk+\vq)}g^{-1},\\
&=\sum_{\vk}\sum_{mn}\sum_{m'n'}[\Lambda_{\vk}(\vq)]_{mn}\hat{f}^{\dag}_{m',g\vk}[B(g)]_{\vk,m'm}\hat{f}_{n,g(\vk+\vq)}[B(g)]^*_{\vk,}
\end{split}
\end{equation}





==> tikzlibraryquantikz.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.6
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.6:
%	changed packaging so there isn't a compile warning any more
%	modified the meter command so that \meter[draw=blue]{} colours everything blue, not just outline.
%	added trash command
%	added \ctrlbundle command so that \ctrl works well with \qwbundle[alternate]. If you supple \ctrlbundle[2]{}, then the bundle only contains 2 wires instead of the default of 3
%	\qwbundle[alternate] now also works with the parameter \qwbundle[alternate=2] to only have 2 wires in the bundle.
%	added \midstick. Works a bit like rstick and lstick, but reserves space for the text. Can choose to have brackets=none|left|right|both (default is both). Gives better method for circuit identities and other things.
%	added "align equals at" key for setting circuit identities (specifies wire number that should line up with equals. can be non-integer)
%	added makeebit command. accepts one parameter which is the text. Haven't got tyling and different angles of the split working yet.
%   added bundle option to supplement nwires and cwires.
%	fixed bug where you couldn't put a wire command after the declaration of a multi-qubit gate command.
%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

%\ProvidesPackage{quantikz}[2020/04/27 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools,pgfmath}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings,math}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\pgfkeysgetvalue{/quantikz/bundle}{\bundle}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\IfInList{1}{\bundle}{\qwbundle[alternate]{}}{\qw}}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomc{\noexpand\vqbundleexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\IfInList{\val}{\bundle}{\newcomc}{\newcomb}}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}%
 		\dotikzset%
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}%
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}%
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1%
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}%
 		   \dotikzset%
 		   \globaldefs=0%
%		
 	}
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%import options
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}

\newcommand\midstick[2][]{%
	\hphantom{\text{gg#2gg}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\mn{\the\numexpr\m-1\relax}
	\edef\k{\the\numexpr\n+\quantwires-1\relax}
	\settowidth{\myl}{gg#2gg}
	%if more than 1 wire, need to reserve space for each wire
	\ifthenelse{\quantwires=1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={\the\myl}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
      	\globaldefs=0
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@mid\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
	}{
	\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[anchor=mid,#2]center:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(midgr-\row-\col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\row-\col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(midgr-\row-\col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\row-\col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

\DeclareDocumentCommand{\makeebit}{O{-45}O{}m}{
	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(#1)}!#1:(\tikztotarget)$) node [anchor=east,style={#2}]{#3} -- (\tikztotarget) }]{d}
}

% \newcommand{\makeebit}[2][-45]{
% 	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!0.707!#1:(\tikztotarget)$) node [anchor=east]{#2} -- (\tikztotarget) }]{d}
% }

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals\globaldefs=0}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.base)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}
}}
%\show\temp
\temp
}
}

%initialise all the pgfkeys for key=value parameter passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}},/tikz/align equals at/.code={\setmiddle{#1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.default=1,alternate/.code={\def\helper{#1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1},bundle/.initial={-1},brackets/.is choice,brackets/.initial=both}
\pgfkeys{/quantikz,brackets/.cd,none/.code={\def\leftbrace{0}\def\rightbrace{0}},left/.code={\def\leftbrace{1}\def\rightbrace{0}},right/.code={\def\leftbrace{0}\def\rightbrace{1}},both/.code={\def\leftbrace{1}\def\rightbrace{1}}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {} \qw}


%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
\newcommand{\vqbundleexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper>0}{
		\arrow[arrows,yshift=0.1cm]{l}
		\ifthenelse{\helper=1}{\arrow[arrows]{l}}{}
		\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}\qw
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
	trash/.style={path picture={\draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},minimum height=2.5em,minimum width=2em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}
